CARROT: A Cost Aware Rate Optimal Router

With the rapid growth in the number of Large Language Models (LLMs), there has been a recent interest in LLM routing, or directing queries to the cheapest LLM that can deliver a suitable response. We conduct a minimax analysis of the routing problem, providing a lower bound and finding that a simple router that predicts both cost and accuracy for each question can be minimax optimal. Inspired by this, we introduce CARROT, a Cost AwaRe Rate Optimal rouTer that selects a model based on estimates of the models' cost and performance. Alongside CARROT, we also introduce the Smart Price-aware ROUTing (SPROUT) dataset to facilitate routing on a wide spectrum of queries with the latest state-of-the-art LLMs. Using SPROUT and prior benchmarks such as Routerbench and open-LLM-leaderboard-v2 we empirically validate CARROT's performance against several alternative routers.

==> YK-macros.tex <==

\def\Avar{\mathrm{Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{\mathrm{aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{\mathrm{avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{\mathrm{bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{\mathrm{Ber}}
\def\bin{\mathrm{bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{\mathrm{cat}}
\def\Cov{\mathrm{Cov}}
\def\cov{\mathrm{cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{\mathrm{cl}}
\def\complex{{\bC}}
\def\cone{\mathrm{cone}}
\def\conv{\mathrm{conv}}
\def\deq{\overset{d}{=}}
\def\det{\mathrm{det}}
\def\diag{\mathrm{diag}}
\def\diam{\mathrm{diam}}
\def\dist{\mathrm{dist}}
\def\dom{\mathrm{dom}}
\def\doop{\mathrm{do}}
\def\dto{\overset\mathrm{d}{\to}}
\def\Ex{{\bE}}
\def\Exp{\mathrm{Exp}}
\def\exp{\mathrm{exp}}
\def\eg{{\it e.g.}}
\def\epi{\mathrm{epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{\mathrm{iid}}
\def\ind{\perp \!\!\! \perp}
\def\intr{\mathrm{int}}
\def\integers{{\bZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{\mathrm{KL}}
\def\ker{\mathrm{ker}}
\def\lspan{\mathrm{span}}
\def\maximize{\mathrm{maximize}}
\def\med{\mathrm{med}}
\def\minimize{\mathrm{minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{\mathrm{Poi}}
\def\Pr{{\bP}}
\def\peq{\overset\mathrm{p}{=}}
\def\plim{\mathrm{plim}}
\def\proj{\mathrm{proj}}
\def\prox{\mathrm{prox}}
\def\pto{\overset\mathrm{p}{\to}}
\def\ran{\mathrm{ran}}
\def\rank{\mathrm{rank}}
\def\reals{{\bR}}
\def\relint{\mathrm{relint}}
\def\sign{\mathrm{sign}}
\def\subjectto{\textrm{subject to}}
\def\supp{\mathrm{supp}}
\def\symm{{\bS}}

\def\tr{\mathrm{tr}}
\def\tube{\mathrm{tube}}
\def\TV{\mathrm{TV}}
\def\unif{\mathrm{unif}}
\def\Var{\mathrm{Var}}
\def\var{\mathrm{var}}
\def\vct{\mathrm{vec}}
\def\veps{\varepsilon}
\def\vol{\mathrm{vol}}
\def\zeros{\mathbf{0}}

\def\openllm{\texttt{open-LLM-leaderboard-v2}}
\def\routerbench{\texttt{RouterBench}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> sections/abstract.tex <==
% There is a rapidly growing number of open-source Large Language Models (LLMs) and benchmark datasets to compare them. While some models dominate these benchmarks, no single model typically achieves the best accuracy in all tasks and use cases. In this work, we address the challenge of selecting the best LLM out of a collection of models for new tasks. We propose a new formulation for the problem, in which benchmark datasets are repurposed to learn a "router" model for this LLM selection, and we show that this problem can be reduced to a collection of binary classification tasks. We demonstrate the utility and limitations of learning model routers from various benchmark datasets, where we consistently improve performance upon using any single model for all tasks.

% With the rapid growth in the number of Large Language Models (LLMs), there has been a recent interest in \emph{LLM routing}, or directing queries to the cheapest LLM that can deliver a suitable response. %This goal often hints at balancing between cost and performance, \eg\ proprietary models offer high performance but are costly, while smaller open-source models are more affordable but frequently underperform. 
% Following this line of work, we introduce CARROT, a Cost AwaRe Rate Optimal rouTer that can select models based on any desired trade-off between performance and cost. Given a query, CARROT selects a model based on estimates for model cost and performance. Its simplicity lends CARROT computational efficiency, while our theoretical analysis demonstrates minimax rate-optimality in its routing performance. Alongside CARROT, we also introduce a new benchmark dataset, the Scalable Price-aware Routing (\newdata) dataset, to facilitate routing with the latest state-of-the-art LLMs. Using \newdata\ and prior benchmarks such as Routerbench and open-LLM-leaderboard-v2 we empirically validate CARROT's performance against several alternative routers. %using the Routerbench, open-LLM-leaderboard-v2 benchmark datasets. Along side CARROT, we also introduce a new benchmark dataset, the Scalable Price-aware Routing (\newdata) dataset, to facilitate routing with latest state-of-the-art LLMs and validate CARROT's performance on \newdata.

% \my{also collect our own dataset with recent models}







%Our core idea relates the routing problem to a classification task with multiple objectives (cost and performance) and then exploits an explicit form of oracle routers to develop this plug-in approach.  We use this plug-in approach to understand the complete cost versus performance trade-off in two benchmark datasets, namely \routerbench\ and \openllm. In particular, for \routerbench\ through routing, we were able to obtain a performance similar to that of GPT-4 at half the cost. On a more technical note, we broaden the framework of minimax study for nonparametric classifications on two fronts: more than two classes and multiple objectives.

With the rapid growth in the number of Large Language Models (LLMs), there has been a recent interest in \emph{LLM routing}, or directing queries to the cheapest LLM that can deliver a suitable response. 
Following this line of work, we introduce CARROT, a Cost AwaRe Rate Optimal rouTer that can select models based on any desired trade-off between performance and cost. Given a query, CARROT selects a model based on estimates of models' cost and performance. Its simplicity lends CARROT computational efficiency, while our theoretical analysis demonstrates minimax rate-optimality in its routing performance. Alongside CARROT, we also introduce the Smart Price-aware ROUTing (\newdata) dataset to facilitate routing on a wide spectrum of queries with the latest state-of-the-art LLMs. Using \newdata\ and prior benchmarks such as Routerbench and open-LLM-leaderboard-v2 we empirically validate CARROT's performance against several alternative routers.

==> sections/conclusion.tex <==
\section{Discussion}
\label{sec:discussion}
% In this paper, we have introduced a series of routers  based on plug-in estimators that output predictions for model cost and accuracy given a query. These routers are computationally efficient in that one only needs to fit the plug-in estimators to smoothly traverse the Pareto frontier of LLM cost and accuracy on a given data set. To establish the statistical efficiency of our routers, we have provided an information-theoretic lower bound on the excess risk of any router in Theorem \ref{thm:lower-bound}. This lower bound is dependent on the smoothness of the underlying accuracy/cost functions (Assumption \ref{assmp:smooth}), the margin of the oracle router (Assumption \ref{assmp:margin}) and the convex combination coefficients $\mu$ used to measure the risk of the router. Through Theorem \ref{thm:upper-bound} we have seen that for an appropriate choice of plug-in estimate (e.g. Local Polynomial Regression) the minimax risk of our routers achieves the lower bound previously established. In practice, we introduced two systems of plug-in estimates for routing: the first uses roberta-base while the second uses a non-parametric regressor (KNN) on text embeddings. On both open-LLM-leaderboard-v2 and RouterBench, each of the routers can achieve performance equal to (or greater than) the best models at significantly reduced cost.

We introduced CARROT, a plug-in based router that is both computationally and statistically efficient. The computational efficiency stems from the requirement of merely calculating the plug-in estimators (see Algorithm \ref{alg:pareto-routers}) to  perform routing %smoothly traverse the Pareto frontier of cost and accuracy for given group LLMs and dataset. 
Since collecting adequate data for router training might be challenging, we investigate CARROT's statistical efficiency in routing through a minimax rate study. To establish the statistical efficiency of CARROT, we have provided an information-theoretic lower bound on the excess risk of any router in Theorem \ref{thm:lower-bound} and corresponding upper bound for CARROT in Theorem \ref{thm:upper-bound}. To ensure a broad scope for CARROT to a diverse set of queries \emph{and} the latest state-of-the-art LLMs, we also introduced the \newdata\ dataset. %Using \newdata\ and other benchmarks such as Routerbench and open-LLM-leaderboard-v2 we empirically validate CARROT's performance. %Overall, our work presents a robust strategy toward building a router with a broad scope across queries, LLMs, and performance metrics.

Our routing and data approach is designed to be forward-looking. CARROT can incorporate many metrics besides performance and cost; an important next step is to explore which other metrics can improve LLM-based decision-making in practice. A related future goal is to benchmark our SPROUT-trained router on enterprise use cases like the Domain Intelligence Benchmark Suite (DIBS)\footnote{\url{https://www.databricks.com/blog/benchmarking-domain-intelligence}} to locate areas of improvement needed in our data.

% Likewise, on release, SPROUT will be designed to include new user queries and new models. Another future goal is to benchmark the \newdata\ data set itself. For example, one could battle test routers trained on \newdata\ a Domain Intelligence Benchmark Suite (DIBS)\footnote{\url{https://www.databricks.com/blog/benchmarking-domain-intelligence}} to locate areas of improvement needed in our data.

==> sections/experiment.tex <==
\section{Routing in benchmark case-studies}
\label{sec:routing-application}
We use CARROT (Algorithm \ref{alg:pareto-routers}) to perform routing on several benchmark datasets. %task on two benchmarks: {RouterBench} \citep{hu2024routerbench} and {Open LLM leaderboard v2} \cite{open-llm-leaderboard-v2}. The broad question that we address here is to understand the performance vs. cost trade-off in LLM predictions. 
% \SM{revisit this once we have all the expt. details.}


\subsection{Datasets} \label{sec:datasets}

%\begin{wrapfigure}[17]{r}{0.5\textwidth} % 'r' for right, '0.4\textwidth' for width

%\vspace{-0.3cm}
    %\centering
    %\includegraphics[width=\linewidth]{plots/open-llm.pdf} % Replace with your image file
    %\caption{This is a wrapped figure.}
    %\label{fig:wrapped}
    %\label{fig:open-llm-leaderboard}
%\end{wrapfigure}


\paragraph{RouterBench:} RouterBench \citep{hu2024routerbench} is a benchmark dataset for routing tasks consisting of approximately 30k prompts and responses from eleven ($M = 11$) different LLMs.  The data includes prompts from 8 benchmarks covering commonsense reasoning, knowledge-based understanding, conversation, math, and coding. %Paired with each question are model responses, estimated costs associated with the responses (which need to be predicted at test time), and finally a performance score on whether a model got the answer correct. All prompts have a single correct answer, and LLM predictions are compared with that correct answer to obtain a performance score as $0/1$, where $1$ corresponds to a correct answer.  
\paragraph{Open LLM leaderboard:} The {Open LLM leaderboard v2}\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard}} \citep{open-llm-leaderboard-v2} is an open-source benchmarking platform that comprises responses and evaluations of a collection of LLMs on six benchmarks comprising a diverse collection of tasks. %As before, the dataset includes the questions, responses from LLMs, and their evaluation scores as $0/1$ based on whether the answer was correct. 
%For this dataset, we focus on the scenario where cost can be deterministically computed for each LLM once we know the input prompt; this scenario is a good approximation to situations in which LLMs are required to sample just a few tokens to accomplish the target task. To compute the cost of an LLM query, we tokenize the input prompt and compute the cost according to the guideline of TogetherAI \footnote{\url{https://www.together.ai/pricing}}. We use $M=18$ different open language models both available in the Open LLM leaderboard v2 and on TogetherAI, including model families such as LLaMa-3.1, Qwen2.5, and Gemma 2. More related details are provided in the Appendix \ref{append:llms_open}. 
%We focus on the following five benchmarks (around 21k examples) from the Open LLM leaderboard v2, which comprise multiple-choice questions: MATH Lvl 5 \citep{hendrycks2021measuringmathematicalproblemsolving}, MMLU-PRO \citep{wang2024mmluprorobustchallengingmultitask}, BBH \citep{suzgun2022challengingbigbenchtaskschainofthought}, GPQA \citep{rein2023gpqagraduatelevelgoogleproofqa}, MUSR \citep{sprague2023musr}. These five benchmarks are varied and designed to simulate real-world scenarios where LLMs encounter a wide range of prompts. MATH Lvl 5 focuses solely on mathematical word problems, whereas MMLU-PRO and GPQA include both mathematical and advanced science questions. In contrast, BBH emphasizes logical deduction and linguistic reasoning challenges. Lastly, MuSR serves as a benchmark for assessing multistep soft reasoning tasks framed within natural language narratives. In situations in which queries are diverse, the router can explore the strengths and weaknesses of each language model.
\paragraph{\newdata:} We introduce (and evaluate CARROT on) \newdata, a large and diverse dataset designed for training and evaluating routers. \newdata\ integrates 13 state-of-the-art language models and prompts from 6 benchmarks, including GPQA \citep{rein2023gpqagraduatelevelgoogleproofqa}, MuSR \citep{sprague2024musrtestinglimitschainofthought}, MMLU-Pro \citep{wang2024mmluprorobustchallengingmultitask}, MATH \citep{hendrycks2021measuringmathematicalproblemsolving}, OpenHermes \citep{teknium_openhermes_2.5}, and RAGBench \citep{friel2025ragbenchexplainablebenchmarkretrievalaugmented}. Compared to existing routing benchmarks such as RouterBench, \newdata\ offers several key advantages: 
\begin{enumerate}
    \item \newdata\ encompasses a highly diverse set of questions, including instruction queries.
    % , which is feasible due to the evaluation based on LLaMa-3.1-70b-Instruct. 
    \item Unlike previous benchmarks, it does not rely on few-shot prompting and utilizes chat templates appropriate for each model, making it more representative of real-world use cases.
    \item It leverages LLaMa-3.1-70b-Instruct \citep{grattafiori2024llama3herdmodels} to evaluate LLM responses against the ground truth, similarly to \citet{ni2024mixeval}. This is crucial for evaluating on open-ended instruction queries as well as mitigating errors associated with traditional automatic evaluation methods like exact match.
    % \footnote{Without in-context examples and when using chat templates LLMs tend to perform better, but exact match evaluation is no longer reliable due to varying answer styles of LLMs.}
    \item We provide input and output token counts for each LLM-prompt pair, enabling flexibility when conducting cost-aware analysis.
\end{enumerate}
We will open-source \newdata\ and a platform that allows practitioners to extend \newdata\ by adding new queries and seamlessly evaluating state-of-the-art models on them. For further details, please refer to Appendix \ref{sec:append:sprout}.
% First,  Second,  Finally, 



%\SM{comment about the diversity in task in these two benchmarks? and how router can help? Connect this to intro.}

\subsection{Estimating the oracle router}
CARROT requires an estimate for the function $\Phi^\star_m(X) = \Ex_P[ Y_m\mid X]$. In our benchmark tasks, $Y_m$ is 2-dimensional, consisting of model performance measured as accuracy and model cost measured in dollars. In the RouterBench and \newdata\ datasets the cost is treated as unknown, while in the Open LLM leaderboard v2, most evaluations are likelihood-based, thus cost is essentially the length of the input, i.e., a known function. In all cases, the accuracy $Y_{\text{acc}, m}$ is binary, and thus %thus $\Phi^\star_m(X) = P(Z_m = 1\mid X)$.  
we can view its estimation as a binary classification problem, where our objective is to predict the probability that $m$-th model will answer the question $X$ correctly, \ie\ $P_m(X) = P(Y_{\text{acc}, m} = 1\mid X)$) $Y_{\text{acc}, m}$. Using this intuition, we train several multi-label classification models $\widehat P: \cX \to [0, 1]^M$ on a training data split consisting of $80\%$ of the full dataset, where the $m$-th coordinate of $\widehat{P}(X)$ is the predicted probability that $m$-th model accurately answers the question $X$. %, \ie\ $\widehat \Phi_m(X) = \widehat P(Z_m = 1\mid X)$. 
To train $\widehat P$ we consider two procedures: 
\begin{enumerate}
    \item  {\bf CARROT (KNN):} We embed the model inputs using the {text-embedding-3-small} model from OpenAI \citep{openai2023textembedding3small}. On these text embeddings, we train a multi-label K-nearest-neighbors (KNN) classifier.

    \item {\bf CARROT (Roberta):} We fine-tune the pre-trained weights of the {{roberta-base}}\footnote{\url{https://huggingface.co/FacebookAI/roberta-base}} architecture. In order to enhance efficiency, across $m$ we allow $\hat{P}$ to share the same network parameters, except for the final classification layer.
    
\end{enumerate}
%(i) We fine-tune the pre-trained weights of the {\texttt{roberta-base}}\footnote{https://huggingface.co/FacebookAI/\texttt{roberta-base}} architecture; to enhance efficiency across $m$ we allow $\hat{P}$ to share the same network parameters, except for the final classification layer. (ii) %{\texttt{roberta-base}}\footnote{https://huggingface.co/FacebookAI/\texttt{roberta-base}} and %\texttt{bert-base-case}\footnote{https://huggingface.co/google-bert/bert-base-uncased}. 
%o further enhance our predictive ability for model correctness, we take a simple multi-task learning approach \citep{caruana1993multitask} to train the $\widehat \Phi_m$'s; they share the same network parameters, except for the final classification layer, which is based on the assumption is that the representation at the penultimate layers for $\widehat \Phi_m$'s are identical. We utilize a \texttt{HuggingFace} API framework \footnote{https://huggingface.co/docs/transformers/en/tasks/sequence\_classification} for training the $\widehat\Phi$, whose exact choices of hyperparameters are provided in Appendix \ref{}. 

As mentioned above, in the RouterBench and \newdata\ task the cost remains to be estimated. We train multi-label regression models $\widehat C: \cX \to \reals^M$, where $\hat{C}_m(X) =\mathbb{E}[Y_{\text{cost}, m}|X]$ is the estimated cost of calling model $m$ for query $X$. In the case of \newdata\ we actually estimate the input and output token count, and convert this to a cost using collected pricing numbers (see Table \ref{tab:price_by_token_newdata}). Depending on the technique used for performance estimation, we use either the {roberta-base} or text-embedder plus KNN strategy outlined above for fitting $\hat{C}$ (note that the models may be altered for a multi-output regression task, but otherwise remain identical).  In the case of Open LLM leaderboard v2, we compute the cost of input $X$ by calculating its length measured as the number of input tokens and retrieving the price per token from TogetherAI (see Table  \ref{tab:llms_open} for prices per 1M of input tokens).

Having estimated the $\widehat \Phi_m$'s, we use them in Algorithm \ref{alg:pareto-routers} to estimate the oracle routers and predict their performances vs costs on the remaining $20\%$ test split of the dataset. These cost-accuracy tradeoff curves are provided in Figure \ref{fig:RouterBench-main} (for RouterBench), Figure  \ref{fig:rexp_open_llm} (Open LLM leaderboard v2), and Figure \ref{fig:ROOT In Distribution} (for \newdata) along with the accuracies and costs of the individual LLMs within the dataset. 

%\SM{also plot how many $\%$ of times GPT4 was called by the router?}

% Our Algorithm \ref{alg:pareto-routers} requires an estimate for the loss regression function $\Phi^\star_m(X) = \Ex_P[\ell\{ Y, f_m (X)\}\mid X]$. Furthermore, a key takeaway from our rate upper bound analysis in Section \ref{sec:upper-bound} is that the performance of our estimated routers depends on the rate of convergence for estimating $\Phi^\star_m(X) = \Ex_P[\ell\{ Y, f_m (X)\}\mid X]$. Alternatively speaking, we need to estimate $\Phi^\star_m(X)$ accurately. 

% Returning to our benchmark case-studies, the $Z_m = \ell\{ Y, f_m (X)\}$'s are binary, and thus $\Phi^\star_m(X) = P(Z_m = 1\mid X)$.  Therefore, we can view the estimation of $\Phi^\star_m(X)$ as a binary classification problem, where our objective is to predict whether the model $m$ will answer the question $X$ correctly. Using this idea, we train a multi-label classification model $\widehat \Phi: \cX \to [0, 1]^M$ on a training datasplit consisting of $80\%$ of the full dataset, where the $m$-th coordinate of $\widehat \Phi(X)$ is the predicted probability that $m$-th model accurately answers the question $X$, \ie\ $\widehat \Phi_m(X) = \widehat P(Z_m = 1\mid X)$. We train $\widehat\Phi$ with \texttt{\texttt{roberta-base}}, \texttt{bert-base-case} architectures. To further enhance our predictive ability for model correctness, we take a simple multi-task learning approach \citep{caruana1993multitask} to train the $\widehat \Phi_m$'s; they share the same network parameters, except for the final classification layer. 

% Having estimated the $\widehat \Phi_m$'s we use them in our Algorithm \ref{alg:pareto-routers} to estimate the Pareto routers and predict their performances vs costs on the remaining $20\%$ test split of the dataset. These accuracy-cost trade-off curves are provided in Figure \ref{}, along with the accuracies and costs of the individual LLMs within the dataset. 

\subsection{Baseline methods}
%We consider two families of benchmarks. The first is a collection of methods that learn a binary router from preference data, while the second baseline is an inefficient version of our estimates for the routing Pareto frontier.
\citet{ong2024routellmlearningroutellms} (RouteLLM) proposes a collection of methods for learning binary routers from preference data (data consisting of queries $q$ and labels $l_{i,j}$ indicating a winner between model $i$ and $j$). While the usage of preference data is slightly different from ours, we implement their methods on our data by creating pseudo-preference data between two models. In particular, we select a costly and high-performing model and a cheaper model and say the costly model wins if and only if it is correct while the cheaper model is incorrect. On this pseudo preference data, we fit two methods from \citet{ong2024routellmlearningroutellms} for learning win probabilities between expensive and cheap models: the first is a matrix factorization method, called {\bf RouteLLM (MF)}, while the second uses fine-tuned {roberta-base}, called {\bf RouteLLM (Roberta)}. A follow-up method to these is Routing on Random Forests (RoRF) from Not-Diamond \citep{notdiamond2023rorf}, referred to as {\bf Not-Diamond RoRF}. This method uses a text-embedder and random forest model to predict the win probability; we provide a comparison to this method with the {text-embedding-3-small} embedder from OpenAI. As in \citet{notdiamond2023rorf}, we use a slightly different procedure to construct the preference data; a label can take one of four possible values (one for each combination of correct/incorrect from each model), and the costly model is favored if either both models are wrong or the cheaper model is incorrect while the expensive model is correct. For RouterBench, we consider GPT-4 and mixtral 8x7b to be the costly and cheaper models while for the Open LLM Leaderboard, we use Qwen2.5 72b and Qwen2.5 7b.

%\textbf{ERM Router:} In the original RouterBench paper, the authors propose using empirical risk minimization (ERM) and linear interpolation to traverse the routing Pareto frontier \citep{hu2024routerbench}. We implement the ERM router and demonstrate that our method allows the practitioner to traverse the Pareto frontier smoothly. This essentially acts as an empirical verification of Lemma \ref{lemma:oracle-router}
\subsection{Results} %In both {RouterBench} and {Open LLM leaderboard v2} benchmarks we train the loss regressor $\widehat \Phi$ over ten different training and test splits of the datasets that are determined by some prespecified seed values. In both Figures \ref{fig:open-llm-leaderboard} and \ref{fig:RouterBench} we provide error-bars for both average accuracy and cost metrics calculated for the individual LLMs and estimated routers for \openllm\ and \RouterBench\ benchmarks. In both cases, the effect of the baseline architecture (\texttt{\texttt{roberta-base}} vs \texttt{bert-base-case}) were negligible, as we did not see significant differences in the estimated Pareto curves. 

\begin{figure}
    \centering
        \includegraphics[width=0.38\textwidth]{plots/RouterBench (2).pdf} 
        %\caption{Test 1}
        %\label{fig:RouterBench}
    %\hfill
    %\begin{minipage}{0.49\textwidth}
      % \includegraphics[width=\textwidth]{plots/router-vs-gpt4.pdf}
      %  \caption{Test 2}
     %   \label{fig:router-vs-gpt4}
    %\end{minipage}
    \vspace{-0.3cm}
\caption{RouterBench: performance of several routers and individual LLMs on test data-split.}
\label{fig:RouterBench-main}
\end{figure}

\paragraph{Performance against baselines:} In {RouterBench} we were unable to achieve significantly better accuracy than GPT-4; however, we were able to greatly reduce the prediction cost. A direct comparison between routers and GPT-4 with respect to average accuracy versus cost is provided in Figure \ref{fig:RouterBench-main}, where we see that routers can achieve an accuracy similar to GPT-4 at half the cost, while achieving $95\%$ of the accuracy at only $20\%$ of the cost. On the other hand, we showed that CARROT can outperform the best model (Qwen2-72B) by a large margin in {Open LLM leaderboard v2} (see Figure \ref{fig:rexp_open_llm}). In both datasets, we see that our routers significantly outperform the binary routers of \citet{ong2024routellmlearningroutellms} and \citet{notdiamond2023rorf}. This is due to the fact that we route to \emph{all possible models}, which increases the accuracy coverage and decreases the cost of the cheapest accurate model for a given query.
\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{plots/hf-leaderboard1.pdf}
    \vspace{-0.3cm}
    \caption{Open LLM leaderboard v2: performance of several routers and individual LLMs on test data-split.}
    \label{fig:rexp_open_llm}
\end{figure}
%In {Open LLM leaderboard v2}, the model {Qwen2-72B} has the best accuracy ($0.563$) %\pm 0.008)
%but has the highest cost (\$$10^{-9}  %\pm 5.5 \times 10^{-6}
%$ per query) while in RouterBench GPT-4 has the best accuracy %($0.833 %\pm %0.008
%$) but has the highest cost (\$$3.3\times 10^{-4} %\pm 5.5 \times 10^{-6}
%$ per query).% Through routing, on Open LLM leaderboard v2 we were able to improve the accuracy almost by $5\%$ and reduce the prediction cost to one-fourth of the previous cost (see Figure \ref{fig:rexp_open_llm}). %(for $\lambda = 0.995$  and  {\texttt{roberta-base}} architecture the accuracy is... %$0.592 \pm 0.007$ and the cost is $5.08\times 10^{-5} \pm 8.8\times 10^{-7}$). 

To verify our theory, we also compare to the ERM router, which directly minimizes ERM risk of \eqref{eq:RM} for a particular combination of accuracy and cost metrics. CARROT matches the ERM router performance, as demonstrated in Appendix Figures \ref{fig:rbenchsupp} and \ref{fig:rexp_open_llm2}, verifying Lemma \ref{lemma:oracle-router}.%the theoretical findings.

% For simplicity, we reserve comparisons of our CARROT to the ERM router, that directly minimizes ERM risk of \eqref{eq:RM} for a particular combination of accuracy and cost metrics, to the supplementary material (\cf\ Figures \ref{fig:rbenchsupp} and \ref{fig:rexp_open_llm2}).

\paragraph{Performance on \newdata:} The performance of CARROT on \newdata\ is illustrated in Figure \ref{fig:ROOT In Distribution}; a trend similar to our findings for RouterBench and the Open-LLM Leaderboard-v2 emerges. Moreover, Figure \ref{fig:IBMMix-spider} shows that CARROT can achieve similar or better performance of {GPT-4o} with a fraction of the cost. 
\begin{figure}
    \centering
\includegraphics[width=.8\linewidth]{plots/fmselect_perf_cost.pdf}

\vspace{-0.3cm}
    \caption{Test performance on \newdata.}
    \label{fig:ROOT In Distribution}
\end{figure}

%In \texttt{RouterBench}  the \texttt{gpt-4-1106-preview} model, which is often considered as the state of the art, had the highest accuracy ($0.788 \pm 0.004$) but at the highest cost ($0.003 \pm 4.02 \times 10^{-5}$). Although we were unable to achieve significantly better accuracy than GPT-4, we were able to greatly reduce the prediction cost. A direct comparison between routers and GPT-4 with respect to average accuracy versus cost is provided in Figure \ref{fig:router-vs-gpt4}, where we see that routers can achieve an accuracy similar to GPT-4 at half the cost, while achieving $95\%$ of the accuracy at only $20\%$ of the cost. 

%\paragraph{Ablation studies:}



% \begin{figure}[h]
%   \centering
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth]{plots/RouterBench.pdf}
%     \caption{First subfigure}
%     \label{fig:RouterBench}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth]{plots/router-vs-gpt4.pdf}
%     \caption{Second subfigure}
%     \label{fig:router-vs-gpt4}
%   \end{subfigure}
%   \caption{A figure with two subfigures}
%   \label{fig:main}
% \end{figure}


\paragraph{How CARROT chooses models:} %We take this opportunity to provide interpretable insights into our model selection process in this application. 
Figure \ref{fig:model selection} presents the distribution of selected models in \newdata\ across some (average cost, average accuracy) pairs in the test split. As we move from left to right in Figure \ref{fig:model selection}, the selection strategy gradually shifts from prioritizing cost efficiency with smaller models such as {llama-3-2-1b-instruct} and {llama-3-2-3b-instruct} to favoring more capable and expensive models like {llama-3-3-70b-instruct}, {gpt-4o}, and {gpt-4o-mini}.

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{plots/fmselect_model_selection.pdf}
    \vspace{-0.3cm}
    \caption{Model selection proportions on \newdata\ across several accuracies on the test split.}
    \label{fig:model selection}
\end{figure}






==> sections/extensions.tex <==
\section{Routing in a general multi-objective framework}\label{sec:general-multi-obj}

In this section, we discuss a natural extension of the routing problem with general metrics. Since most of the constructions are very similar to the construction in the Introduction section \ref{sec:intro}, we keep our discussion short.  Say, we are provided $M$ pre-trained models, denoted as $f_1, \dots,f_M$. Given model $f_m$ and a sample point $(X, Y)$,  we are interested in $L$ different loss metrics, among which the first $L_1 $ many, denoted as $\ell_1\{f_m; X, Y\} , \dots, \ell_{L_1}\{f_m; X, Y\}$, depends on $f_m$, $X$ and $Y$, while the next $L_2 = L - L_1$ many, denoted as $\ell_{L_1+ 1}(f_m; X), \dots , \ell_{L}(f_m; X)$, depends only on $f_m$ and $X$.  In that case we consider a compromise between these $L$ losses: for an $\lambda = (\lambda_1 , \dots, \lambda_L) \in\Delta^{L-1} $ the linear loss trade-off in eq. \eqref{eq:linearized-loss} naturally extends to 
\begin{equation} \label{eq:linearized-loss-gen}
 \textstyle \eta_{\lambda, m}(X, Y) =  \sum_{l = 1}^{L_1}\lambda_l \ell_l\{f_m; X, Y\} + \sum_{l = L_1 + 1}^{L}\lambda_l \ell_l\{f_m; X\}   \,.
\end{equation} 
To make it even more general, assume that we have a classification task with $M$ classes, \ie \ the outcome $Y \in \{1, \dots, M\}$ is now categorical. Additionally, as a multi-objective problem we have $L$ different loss metrics, among which the first $L_1 $ many $\ell_1\{m; X, Y\} , \dots, \ell_{L_1}\{m; X, Y\}$ are losses  of predicting a sample $(X, Y)$ as the class $m$, while the next $L_2 = L - L_1$ many $\ell_{L_1+ 1}\{m; X\}, \dots , \ell_{L}\{m; X\}$ is the cost of predicting the sample $X$ as the class $m$. Then the aggregated loss is 
\begin{equation} \label{eq:linearized-loss-gen-2}
 \textstyle \eta_{\lambda, m}(X, Y) =  \sum_{l = 1}^{L_1}\lambda_l \ell_l\{m; X, Y\} + \sum_{l = L_1 + 1}^{L}\lambda_l \ell_l\{m; X\}   \,.
\end{equation} 

For a particular $\lambda \in \Delta^{L-1}$ we want to estimate the optimal/Bayes/admissible classifier $g_\lambda^\star$ that minimized the average of the aggregates loss trade-off:
\begin{equation}
    \textstyle g_\lambda^\star = \argmin_{g: \cX \to [M]}  \Ex_P\big[\sum_{m = 1}^M \bbI\{g(X) = m\} \eta_{\lambda, m} (X, Y) \big ]
\end{equation}
Similar to Lemma \ref{lemma:oracle-router}, defining $\Phi_{l, m}^\star(X) = \Ex[\ell_l\{f_m; X,Y\} \mid X]$ for $l \in [L_1]$ and $\Phi_{l, m}^\star(X) = \ell_l\{f_m; X\} $ for $l \in \{L_1 + 1, \dots, L\}$ the Bayes classifier $g_\lambda^\star$ has the explicit form  (\cf\ Lemma \ref{lemma:bayes-classifier-gen})
\begin{equation}\label{eq:oracle-router-gen}
  \textstyle  g_\lambda^\star (X) = \argmin_m  \eta_{\lambda, m}(X), ~~ \eta_{\lambda, m}(X) = \sum_{l = 1}^L \lambda_l \Phi_{l, m}^\star (X)\,.
\end{equation}
A natural extension of Algorithm \ref{alg:pareto-routers} requires us to estimate each of the functions $\Phi_{l, m}^\star$ as $\widehat \Phi_{l, m}$ then estimate all Bayes classifiers in a one-shot plug-in approach as:
\[
\textstyle \widehat g_\lambda(X) = \argmin_m  \{\sum_{l = 1}^L \lambda_l \widehat \Phi_{l, m} (X) \}\,.
\] 
Note that, for $l \ge L_1+ 1$ the functions $\Phi_{l, m}^\star$ are known, so they need not be estimated; in these cases, we simply let $\widehat \Phi_{l, m} = \Phi_{l ,m}^\star$. 
Having estimated $\widehat g_\lambda$, we can then evaluate them on a test data split with respect to each of the individual metrics to estimate the Pareto frontier and examine the optimal trade-off between the objectives.
We describe the procedure in Algorithm \ref{alg:pareto-routers-gen}.  

\begin{algorithm}
    \begin{algorithmic}[1]
\Require Dataset $\cD_n$
\State Randomly split the dataset into training and test splits: $\cD_n = \cD_{\text{tr}} \cup \cD_{\text{test}}$. 
\State  Learn estimates $\widehat \Phi_{l, m} (X)$ of the function $\Phi_{l, m}^\star(X)$ using the training split $\cD_{\text{tr}}$. 
\For{$\lambda \in \Delta^{L-1}$}
\State  Define $\widehat \eta_{\lambda, m}(X) =  \sum_{l = 1}^L \lambda_l \widehat \Phi_{l, m} (X)  $ and 
 $\widehat g_\lambda(X) = \argmin_m \widehat \eta_{\lambda, m}(X)$
 \For{$l \in \{1, \dots, L\}$}
 \State Calculate $\widehat \cE_{l, \lambda}  =  \frac1{|\cD_{\text{test}}|} \sum_{(X, Y) \in \cD_{\text{test}}}  \ell_l\{Y, f_{\widehat g_\lambda(X)}(X)\}$
 \EndFor
\EndFor

\Return $\{g_\lambda: \lambda \in \Delta^{L-1}\}$ and $\widehat\cF = \{(\widehat \cE_{1, \lambda}, \dots, \widehat \cE_{L, \lambda}): \lambda \in \Delta^{L-1}\}$. 
\end{algorithmic}
\caption{Learning of Bayes classifiers}
\label{alg:pareto-routers-gen}
\end{algorithm}


Except for some minor differences, the minimax rate analysis of the estimate of $g_\lambda^\star$ is identical to Section \ref{sec:lower-bound}. We assume that
\begin{enumerate}
    \item For $1 \le l \le L_1$ the $\Phi_{l, m}^\star$ functions are $(\beta_l, K_{\beta, l})$-smooth, which is similar to the Assumption \ref{assmp:smooth}. Recall the discussion following Assumption \ref{assmp:smooth}; (1) Since $\Phi_{l, m}$ are known for $l \ge L_1 + 1$ a smoothness assumption on them is not necessary, and (2) We could assume different smoothness for different $\Phi_{l, m}^\star$, \ie\ they are $\beta_{l, m}$ smooth, but the rate will only involve the smallest smoothness, \ie\ $\beta_{l, \min} = \min_m \beta_{l, m}$. Thus, for simplicity, we assume that for a given $l$ the $\beta_{l, m}$ are identical for different $m$. 
    \item The margin condition in Assumption \ref{assmp:margin} is satisfied with the new definition of $\eta_{\lambda, m}(X) = \Ex[\eta_{\lambda, m}(X, Y)\mid X]$ with parameters $(\alpha, K_\alpha)$.
    \item  The $P_X$ is compactly supported and satisfies the strong density condition, as in the assumption \ref{assmp:strong-density}.
\end{enumerate}

%  and that the margin condition is satisfied  Furthermore, we assume the 
% \SM{talk about how the worst smoothness parameter is the one that matters.}


Under these assumptions, we establish the upper and lower bound analysis for the minimax rate of convergence in excess risk
\[
\textstyle \cE_P(g, \lambda) = \cL_P(g, \lambda) - \cL_P(g_\lambda^\star, \lambda)\,.
\]
For this purpose, let us quickly recall the notation and definitions necessary to describe the lower and upper bounds. We denote the class of all probability distributions on $\cX \times \cY$ space by $\cP$.
We also denote $\Gamma = \{g: \cX \to [M]\}$ as the set of all classifiers and $\cA_n$ as the class of learning algorithms, such that an algorithm $\cA_n \ni A_n: \cZ^n \to \Gamma $ that takes the dataset $\cD_n $ as input and produces a classifier $A_n(\cD_n): \cX \to [M]$.

\begin{theorem}
\label{thm:bound-gen}
Suppose that $\max_{l \in  [L_1]}\beta_l <  \nicefrac{d}{\alpha}$. Then we have the following lower and upper bounds for the excess risk. 
\begin{itemize}
    \item {\bf Lower bound:} For $n \ge 1$  and $A_n \in \cA_n$ define $\cE_P(A_n, \lambda) = \Ex_{\cD_n}\big[\cE_P\big(A_n(\cD_n), \lambda\big)\big]$. There exist constants $c_1, c_2> 0$ that are independent of $n$ and $\lambda$ such that for any $n\ge 1$ and $ \lambda \in \Delta^{L-1}$ we have the lower bound
    \begin{equation} \label{eq:lower-bound-gen}
      \textstyle  \min\limits_{A_n \in \cA_n} \max\limits_{P \in \cP} ~~ \cE_P(A_n, \lambda) \ge c \big \{\sum_{l = 1}^{L_1}\lambda_l n^{- \frac{\beta_l}{2\beta_l + d}}\big\}^{1+\alpha} \,.
    \end{equation}  
    \item  {\bf Upper bound:} For $l \le L_1$ and $m\in [M]$ suppose that there are estimators $\widehat\Phi_{l, m}$ for $\Phi^\star_{l, m}$ that satisfies the following: for constants $\rho_{l, 1}, \rho_{l, 2} > 0$ and any $n \ge 1$ and $t > 0$ and almost all $X$ with respect to $P_X$ we have 
    \begin{equation} \label{eq:concentration-phi-gen}
        \max_{P\in \cP} P \big \{ \max_m \big |\widehat \Phi_{l, m} (X) - \Phi^\star_{l, m}  (X)\big |  \ge t\big \} \le  \rho_{l, 1} \exp\big (- \rho_{l,2} a_{l, n}^2 t^2 \big )\,,  
    \end{equation}  where the sequence $\{a_{l, n}; n \ge 1\}\subset (0, \infty)$  increases to $\infty$. Then there exists a $K> 0$ such that for any $n \ge 1$ and $\lambda \in \Delta^{L-1} $ the excess risk for the router $\widehat g_\lambda$ in Algorithm \ref{alg:pareto-routers-gen} is upper bounded as 
    \begin{equation} \label{eq:upper-bound-gen}
      \textstyle   \max\limits_{P\in \cP} \Ex_{\cD_n}\big [\cE_P(\widehat g_\lambda,\lambda)\big ] \le K \big\{ \sum_{l = 1}^{L_1}\lambda_l a_{l, n}^{-1}\big\} ^{1+ \alpha}\,. 
    \end{equation}
    \item  {\bf Local polynomial estimator:} Assume that $\ell_l \{Y_i, f_m(X_i)\}$ are sub-Gaussian, \ie\ there exists constants $c_{l, 1}$ and $c_{l, 2}$ such that  
    \[
    \textstyle P\big ( |\ell_l \{Y, f_m(X)\} | > t \mid X\big ) \le c_{l, 1} e^{-c_{l, 2}t^2}\,. 
    \] If $\psi$ satisfies the regularity conditions with parameter $\beta_l$ in (\cf\ Definition \ref{def:kernel-reg})  and $k = \lfloor \beta_l \rfloor$ then for $h = n^{-\frac{1}{2\beta_l + d}}$ the inequality in \eqref{eq:concentration-phi-gen} holds for 
    \begin{equation}\label{LPR-gen}
    \widehat \Phi_{l, m}(x_0) = \widehat\theta_{x_0}^{(m)}(0), ~~ \widehat \theta_x^{(m)} \in \argmin_{\theta \in \Theta(k)}  \textstyle \sum_{i = 1}^n \psi (\frac{X_i - x_0}{h}) \big [\ell \{Y_i, f_m(X_i)\} - \theta (X_i -x_0 )\big]^2 \,. 
\end{equation}
    with $a_{l, n} = n^{\nicefrac{2\beta_l}{(2\beta_l + d)}}$, where $\Theta(k)$ is the class of all $k$ degree polynomials. 
\end{itemize} 

  
\end{theorem}
% \SM{Discuss the optimality in remarks.} 
\SM{comment about $\max_{l \in  [L_1]}\beta_l <  \nicefrac{d}{\alpha}$.}
We end our section with a few remarks. 

\begin{remark}[Rate optimality for plug-in routers]

Firstly, given that the upper bound in eq.  \eqref{eq:upper-bound-gen} for plug-in router described in Algorithm \ref{alg:pareto-routers-gen} with local-polynomial estimator for $\widehat \Phi_{l, m}(X)$ achieves the same rate of convergence as the lower bound in \eqref{eq:lower-bound} we conclude that the minimax optimal rate of convergence in excess risk is 
\begin{equation} \label{eq:optimal-rate-gen}
    \textstyle \min\limits_{A_n \in \cA_n} \max\limits_{P \in \cP} ~~ \cE_P(A_n, \lambda) \asymp \cO \Big(\big \{\sum_{l = 1}^{L_1}\lambda_l n^{- \frac{\beta_l}{2\beta_l + d}}\big\}^{1+\alpha}\Big)\,. 
\end{equation} Moreover, this also implies that the plug-in router can achieve this optimal rate as long as the bounds in eq. \eqref{eq:concentration-phi-gen} are satisfied with $a_{l, n} = n^{\nicefrac{2\beta_l}{(2\beta_l + d)}}$. 
    
\end{remark}

\begin{remark}[Difficulty in routing with respect to $\lambda$]
Moreover, the rate in eq. \eqref{eq:optimal-rate-gen} implies that for a smaller $\lambda_l$ the errors in estimating $\Phi_{l, m}^\star$ have a lesser impact on the excess risk convergence. This conclusion is very much related to our Remark \ref{remark:diff-in-lambda-lb}, and thus we keep our discussion brief and ask readers to revisit the said remark. We end with a quick observation that the hardest instance to classify is when $\lambda_{l_{\min}} = 1$ for the lowest smoothness parameter, \ie\ $l_{\min} = \argmin_{l \le L_1} \beta_l$. 

    
\end{remark}


\begin{remark}

{\bf (Minimax rate study for non-parametric classification with multiple objectives)}
Compared to \citet{audibert2007Fast}, our study of the optimal minimax rate provided in this section generalizes the setting on three fronts: (1) the number of classes can be more than two, (2) general classification loss functions beyond $0/1$-loss and (3) multiple objectives. In this general setting, we show that the plug-in classifiers described in Algorithm \ref{alg:pareto-routers-gen} are both computationally and statistically (rate optimal) efficient for estimating the entire class of Bayes classifiers $\{g_\lambda^\star: \lambda\in \Delta^{L-1}\}$. 
    
\end{remark}

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Consider a prediction task: Let $(X, Y)$ be a random pair that takes a value in the space $\cZ \triangleq \cX \times \cY$ with a joint distribution $P$. We consider $X \in \cX \subset \reals^d $ as covariates and $Y \in \cY$ as the response, and given $X$ we want to predict $Y$ as a function of $X$.  Although the standard approach would be to learn a prediction model $f: \cX \to \cY$ from $\cD$ using statistical learning methods, learning such $f$ is often very challenging due to the requirement of a large sample size and computing resources. 


Consider a standard prediction task: for an $(X, Y) \in \cX \times \cY$ drawn from the distribution $P$ we want to predict $Y$ using $X$, where $\cX \subset \reals^d$ is the covariates space and $\cY$ is the response space. For the prediction task, we want to learn a predictor $f : \cX \to \cY$ such that, given a new $(X, Y) \sim P$, the error in predicting $Y$ as $f(X)$ is as small as possible. To learn such $f$, we have a dataset $\cD_n = \{(X_i, Y_i)\}_{i = 1}^n \subset \cX \times \cY$ of size $n$ drawn \emph{i.i.d.} from the distribution $P$, and a standard statistical technique is to estimate $f$ by minimizing an empirical risk calculated with $\cD_n$. 
In this paper, we are particularly interested in prediction tasks in which learning $f$ in such a manner is very challenging or even impossible due to the requirements of a large sample size and computing resources. Instead, we have access to a collection of pre-trained models $f_1, \dots, f_M: \cX \to \cY$ that may aid our prediction task, and for a new $X$ we want to pick the ``best capable'' model for prediction.  


As a motivating example, consider the task of building a question and answering (Q\&A) system, \ie\ we want to learn a large language model (LLM) for text generation, which, given a question, generates the correct answer. As is well known by now, training such models from scratch is notoriously difficult in terms of their required data and computation resources, and is certainly outside of the capacity of an everyday researcher. As a more feasible approach, we turn to the Internet, where a collections of pre-trained LLMs are readily available for our use. Rather than training an LLM from scratch, we pick the ``best capable'' model to answer a question.


% But LLMs come in a wide variety of LLMs exist; in terms of their \emph{sizes}, which can range in size from one billion to hundreds of billions of parameters; \emph{expertise}, based on the dataset on which it has been trained, \eg text, math or science Q\&A, as well as \emph{costs} to obtain a prediction.
% Broadly speaking, larger models tend to be more capable but
% come at a higher cost, while smaller models tend to be less capable but cheaper to serve.
% Thus, a learner is presented with the problem of choice: given a new question, which LLM is best suited? 


There is a wide variety of LLMs available in the Internet --- their \emph{sizes} range from less than a billion to hundreds of billion of parameters; they may have a diverse \emph{expertise} based on their training datasets, \eg\ reasoning, math or coding Q\&A's; as well as their \emph{costs} of prediction might also be different. Broadly speaking, larger models (\eg\ GPT4) tend to be more capable but
come at a higher cost, while smaller models tend to be less capable but are cheaper to serve. 
In terms of model capability, we focus on the two following metrics: 
\begin{itemize}
    \item {\bf Prediction error:} we have a prediction loss function $\ell$ such that the error in predicting a response $Y$  as $f_m(X)$ from the $m$-th model is $\ell\{Y, f_m(X)\} \in \reals$. We want to pick the model with the smallest prediction error. 
    \item {\bf Prediction cost:} together with a pre-trained model $f_m$, we also have a cost function $\kappa_m: \cX \to \reals$ that, given an input $X$, quantifies the cost of obtaining the prediction $f_m(X)$ as $\kappa_m(X)$. Usually, the prediction cost for an LLM is related to factors such as the sizes of models, input tokens, etc. 
\end{itemize}
Intuitively, we would like to use a more expensive model like GPT4 for a question that is difficult to answer. On the other hand, a smaller model with less prediction cost might be sufficient for a question that is easy to answer. Thus, we want to find the LLM that can correctly answer a question at the cheapest prediction cost. 

% Thus, we have a problem of choice: \emph{given a new question, which LLM is best suited to answer it?} 



The task of picking the best prediction model is called \emph{routing} and has attracted a growing interest in the LLM community \citep{lu2023routing,wang2023fusing}, due to it's capability of harnessing the complementary expertise of a heterogeneous class of LLMs to achieve better performance at a reduced prediction cost. 
% To formally introduce the problem, assume that we have access to $M$ pre-trained models $f_1, \dots, f_M: \cX \to \cY$ and given a new $X\in \cX$ we need to pick the ``best capable'' one to predict $Y$. 
In this paper, we consider routing with two metrics, namely prediction error and cost, but our framework can also be extended to more than two metrics (\cf\ Section \ref{sec:general-multi-obj}). As hinted before, the two metrics are often at odds with each other: a larger model will have a smaller prediction error, but at a higher cost, whereas a smaller model will have a lower prediction cost but a higher prediction error. This is a well-known issue in most multi-objective learning problems and in such scenarios it is often standard to consider a ``trade-off'' between the prediction error and the cost via a simple weighted linearization: for $\lambda \in [0,1 ]$ we define the trade-off loss as 
\begin{equation} \label{eq:linearized-loss}
  \eta_{\lambda, m}(X, Y) =  \lambda \ell\{Y, f_m(X)\} + (1 - \lambda) \kappa_m(X)  \,.
\end{equation}
For such a particular trade-off our routing problem is formalized as the following: learn a function $g: \cX\to \{1, \dots, M\}$ 
that predicts the index of the model to be used for predicting the final outcome, \ie\ given an $(X, Y)$ we predict $Y$ as $f_{g(X)}(X)$. We refer to such a $g$ as \emph{router}. We want to learn the best possible router, also referred to as oracle router and Pareto router, that  
minimized the average trade-off loss: 
\begin{equation} \label{eq:risk-trade-off}
  \textstyle g_\lambda^\star =   \argmin_g \big \{ \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y) \big]\big \} \,.
\end{equation} Here, the $\lambda$ in the subscript of  $g_\lambda^\star$ emphasises the dependence of oracle router on the trade-off parameter $\lambda$, as for different $\lambda$'s the  $g_\lambda^\star$'s might be different. 

By this point, the readers may have realized that this is inherently a classification problem; routers are essentially classifiers, whose outcomes are indices of LLMs. Often, this is more tractable than learning a predictor $f:\cX \to \cY$ from scratch or through fine-tuning, especially when $P$ includes a diverse set of prediction tasks. 
Both of our benchmark datasets contain the
MMLU \citep{hendrycks2020measuring},
which is a multiple choice question-answer benchmark with 57 different tasks organized by topics. The Open LLM Leaderboard \citep{open-llm-leaderboard-v2} combines MMLU with five other question-answer datasets. While one may find it challenging to train an LLM that is strictly the best on all of these benchmarks, a more feasible approach is to \emph{route through} pre-trained models that are expert in those particular tasks.


Since routing is essentially a classification problem, we can use standard statistical learning techniques to learn the oracle routers; given a $\lambda$ we estimate $g_\lambda^\star$ using an empirical risk minimization (ERM): 
\begin{equation} \label{eq:ERM}
  \textstyle  \widehat g_\lambda = \argmin_g \frac1n \sum_{i = 1}^n \sum_{m = 1}^M \ell_{\text{class}}(g(X_i), m) \eta_{\lambda, m}(X_i, Y_i)\,. 
\end{equation} where $\ell_{\text{class}}$ is a suitable loss for multiclass classification. Moreover, we can evaluate the predictive error and cost for  $\widehat g_\lambda$ on a different test data split $\cD_\text{test} = \{(X_i' ,Y_i')\}_{i = 1}^{n_{\text{test}}} \sim  \textrm{iid} ~  P $: 
\begin{equation} \label{eq:perf-cost}
   \textstyle  \widehat \cE_\lambda  =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \ell\{Y_i', f_{\widehat g_\lambda(X_i')}(X_i')\}, ~~ \widehat \cC _\lambda =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \kappa_{\widehat g_\lambda(X_i')}(X_i')\,. 
\end{equation}



% In our formulation of model routing, we only need to learn a classifier with outcome space $[M]$ that selects the best-suited model for prediction. In other words, we have reduced the outcome space from an arbitrary $\cY$ to a mere $[M]$. 


% such that given a new $(X, Y)$ the model model indexed by $g(X)$ is best suited to predict the outcome $Y$, \ie\ 




% Now, we want to learn a function $g: \cX \to \{1, \dots , M\}$ which, for a new $X$, predicts that the model indexed by $g(X)$ is best suited to predict the outcome. We refer to this $g$ as \emph{router}. For a pair $(X, Y)$ a router $g$  incurs a trade-off loss $\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y)$, and naturally, we want to the best router that minimizes the average of trade-off loss: 
% \begin{equation} \label{eq:risk-trade-off}
%   \textstyle  \min_g \big \{ \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y) \big]\big \} \,.
% \end{equation}
% At this point, the reader may have realized that this is a classification problem with $M$ classes. Often, this is more tractable than learning a predictor $f:\cX \to \cY$ from scratch, especially when $\cY$ is very complicated. For our LLM example, $\cY$ is the space of all possible answers, and training a $f:\cX \to \cY$ is very difficult. In our formulation of model routing, we only need to learn a classifier with outcome space $[M]$ that selects the best-suited model for prediction. In another word, we have reduced the outcome space from  an arbitrary $\cY$ to a mere $[M]$. 




% \begin{itemize}
%     \item {\bf Prediction error:} we have a prediction loss function $\ell$ such that the loss for predicting a response $Y$ using the $m$-th model is $\ell\{Y, f_m(X)\} \in \reals$. We want to pick the model with the smallest loss. 
%     \item {\bf Prediction cost:} together with a pre-trained model $f_m$, we also have a cost function $\kappa_m: \cX \to \reals$ that, given an input $X$, quantifies the cost of obtaining the prediction $f_m(X)$ as $\kappa_m(X)$. Usually, this prediction cost is related to factors such as the sizes of models, input tokens, etc. Although a large model (\eg\ GPT4) can accurately answer most questions, they are also more expensive to use. For a question that is easy to answer, we might turn to a smaller model, which can provide a good answer at a much lower cost. 
% \end{itemize}

% Now we are presented with a problem with multiple objectives: prediction error vs. cost. Moreover, they are often at odds with each other: a larger model will have a smaller prediction error, but at a higher cost, whereas a smaller model will have a lower prediction cost but a higher prediction error.  In such scenarios one often considers a ``trade-off'' loss between the prediction error and the cost via a simple weighted linearization: for $\lambda \in [0,1 ]$
% \begin{equation} \label{eq:linearized-loss}
%   \eta_{\lambda, m}(X, Y) =  \lambda \ell\{Y, f_m(X)\} + (1 - \lambda) \kappa_m(X)  \,.
% \end{equation}
% Now, we want to learn a function $g: \cX \to \{1, \dots , M\}$ which, for a new $X$, predicts that the model indexed by $g(X)$ is best suited to predict the outcome. We refer to this $g$ as \emph{router}. For a pair $(X, Y)$ a router $g$  incurs a trade-off loss $\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y)$, and naturally, we want to the best router that minimizes the average of trade-off loss: 
% \begin{equation} \label{eq:risk-trade-off}
%   \textstyle  \min_g \big \{ \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y) \big]\big \} \,.
% \end{equation}
% At this point, the reader may have realized that this is a classification problem with $M$ classes. Often, this is more tractable than learning a predictor $f:\cX \to \cY$ from scratch, especially when $\cY$ is very complicated. For our LLM example, $\cY$ is the space of all possible answers, and training a $f:\cX \to \cY$ is very difficult. In our formulation of model routing, we only need to learn a classifier with outcome space $[M]$ that selects the best-suited model for prediction. In another word, we have reduced the outcome space from  an arbitrary $\cY$ to a mere $[M]$. 
% In general, this routing approach is particularly suited for very complicated $\cY$, as in those cases learning a direct predictive model $f:\cX \to \cY$ usually requires a large dataset and computation resource.  



% Returning to our routing task,  we show in Lemma \ref{lemma:oracle-router}, for $\eta_{\lambda, m} ^\star(X) = \Ex_P [\eta_{\lambda, m}(X, Y) \mid X]$, the best router that minimizes the trade-off risk \eqref{eq:risk-trade-off} is $g_\lambda^\star(X) = \argmin_l ~ \eta_{\lambda, m} ^\star(X)$. We also refer to $g_\lambda^\star$ as a Pareto router. We can use standard statistical learning techniques to learn this Pareto routers; given a $\lambda$ we estimate $g_\lambda^\star$ using an empirical risk minimization (ERM): 
% \begin{equation}
%   \textstyle  \widehat g_\lambda = \argmin_g \frac1n \sum_{i = 1}^n \sum_{m = 1}^M \ell_{\text{class}}(g(X_i), m) \eta_{\lambda, m}(X_i, Y_i)\,. 
% \end{equation} where $\ell_{\text{class}}$ is a suitable loss for multiclass classification. Moreover, we can evaluate the predictive error and cost for  $\widehat g_\lambda$ on a different test data split $\cD_\text{test} = \{(X_i' ,Y_i')\}_{i = 1}^{n_{\text{test}}} \sim  \textrm{iid} ~  P $: 
% \begin{equation}
%    \textstyle  \widehat \cE_\lambda  =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \ell\{Y_i', f_{\widehat g_\lambda(X_i')}(X_i')\}, ~~ \widehat \cC _\lambda =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \kappa_{\widehat g_\lambda(X_i')}(X_i')\,. 
% \end{equation}



% \todo{revise from here.}
\noindent What is a suitable trade-off, \ie\ what is a good choice of $\lambda$? Instead of making this decision on our own, we want users to decide on this based on their preferred trade-off between performance and cost. To aid in this decision, we want to provide them with an estimate of the Pareto frontier curve to exhibit the trade-off in the prediction error and cost
\begin{equation}
    \textstyle \widehat \cF = \{(\widehat \cE _\lambda, \widehat \cC_\lambda ): \lambda \in [0, 1]\}\,, 
\end{equation} along with the class of all estimates of the oracle routers $\{\widehat g_\lambda: \lambda \in [0, 1]\}$. A naive approach could be to report both $\widehat g_\lambda$ and $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ on a sufficiently fine grid of $\lambda$, where for each $\lambda$ on the grid, they are estimated using eq. \eqref{eq:ERM} and \eqref{eq:perf-cost}. But this defeats one the main purpose of the routing problem, reducing the computational requirement, as we now need to learn $\widehat g_\lambda$ on this suitable grid of $\lambda$. 


% Suppose that we want users to pick this $\lambda$ according to their preferred trade-off between performance and cost. For this, we want to provide them with an estimate of the Pareto frontier curve for the error and cost trade-off $\widehat \cF = \{(\widehat \cE _\lambda, \widehat \cC_\lambda ): \lambda \in [0, 1]\}$ so that they can make informed decisions about $\lambda$. Notice that, to calculate $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ we require $\widehat g_\lambda$. So, a naive approach could be to learn $\widehat g_\lambda$ and $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ on a sufficiently fine grid of $\lambda$'s and then interpolate for $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ on the remaining $\lambda$'s to estimate the full curve. But this defeats the main purpose of the routing problem, reducing the computational requirement, as we now need to learn $\widehat g_\lambda$ on this suitable grid of $\lambda$. 


\emph{\bf Is there a more efficient way?} In this paper, we devise a computationally efficient approach to learn $\widehat g_\lambda$ for all $\lambda \in [0, 1]$ and use them to calculate $\widehat \cF$. The key intuition of our approach lies in the mathematical form of the oracle routers:  we establish in Lemma \ref{lemma:oracle-router} that  $g_\lambda^\star(X) = \argmin_m \eta_{\lambda, m} ^\star(X)$  where the loss regression functions $\eta_{\lambda, m} ^\star(X) = \Ex _P[\eta_{\lambda, m}(X, Y)\mid X]$ can be decomposed as  
\begin{equation}\label{eq:reg-decomposition}
    \eta_{\lambda, m} ^\star(X) = \Ex _P[\eta_{\lambda, m}(X, Y)\mid X] = \lambda \Ex_P[\ell\{Y , f_m(X)\}\mid X] + (1 - \lambda) \kappa_m(X)\,. 
\end{equation} 
The decomposition follows directly from Eq. \eqref{eq:linearized-loss}. Within this decomposition, the $\kappa_m$ is known to us, and thus only the $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$ remains unknown. Note that, $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$ is a regression function to predict $\ell\{Y , f_m(X)\}$ using $X$, and therefore can be learned by training a regression model on the training samples, where $\ell\{Y_i, f_m(X_i)\}$'s are treated as responses instead of $Y_i$'s. Let us denote this estimator by $\widehat \Phi_m(X)$. Now, we can replace $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$ by $\widehat \Phi_m(X)$ within the decomposition in eq. \eqref{eq:reg-decomposition} to obtain a plug-in estimator for $\eta_{\lambda, m} ^\star(X)$, denoted as $\widehat \eta_{\lambda, m}(X)$. Then, our estimated router is simply $\widehat g_\lambda (X) = \argmin_{m} \widehat \eta_{\lambda, m}(X)$. In our whole procedure, we only need to estimate $M$ different regression functions $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$, which is \emph{computationally more efficient} than to learn a router for each value of $\lambda$ on a suitable grid. 


While the procedure is computationally efficient, \emph{does it also lead to statistically efficient estimates of the oracle routers?} To answer this question, we perform a minimax investigation on the excess risk (defined in eq. \eqref{eq:excess-risk}), and show that for a suitable choice of $\widehat \Phi_m$ (\cf\ Remark \ref{cor:efficient-routers}) our plug-in routers achieve the minimax optimal rate of convergence. Broadly speaking, the steps in our minimax investigation are as follows: 
\begin{itemize}
    \item In Theorem \ref{thm:lower-bound} we consider a setting similar to non-parametric classification problems considered in \citet{audibert2007Fast} and establish a lower bound on the minimax rate of convergence for the excess risk.
    \item  In Theorem \ref{thm:upper-bound} we establish a matching upper-bound rate of convergence of excess risk when $\widehat \Phi_m(X)$ has a ``suitable'' rate of convergence (\cf\ Corollary \ref{cor:efficient-routers}). 
    \item In Section \ref{sec:reg-fn-estimate} we propose an estimate $\widehat \Phi_m(X)$ that achieves our desired rate of convergence. 
\end{itemize}
Finally, we utilize our approach on two benchmark datasets, namely \texttt{RouterBench}\footnote{https://huggingface.co/datasets/withmartian/routerbench}\citep{hu2024routerbench} and \openllm\
\footnote{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard} \citep{open-llm-leaderboard-v2}
to estimate the oracle routers and the Pareto frontier of error and cost trade-off. 
% Both of the benchmark datasets contain a diverse set of tasks, such as reasoning, math, coding, etc, which necessitates the routing rather than fine-tuning.  
As a sneak peek at our findings, in \routerbench\ through routing, we can achieve performance similar to GPT4 at half the cost, whereas $95\%$ of performance at less than $20\%$ of the cost. 


On a more technical side, our routing task, at its heart, is a multi-objective classification problem. Within this context, our contributions are the following: 
\begin{itemize}
    \item In the context of our routing application, we were required to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$. 
    \item  We establish minimax rates for multi-objective classification problems: in Section \ref{sec:lower-bound} we work with two objectives, namely performance and cost, which is relevant to our routing application, and in Section \ref{sec:general-multi-obj} we further extend the setting to a general instance of multiple objectives. In both cases, we establish that simple plug-in routers are minimax rate optimal for the entire collection of oracle routers. To the best of our knowledge, our paper is the first to analyze minimax optimality on the entire collection of oracle classifiers in classification problems with multiple objectives. 
    \item  For a multi-objective classification problem, we provide a computationally and statistically efficient approach to estimate all the oracle classifiers.  
\end{itemize}



% \SM{(1) talk about the extension to multi class classification, (2) introduction of a new notion of margin and explain how it relates to margin in binary case, (3) }

% We quantify the capability of a model in two front:


% % This problem is called the \emph{routing} problem. \SM{introduce some the routing and related linerature here.}
% % To formally introduce the routing problem, assume that we have access to $M$ pre-trained prediction models $f_1, \dots, f_M: \cX \to \cY$ and given a new $X\in \cX$ we need to pick the ``best capable'' one for our prediction task. We quantify the capability of a model in two front:




% \begin{itemize}
%     \item {\bf Accuracy:} for the response $Y$ and it's prediction $f_m(X)$ we consider a prediction loss function: $\ell\{Y, f_m(X)\} \in \reals$.        
%     \item {\bf Cost:} along with a pre-trained model $f_m$, we also receive a $\kappa_m: \cX \to \reals$ that, given an input $X$, quantifies the cost of obtaining the prediction $f_m(X)$ as $\kappa_m(X)$. \SM{say something a bit more about both loss and the cost.}
% \end{itemize} 



% Now, we're presented with a muli-objective problem, and for a given $\lambda > 0$ it is often standard to choose a combination  $\eta_{\lambda, m}(X, Y) \triangleq  \lambda \ell\{Y, f_m(X)\} + (1 - \lambda) \kappa_m(X)$. To this end, we want to learn a router $g: \cX \to \{1, \dots, L\}$ that minimizes our average cost-adjusted loss:
% \begin{equation}
%   \textstyle  \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = l\} \eta_{\lambda, m}(X, Y) \big]\,.
% \end{equation}
% We provide the oracle router in the following  lemma: 







% \paragraph{The problem: learning the Pareto routers.} Of course, the oracle router depends on $\lambda > 0$, and given a $\lambda$ we can estimate the oracle router model as $\widehat g_\lambda$ using standard statistical learning techniques. But, say, we want to provide users with a class $\widehat \cG = \{\widehat g_\lambda: 0\le  \lambda \le 1\}$ that efficiently estimates the class $\cG^\star = \{g_\lambda^\star: 0\le \lambda\le 1 \}$ of oracle routers, which we call ``Pareto routers''. Together with them, we want to provide estimates of expected performance and cost in $P$, \ie\ an estimate of the Parato metric curve
% \begin{equation}
%     \cM^\star = \big\{ \big(\cL_P(g_\lambda^\star, 1), \cL_P(g_\lambda^\star, 0)\big): 0\le \lambda \le 1 \big\}
% \end{equation}
% so that the said users can make their own informed choice of $\lambda$ by looking at the performance vs. cost ``trade-off''. 

% \paragraph{Efficient learning of the Pareto routers.}
% How do we learn this $\widehat \cG$? Do we train separate routers for separate values of $\lambda$, which might be resource intensive? Through our minimax analysis, we show that $\cG^\star$ can be learned efficiently using a simple two-step procedure:


% \begin{algorithm}
%     \begin{algorithmic}[1]
% \Require data $\cD$
% \State Learn an ``efficient'' predictor $\widehat \Phi: \cX \to \reals^L$ for $\Phi^\star: \cX \to \reals^L$ where the $l$-th co-ordinate of $\Phi^\star(X)$ is $\Phi^\star_l(X) = \Ex_P[\ell\{Y, f_m(X)\}\mid X ]$. The term ``efficient'' is made more precise later in Section \ref{sec:upper-bound}. 
% \State For $0 \le \lambda \le 1$ estimate $\widehat g_\lambda$ as \begin{equation}\label{eq:eff-estimate-router}
%         \widehat g_\lambda(X) = \argmin_l \{\lambda \widehat \Phi(X) + (1 - \lambda) \kappa_m(X)\}\,. 
%     \end{equation}
% \end{algorithmic}
% \caption{Learning of Pareto routers}
% \label{alg:pareto-routers}
% \end{algorithm}


% This two-step procedure greatly reduces our computation burden for the learning of $\cG^\star$ since we no longer need to train $\widehat g_\lambda$ for individual $\lambda$'s, which can be computationally intensive. Instead, we only need to learn $\Phi^\star$ once and easily obtain the class $\widehat\cG$ from \eqref{eq:eff-estimate-router}. 

% \paragraph{Minimax investigation of Pareto routers.} To argue that our two-step procedure in Algorithm \ref{alg:pareto-routers} is minimax rate optimal,  we establish the following: For any $0\le \lambda\le 1$
% \begin{itemize}
%     \item Within a standard setting that is often considered in investigating minimax rates for non-parametric classification problems \citep{audibert2007Fast}, we establish a lower bound for the minimax rate of convergence for the excess risk of a router (\cf\ Theorem \ref{th:lower-bound} ). 
%     \item In Section \ref{sec:upper-bound} we show that as long as $\widehat \Phi$ satisfies the concentration bound in \eqref{} the excess risk of the $\widehat g_\lambda$ defined in \eqref{eq:eff-estimate-router} achieves the same minimax rate of convergence, which establishes that $\widehat g_\lambda$ is minimax rate-optimal.  
% \end{itemize}



% \paragraph{Application to the \texttt{RouterBench} dataset.} \texttt{RouterBench}\footnote{https://huggingface.co/datasets/withmartian/routerbench}\citep{hu2024routerbench} is a Q\&A dataset comprising of over $\sim 30000$ prompts and the responses from 11 different LLMs, along their associated costs and a performance scores. We use our proposed algorithm \ref{alg:pareto-routers} to learn the Pareto routers, where the performance score predictor $\widehat \Phi$ is trained on a training split of the dataset  and estimate the Parato metric curve on the remaining test split. \SM{Say somethings about the findings in a couple of lines. Keep it short.}


% \SM{Possible generalization to multiple metrics. This can go into conclusion section.}



\paragraph{Organization of the paper.} We end our introductory section with a short description of the organization of our paper. In Section \ref{sec:lower-bound} we establish information-theoretic lower bounds on the excess risk in estimating oracle routers and develop a computationally efficient algorithm to estimate them that achieves the same rates in their upper bound. In Section \ref{sec:routing-application} we use this algorithm for routing in two benchmark datasets. In Section \ref{sec:general-multi-obj} we extend the routing problem to general metrics and discuss an efficient estimation algorithm and establish minimax optimal rate of convergence for the oracle routers, which is in the similar vain in Section \ref{sec:lower-bound}. We end our paper with a discussion in Section \ref{sec:discussion}. 


\subsection{Related literature}


\paragraph{Performance vs cost trade-off in LLM predcitions.} Several recent studies have explored optimizing the cost and performance trade-offs in the implementation of
large-language models (LLMs). LLM-BLENDER \citep{jiang2023llm} ensembles outcomes from
multiple LLMs to select the best response. Frugal-ML, Frugal-GPT \citep{chen2020frugalml,chen2023frugalgpt} and FrugalFoE \cite{wang2023fusing} employ an LLM cascade to sequentially query LLMs until a reliable response is found. AutoMix \citep{madaan2023automix} relies on a smaller model to self-verify its response before potentially considering a larger model. While these approaches rely
on multiple LLM queries, our approach routes each query to a single LLM, an approach also considered in \citet{hu2024routerbench}. We complement these works by providing a statistically principled approach to learning this performance vs. cost trade-off. 

\paragraph{Ensemble learning.} The routing problem is closely related to ensemble learning that combines multiple models to obtain better performance. Classical ensemble methods include bagging (bootstrap aggregating), boosting, and
stacking (model blending) \citep{breiman1996bagging,breiman1996stacked,freund1996experiments,friedman2001greedy,wolpert1992stacked}. Most of these works implicitly assume that the models in the ensemble have \emph{similar expertise}, and
thus it is beneficial to aggregate their predictions, whereas in our case, models may have \emph{complementary expertise}, and averaging their outputs might be detrimental because most of them may not be suitable for an input. Therefore, we choose to predict using the model with the best outcome, rather than aggregating them. 

\paragraph{Minimax study in non-parametric classification.} One of the earliest work on the minimax rate of convergence in non-parametric classification settings is by \citet{audibert2007Fast}. These techniques were later adopted for investigating the ability of transfer learning under a distribution shift; some prominent examples being \citep{kpotufe2018Marginal,cai2019Transfer,maity2020Minimax}. All of these works consider binary classification with $0/1$ loss. In comparison, our minimax investigation differs in two fronts: we extend the settings to classification with more than two classes and general cost functions. 
% To quantify the difficulty of classification in our extended framework through a margin condition, as done in \citet{audibert2007Fast} for binary classification with $0/1$ loss, we needed to extend the notion of margin appropriately (\cf\ eq. 
 \eqref{eq:margin}). 

\paragraph{Multiobjective learning}

==> sections/intro_new.tex <==
\section{Introduction}
\label{sec:intro}


%The rapid advancement of large-language models (LLMs) is remarkable, as they 

% Large language models (LLMs) can now routinely tackle a variety of tasks in academic, industrial, and everyday contexts \citep{minaee2024large}. This continued success has inspired the rapid introduction of new LLMs for both general and specialized purposes. Although this abundance has the potential to provide practitioners with flexibility, the sheer number of options often makes it challenging to select a suitable model given budget and performance needs. In particular, given a question of interest, how should one know which LLM to send it to? In a perfect world, one might simply opt to use the most powerful model, but for many, this will quickly lead to prohibitive financial and computational costs. 


Large language models (LLMs) have demonstrated the capability to effectively address a diverse array of tasks across academic, industrial, and everyday settings \citep{minaee2024large}. This continued success has catalyzed the rapid development of new LLMs tailored for both general and specialized applications \citep{myrzakhan2024open}. While %the proliferation of these models
this offers practitioners increased flexibility, the vast number of available options may pose a daunting challenge in their real-world deployment. Particularly, determining the optimal LLM for a given query remains a significant challenge. In a perfect world, all queries can be routed to the most powerful model, but for many, this may quickly become prohibitively expensive.

\begin{figure}[h]
    \centering
        \includegraphics[width=0.4\textwidth]{plots/fmselect_gpt4o_comparison.pdf} 
        %\caption{Test 1}
        %\label{fig:RouterBench}
    %\hfill
    %\begin{minipage}{0.49\textwidth}
      % \includegraphics[width=\textwidth]{plots/router-vs-gpt4.pdf}
      %  \caption{Test 2}
     %   \label{fig:router-vs-gpt4}
    %\end{minipage}
\caption{Percent of GPT-4o performance achieved by CARROT across dataset at various discounted costs, where the blue dotted line indicates similar ($100\%$) performance to GPT-4o.}
\label{fig:IBMMix-spider}
\end{figure}

%Although some proprietary models, like GPT-4, offer outstanding performance, they often come with significant costs due to high API prices.

%A common approach to address this issue is to optimize LLMs to maintain a desirable performance at a uniformly cheaper cost. To do so, researchers have tried chain-of-thought reasoning \citep{wei2022chain,wu2023chain} to improve performance (at a relatively fixed cost), and weight quantization \citep{lin2024awq,zhao2024atom} or model distillation \citep{hsieh2023distilling}  to reduce model size. These techniques can be effective in reducing the serving cost of a single model but have not uniformly addressed the cost of deployment that LLMs often incur. %given the rapid rise in the number of available LLMs, these techniques are certainly not scalable in the long run. 

A common approach to address this issue %Another popular approach 
is \emph{routing} \citep{shnitzer2023large, hu2024routerbench, ong2024routellmlearningroutellms, notdiamond2023rorf,akota2024}. There are two paradigms of routing; \emph{non-predictive} routers repeatedly call LLMs and evaluate the responses to select the best one for a given query. Examples include Fusion of Experts (FoE) \citep{wang2023fusing}, FrugalGPT \citep{chen2024frugalgptTMLR}, and techniques that cascade answers from weak to strong LLMs \citep{yue2024largelanguagemodelcascades}. The obvious disadvantage non-predictive routing is the required inference of many LLMS for all queries, even those that are not suitable for the task at hand. As a workaround, researchers have also considered \emph{predictive routers}, which take LLM queries as inputs and output guesses at the most appropriate LLM.  %Routing has several advantages over optimizing a single LLM. First, as we shall see later, it treats each LLM as an input-output black-box, avoiding the need to delve into intricate infrastructure details, thus making it both flexible and scalable. Secondly, routing can allow practitioners to ``customize" the criteria by which LLM's are selected. 
A key limitation of the prior literature on predictive routing is \emph{the avoidance of the cost prediction problem}. In \citet{shnitzer2023large} only performance is considered. The methods RouteLLM %their router cannot handle the inclusion of cost into the model selection desiderata. 
\citep{ong2024routellmlearningroutellms} RoRF \citep{notdiamond2023rorf} incorporates model cost by creating binary routers that select between a large costly model and a cheap small model. While this does incorporate cost, we shall see that the reduced flexibility of binary routing leads to performance degradation in practice. Finally, in \citet{akota2024} cost prediction is considered, but the authors assume that cost may be inferred from available API pricing; this does not hold if model responses are open-ended, and thus may vary in length. 


%\my{discuss limitations of key methods: they don't explicitly consider cost. My paper just tries to choose best model; RouteLLM implicitly considers cost by routing between small and big models, but this limits its ability to benefit from diverse strengths of many available closed- and open-source models.}
%while a single LLM, especially the small ones, may struggle to perform well on an expanding landscape of LLM tasks, by escaping the reliance on a single LLM, routing allows us to benefit from the diversity of LLMs. 
% \SM{mention somewhere that the collection of LLMs can be easily extended on the fly.}

% Let us understand the task of routing from a statistician's point of view. Given spaces of inputs $\cX$ and outputs $\cY$ we have a collection of input-output black-box models, denoted as $f_1, \dots, f_M: \cX \to \cY$.


To address these shortcomings, we develop CARROT: a Cost AwaRe Rate Optimal rouTer and collect the Smart Price-aware Routing (\newdata) dataset. \newdata\ is representative of both performance and cost of state-of-the-art LLMs across varying practical use-cases. Additionally, we use it to train the final version of CARROT. CARROT is designed to function as an estimate of \emph{the oracle router}. As a concrete example of the oracle router, consider model performance and inference cost as the metrics of interest. First, based on their needs, a practitioner selects a convex combination of performance and cost as the model metric. Next, the oracle router takes in a query and produces the LLM that minimizes this specific model metric. To do this selection, the oracle router needs to perfectly predict the metrics of interest (cost, performance) for each model given any query. Inspired by this, CARROT %\my{before talking about plug-in, should we explain what an "oracle" router would look like. Then its limitations motivating the plug-in approach} This leads us to 
utilizes a simple two-stage approach. We first attain an estimator for each of the metrics (\eg\ cost and performance) for each model given a query, then we plug in these estimators to the formed risk function and select a model that minimizes the appropriate convex combination of the estimated metrics. Although CARROT utilizes a simple approach, it has three distinct advantages.

 % \colorbox{red!5!white}
% {\parbox{\dimexpr\linewidth-2\fboxsep}{%
 % \begin{itemize}
  % \item {\bf Computational efficiency.} For any collection of models and any collection of metrics CARROT can estimate the oracle router for any convex combination of the metrics with only one stage of model training.
   %\item {\bf High-quality data} To obtain a router that can be subsequently used in practice, we collect a new routing dataset representative of both performance and cost of state-of-the-art LLMs and varying practical use-cases. 
   % verify the efficacy of CARROT on a new routing dataset  The final version of CARROT is trained on \newdata\, a new, high-quality, routing dataset we develop.
  % \item {\bf Statistical efficiency.} An information-theoretic minimax investigation reveals that CARROT is a statistically efficient estimator for the oracle router in terms of sample complexity.
 % \end{itemize}
 % }}

\paragraph{Computational efficiency:} A practitioner may be interested in several possible convex combinations to understand the trade-offs across various metrics. In that case, learning a router per combination may not be practical. Our approach allows re-use of a plug-in estimate of the metrics for each combination, easing computational concerns. Furthermore, the metrics of interest may vary from practitioner to practitioner. CARROT allows the flexible addition of any metrics; one only needs to acquire estimators for them. As a demonstration of CARROT's efficiency, we utilize it to estimate the Pareto frontier of performance and cost trade-off on 
% two classic benchmark datasets, 
{RouterBench}\footnote{\url{https://huggingface.co/datasets/withmartian/routerbench}}\citep{hu2024routerbench}, open-LLM-leaderboard-v2\
\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard}} \citep{open-llm-leaderboard-v2}, and our new \newdata\ dataset.

\paragraph{New dataset for routing:} \newdata\ covers 13 state-of-the-art language models (e.g. Llama-3-herd \citep{grattafiori2024llama3herdmodels}, GPT-4o \citep{openai2024gpt4}, \etc ) and approximately $45$k prompts from 6 benchmarks covering RAG, science, reasoning, and GPT-4 generated user queries. For all models, we use zero-shot prompting and corresponding chat templates to represent practical use cases and collect input and output token counts to allow flexibility when studying cost-performance trade-offs. We defer further details about \newdata\ and its advantages over other routing datasets to Section \ref{sec:datasets} and Appendix \ref{sec:append:sprout}.

% Furthermore, to ensure that all \newdata\ queries represent real-world use cases, zero-shot prompting is used along with an evaluation system based on MixEval \citep{ni2024mixeval}. We defer further details about \newdata\ and its advantages over other routing datasets to Section \ref{sec:datasets} and Appendix \ref{sec:append:sprout}.

As a sneak peek, in Figure \ref{fig:IBMMix-spider}, we present the ratio of CARROT's performance to GPT-4o's \citep{openai2024gpt4} on several key benchmarks across diverse use cases represented in \newdata. At $30 \%$ of the cost, CARROT matches or exceeds the performance of GPT-4o on each benchmark. Both \newdata\ and the corresponding CARROT router will be publicly released.

% Of course, any router is only as good as the data that it is trained on. To ensure that CARROT is ready to accurately route a diverse set of queries to a state-of-the-art set of LLMs, we also develop (and train on) the Scalable Price-aware Routing (\newdata) dataset. \newdata\
 % covers 13 state-of-the-art language models (e.g. Llama-3-herd \citep{grattafiori2024llama3herdmodels}, GPT-4o \citep{openai2024gpt4}, \etc ) and approximately $45$k prompts from 6 benchmarks covering RAG, science, reasoning, and GPT-4 generated user queries. Furthermore, to ensure that all \newdata\ queries represent real-world use cases, zero-shot prompting is used along with an evaluation system based on MixEval \citep{ni2024mixeval}. We defer further details about \newdata\ and its advantages over other routing datasets to Section \ref{sec:datasets} and Appendix \ref{sec:append:sprout}.
 
%\my{discuss our new dataset - I'll write it}

% Collecting adequate data for training a router has its own challenges; one needs to collect answers along with their evaluations on performance and costs for each combination of LLMs and queries, which could make the whole data generating process expensive. Thus, statistical efficiency is also an important consideration for any routing procedure.

% Collecting adequate data for training router has its own challenge; inference for each query needs to be answers along with their evaluations on performances and costs need to be collected for each combination of LLMs and queries, which could make the data generating process expensive. Thus, statistical efficiency is also an important consideration for any routing procedure.

%Given that training data is not limitless \my{can mention that specifically for routing it is expensive to collect - gotta run all LLMs and evaluate everything - it could be made clear from previous paragraph too}, statistical efficiency is also an important consideration for any routing procedure. 

% \vspace{-0.2cm}

\paragraph{Statistical efficiency} Collecting adequate data to train a router is quite expensive as we need to generate and evaluate with every LLM for every query.
% challenging; for each LLM and every query one must collect a response \emph{and} an evaluation from a judge of that response. By necessity, this collection process must include inference from closed source models such as Claude 3.5 \citep{TheC3} and GPT-4o.  This makes the routing data gathering process expensive; for example, gathering \newdata\ for one model can cost hundreds of dollars.  %answers along with their evaluations on performance and costs for each combination of LLMs and queries, which makes whole data generating process expensive. 
% Clearly, routing data is not limitless, so
Thus, statistical efficiency is an important consideration for any routing procedure. To investigate statistical efficiency, we connect the routing problem to multi-objective classification with a wide class of possible loss functions (this depends on the convex combination of model metrics on hand). Here, identities of the possible models act as the label space of the multi-class classification problem. Given this, one contribution of our work is to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us to introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$.  Additionally, our work analyzes minimax optimality on the entire collection of oracle classifiers in classification problems with all possible trade-offs between multiple objectives, which, to the best of our knowledge, is a novel contribution.

%Our theoretical contributions allow us to establish that simple plug-in routers are minimax rate optimal. This, along with our empirical demonstrations, shows that CARROT is both computationally and statistically efficient. %approach to estimate the entire collection of oracle classifiers.
 
%a model like GPT-4 \citep{openai2024gpt4} may offer outstanding performance, but model calls often come with significant costs due to high API prices. On the other hand, a practitioner could opt to query an open-source LLM (e.g. a model in the Llama family \citep{grattafiori2024llama3herdmodels}) which comes with reduced pricing but at a possibly reduced performance.
%if for any query and any LLM (e.g GPT-4 \citep{openai2024gpt4} or Llama3 \citep{grattafiori2024llama3herdmodels}) the practitioner knew the associated cost and performance, they could always select the cheapest model that provides a satisfactory response.

%At this point, let us take a step back and provide more context to the ``best-suited'' models. A practitioner may be interested in various (conflicting) metrics such as various notions of accuracy, cost, and run time. As a concrete example, consider model performance and inference cost; a model like GPT-4 \citep{openai2024gpt4} may offer outstanding performance, but model calls often come with significant costs due to high API prices. On the other hand, a practitioner could opt to query an open-source LLM (e.g. a model in the Llama family \citep{grattafiori2024llama3herdmodels}) which comes with reduced pricing but at a possibly reduced performance. 
%This hints at a possible trade-off between various metrics of interest. To make it general and satisfy a broad spectrum of users' needs, this paper will develop routers for arbitrary trade-offs.
%\my{small models still cost money or have to self-serve; also cite papers for models} 
%Next, having decided on such a trade-off, the goal of the router is to predict the identity of the LLM that is expected to have the best possible trade-off value.

%This is a standard multi-class classification problem: one can form a trade-off risk function by combining the desired metrics with a suitable convex combination; then the goal is to take a query and pick the model that minimizes the risk. Here, identities of the possible models act as the label space of the multi-class classification problem. In an ideal world, we could produce an oracle router that always picks the model with minimum. To do so, one would need to perfectly predict the metrics of interest (cost, performance) for each model for any query. Inspired by this, we %\my{before talking about plug-in, should we explain what an "oracle" router would look like. Then its limitations motivating the plug-in approach} This leads us to 
%propose a simple two stage router in Section \ref{sec:setup}. We first attain an estimator for each of the metrics (e.g cost or accuracy) for each model given query $X$, then we plug in these estimators to the formed risk function and select a model that minimizes the appropriate convex combination of the estimated metrics.

%Given this, a predictive router is essentially a classifier that predicts the index of the best model, and thus can be efficiently learned by minimizing a standard classification loss using the pairs of query and convex combination of metrics. 

%Although this is a simple approach, it has a couple of distinct advantages. First, a practitioner may be interested in several possible convex combinations to understand the trade-offs across various metrics. In that case, learning a router per combination through direct optimization may not be practical. Our approach allows re-use of a plug-in estimate of the metrics for each model, easing computational concerns. Furthermore, the metrics of interest may vary from practitioner to practitioner. Our approach allows the flexible addition of any metrics; one only needs to acquire estimators for them.



%In short, our plug-in approach  has three advantages: 
%\begin{activitybox}

 %\paragraph{Simplicity.} It is simple, easily interpretable, and adapts to a broad spectrum of users' preferred trade-off, even when a new model or metric is introduced to the problem.

 %\paragraph{Computational efficiency.} It provides a computationally scalable approach to estimate routers for an arbitrary combination of metrics.


 %\paragraph{Statistical efficiency.} An information-theoretic minimax investigation reveals that the plug-in approach is statistically efficient in terms of sample complexity.

%\end{activitybox}



% \colorbox{red!5!white}{\parbox{\dimexpr\linewidth-2\fboxsep}{%
% \begin{itemize}
%  \item {\bf Computational efficiency.} It provides a computationally scalable approach to estimate routers for all combinations of metrics.
%  \item {\bf Statistical efficiency.} An information-theoretic minimax investigation reveals that the plug-in approach is statistically efficient in terms of sample complexity.
% \end{itemize}
% }}
   
%Empirically, our approach has been compared against several state-of-the-art routers on two benchmark datasets, namely {RouterBench}\footnote{https://huggingface.co/datasets/withmartian/routerbench}\citep{hu2024routerbench} and open-LLM-leaderboard-v2\
%\footnote{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard} \citep{open-llm-leaderboard-v2}
%to estimate the oracle routers and the Pareto frontier of performance and cost trade-off. 
% Both of the benchmark datasets contain a diverse set of tasks, such as reasoning, math, coding, etc, which necessitates the routing rather than fine-tuning.  
%As a sneak peek, in routerbench through our routing approach, we can achieve performance similar to GPT4 at half the cost, and $95\%$ of performance at less than $20\%$ of the cost. 

%On the theoretical side, the routing problem, at its heart, is a multi-objective classification problem with a wide class of possible loss functions (this depends on the convex combination of model metrics on hand). Given this, one contribution of our work is to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$.  Additionally, our work analyzes minimax optimality on the entire collection of oracle classifiers in classification problems with all possible trade-offs between multiple objectives, which, to the best of our knowledge, is a novel contribution.
%\my{we haven't established the connection between routing and classification yet - maybe do it earlier when explaining oracle router and plug-in router}

% Our theoretical contributions allow us to establish that simple plug-in routers are minimax rate optimal. This, along with our empirical demonstrations, shows that CARROTS is both computationally and statistically efficient. %approach to estimate the entire collection of oracle classifiers.

%\begin{itemize}
    %\item In the context of our routing application, we were required to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$. 
    %\item  We establish minimax optimal rates for multi-objective classification problems, which, to the best of our knowledge, is the first to analyze minimax optimality on the entire collection of oracle classifiers in classification problems with multiple objectives. 
    %\item  For a multi-objective classification problem, we establish that simple plug-in routers are minimax rate optimal, which provides a computationally and statistically efficient approach to estimate the entire collection of oracle classifiers.  
%\end{itemize}


\subsection{Related literature}


\paragraph{Performance vs cost trade-off in LLM predictions.} Several recent studies have explored optimizing the cost and performance trade-offs in the implementation of
large-language models (LLMs). LLM-BLENDER \citep{jiang2023llm} ensembles outcomes from
multiple LLMs to select the best response. Frugal-ML, Frugal-GPT \citep{chen2020frugalml,chen2024frugalgptTMLR} and FrugalFoE \cite{wang2023fusing} employ an LLM cascade to sequentially query LLMs until a reliable response is found. AutoMix \citep{madaan2023automix} relies on a smaller model to self-verify its response before potentially considering a larger model. While these approaches rely
on multiple LLM queries, our approach routes each query to a single LLM, an approach also considered in \citet{hu2024routerbench}. We complement these works by providing a statistically principled approach to learning this performance vs. cost trade-off. 

\paragraph{Ensemble learning.} The routing problem is closely related to ensemble learning that combines multiple models to obtain better performance. Classical ensemble methods include bagging (bootstrap aggregating), boosting, and
stacking (model blending) \citep{breiman1996bagging,breiman1996stacked,freund1996experiments,friedman2001greedy,wolpert1992stacked}. Most of these works implicitly assume that the models in the ensemble have \emph{similar expertise}, and
thus it is beneficial to aggregate their predictions, whereas in our case, models may have \emph{complementary expertise}, and averaging their outputs might be detrimental because most of them may not be suitable for an input. Therefore, we choose to predict using the model with the best outcome, rather than aggregating them. 

\paragraph{Minimax studies in non-parametric classification.} One of the earliest works on the minimax rate of convergence in non-parametric classification is \citet{audibert2007Fast}. These techniques were later adopted for investigating the ability of transfer learning under a distribution shift
% ; some prominent examples being
\citep{kpotufe2018Marginal,cai2019Transfer,maity2022minimax}. All of these works consider binary classification with $0/1$ loss. In comparison, our minimax investigation differs on two fronts: we extend the settings to classification with more than two classes and general cost functions. 
% To quantify the difficulty of classification in our extended framework through a margin condition, as done in \citet{audibert2007Fast} for binary classification with $0/1$ loss, we needed to extend the notion of margin appropriately (\cf\ eq. 
 % \eqref{eq:margin}). 

% \paragraph{Multiobjective learning}

\subsection{Notation and preliminaries}

To begin, let us introduce our notation. We have $M$ pre-trained LLMs indexed as $m \in [M] = \{1, \dots, M\}$ and $K$ metrics indexed as $k\in [K] = \{1, \dots, K\}$. %Throughout our paper, we index the models as $m \in [M]$ and the metrics as $k \in [K]$. 
We denote a generic input or query as $X\in \cX$, where $\cX$ is the space of inputs.  Thus, for any input $X$, the metrics of interest are stored in a $M\times K$ matrix. We denote this matrix as $Y \in \reals^{M \times K}$, whose $(m, k)$-th entry $[Y]_{m, k}$ is the metric value for obtaining a prediction from the $m$-th model evaluated with respect to $k$-th metric.  For all metrics, we assume that a lower value is preferred. With this convention, we shall also refer to them as risks. For a probability distribution $P$ in the sample space $\cX \times \reals^{M\times K}$ we assume that the training dataset $\cD= \{(X_i, Y_i)\}_{i = 1}^n$ is an $\iid$ sample from $P$. 

 For the probability distribution $P $ defined on the space $\cX \times \reals^{M \times K}$, we denote the marginal distribution of $X$ by $P_X$. Let us denote $\supp(\cdot)$ as the support of a probability distribution. Within the space $\reals^d$, we denote $\Lambda_d$ as the Lebesgue measure, $\|\cdot\|_2$ and $\|\cdot\|_\infty$ as the $\ell_2$ and $\ell_\infty$-norms, and $\cB(x, r, \ell_2)$ and $\cB(x, r, \ell_\infty)$ as closed balls of radius $r$ and centered at $x$ with respect to the $\ell_2$ and $\ell_\infty$-norms. 

==> sections/lower-bound.tex <==
\section{Statistical efficiency of CARROT} 
\label{sec:lower-bound}

In this section we establish that, under certain conditions, the plug-in approach to routing is minimax optimal. To show this, we follow two steps:
\begin{itemize}
    \item First we establish an information theoretic lower bound on the sample complexity for learning the oracle routers (\cf\ Theorem \ref{thm:lower-bound}). 
    \item Next, establish an upper bound for the minimax risk of plug-in routers (\cf\ Theorem \ref{thm:upper-bound}). We show that under sufficient conditions on the estimates of $\Ex[Y\mid X]$ the sample complexity in the upper bound matches the lower bound. Together, they imply the statistical efficiency of the plug-in approach.  
    % We also suggest an estimate for $\Ex[Y\mid X]$ that meets the needed conditions for CARROT to be rate optimal.  
\end{itemize} 


%For our minimax analysis we begin with some notation. For the probability distribution $P $ defined on the space $\cX \times \reals^{M \times K}$, we denote the marginal distribution of $X$ by $P_X$. Let us denote $\supp(\cdot)$ as the support of a probability distribution. Within the space $\reals^d$, we denote $\Lambda_d$ as the Lebesgue measure, $\|\cdot\|_2$ and $\|\cdot\|_\infty$ as the $\ell_2$ and $\ell_\infty$-norms, and $\cB(x, r, \ell_2)$ and $\cB(x, r, \ell_\infty)$ as closed balls of radius $r$ and centered at $x$ with respect to the $\ell_2$ and $\ell_\infty$-norms. 

% We denote $\Ex_P[\ell \{ Y, f_m(X)\}\mid X]$ as $\Phi^\star_m(X)$. Then, following eq. \eqref{eq:reg-decomposition} the regression function $\eta_{\lambda, m}^\star(X) = \Ex_P[\eta_\lambda(X, Y)]$ has the decomposition $\eta_{\lambda, m}^\star(X) = \lambda \Phi^\star_m(X) + (1 - \lambda) \kappa_m(X)$. In the following lemma, we provide a formulation of oracle routers using this decomposition, which will be useful for developing their computationally efficient estimates. 
% \begin{lemma} \label{lemma:oracle-router}
%     For any $0 \le \lambda \le 1$  the oracle router $g_\lambda^\star$ that minimizes the loss $\cL_P(g, \lambda)$ is 
%     \begin{equation} \label{eq:oracle-router-2}
%         \textstyle g_\lambda^\star(X) = \argmin_m ~ \eta_{\lambda, m} ^\star(X) = \argmin_m ~ \{ \lambda \Phi^\star_m(X) + (1 - \lambda) \kappa_m(X)\}\,.
%     \end{equation}
% \end{lemma}

We begin with a notational convention for $g_\mu^\star(X)$. If the minimum is attained at multiple $m$'s, we consider $g_\mu^\star(X)$ as a subset of $[M]$. On the contrary, if the minimum is uniquely attained, then $g_\mu^\star(X)$ refers to both the index $m_X$ where the minimum is attained and the singleton set $\{m_X\} \subset [M]$. The distinction should be clear from the context.

We also generalize slightly to the setting where the last $K_2$ metrics are known functions of $X$, \ie\ for $m \in [M], k \in \{K - K_2 +1 , \dots K\}$ there exist known functions $f_{m, k}: \cX \to \reals$ such that $[Y]_{m, k} = f_{m, k}(X)$. Since $\Ex[[Y]_{m, k}\mid X] = f_{m, k}(X)$ are known for $k \ge K - K_2 +1 $ they don't need to be estimated. 
% We shall see the presence of known metrics has consequences for the sample complexity (\cf\ Remark \ref{remark:difficulty-routing}). We also define $K_1 = K - K_2$ as the number of known metrics.    

\subsection{Technical Assumptions}

%Let us discuss a notational convention for $g_\lambda^\star(X)$. The minimum can be attained at multiple $m$'s. In that case, $g_\lambda^\star(X) \subset [M]$. However, when the minimum is uniquely attained, the $g_\lambda^\star(X)$ refers to both the index $m_X$ where the minimum is attained and the singleton set $\{m_X\} \subset [M]$. The distinctions should be clear from the contexts.


%We also assume that the last $K_2$ many metrics are known functions of $X$, \ie\ for $m \in [M], k \in \{K - K_2 +1 , \dots K\}$ there exist known functions $f_{m, k}: \cX \to \reals$ such that $[Y]_{m, k} = f_{m, k}(X)$. Since $\Ex[[Y]_{m, k}\mid X] = f_{m, k}(X)$ are known for $k \ge K - K_2 +1 $ within the Algorithm \ref{alg:pareto-routers}, they don't need to be estimated. We shall see its consequence in the study sample complexity. Define $K_1 = K - K_2$.    



The technical assumptions of our minimax study are closely related to those in investigations of non-parametric binary classification problems with $0/1$ loss functions, \eg\  \citet{cai2019Transfer,kpotufe2018Marginal,maity2022minimax,audibert2007Fast}. In fact, our setting generalizes the classification settings considered in these papers on multiple fronts: (i) we allow for general loss functions, (ii) we allow for more than two classes, and (iii) we allow for multiple objectives. %So, before we describe the assumptions, 

To clarify this, we discuss how binary classification is a special case of our routing problem. %This connection will be later used for adapting the standard assumptions considered in these papers to our setting. 

\begin{example}[Binary classification with $0/1$-loss] \label{example:binary-classification}
    Consider a binary classification setting with $0/1$-loss: we have the pairs $(X, Z) \in \cX \times \{0, 1\}$ and we want to learn a classifier $h: \cX \to\{0, 1\} $ to predict $Z$ using $X$. This is a special case of our setting with $M = 2$ and $K= 1$, where for $m \in \{0, 1\}$ the $[Y]_{m, 1} = \bbI\{Z \neq m\}$. Then the risk for the classifier $h$, which can also be thought of as a router, is 
\begin{align*}
\textstyle \cR_P(h) & \textstyle = \Ex\big[\sum_{m \in \{0, 1\}}[Y]_{m, 1} \bbI\{h(X) = m\} \big]\\ 
& = \Ex\big[ \bbI\{h(X) \neq Z\} \big]\,,
\end{align*} the standard misclassification risk for binary classification. 
\end{example}

% \SM{Mention that for $\lambda = 0$ the oracle router is precisely known. Thus, we only focus on the cases of $\lambda > 0$.}

We assume that $\supp(P_X)$ is a compact set in $\reals^d$. This is a standard assumption in minimax investigations for non-parametric classification problems \citep{audibert2007Fast,cai2019Transfer,kpotufe2018Marginal,maity2022minimax}. 
Next,  we place H\"older smoothness conditions on the functions $\Phi_m^\star$. This controls the difficulty of their estimation. For a tuple $s = (s_1 , \dots, s_d) \in (\bN \cup \{0\})^d$ of $d$ non-negative integers  define $|s| = \sum_{j = 1}^d s_j$ and for a function $\phi: \reals^d\to \reals$ and $x = (x_1, \dots, x_d) \in \reals^d$ define the differential operator: 
\begin{equation}
  \textstyle  D_s(\phi, x) = \frac{\partial^{|s|}\phi(x)}{\partial x_1^{s_1} \dots \partial x_d^{s_d}}\,, 
\end{equation} assuming that such a derivative exists. Using this differential operator we now define the H\"older smoothness condition: 

\begin{definition}[H\"older smoothness]
   For $\beta, K_\beta >0$ we say that $\phi:\reals^d \to \reals$ is $(\beta, K_\beta)$-H\"older smooth on a set $ A \subset \reals^d$ if it is $\lfloor \beta \rfloor$-times continuously differentiable on $A$ and for any $x, y \in A $ 
   \begin{equation}
       |\phi(y) - \phi_x ^{(\lfloor \beta \rfloor)}(y)| \le K_\beta \|x - y\|_2^\beta\,,
   \end{equation} where 
$\phi_x ^{(\lfloor \beta \rfloor)}(y) = \sum_{|s| \le \lfloor \beta \rfloor} D_s(\phi, x) \{\prod_{j = 1}^d(y_j - x_j)^{s_j}\} $ is the $\lfloor \beta \rfloor$-order Taylor polynomial approximation of $\phi(y)$ around $x$. 
\end{definition}
With this definition, we assume the following:
\begin{assumption}\label{assmp:smooth}
    For $m \in [M]$ and $k \in [K_1]$ the 
    % functions $\kappa_m$ and 
    $[\Phi(X)]_{m, k}$ is $(\gamma_{k}, K_{\gamma, k})$-H\"older smooth. 
\end{assumption} 
%The H\"older smoothness assumption controls how well a non-parametric function can be estimated \citep{fan1997local}, where higher smoothness parameters lead to a smaller error in estimation. 
This smoothness parameter will appear in the sample complexity of our  plug-in router. Since the $[\Phi(X)]_{m, k}$ are known for $k \ge K_1 + 1$ we do not require any smoothness assumptions on them.

% Note that the assumption implies for any $\lambda\in [0, 1]$ and $m \in [M]$ the $\eta_{\lambda, m}^\star = \lambda \Phi_m^\star + (1 - \lambda) \kappa_m$ are also $(\beta, K_\beta)$-H\"older smooth.
% The smoothness on the $\Phi_m^\star$ functions controls their complexity: the higher smoothness implies a lower complexity and is easier to estimate. \SM{Talk about how different complexity would lead to the rate at lowest smoothness. Argue it through the estimation of the differences. And also talk about how smoothness in $\kappa_m$ is not necessary.}
% Before we move on, we want to make a few remarks about this smoothness assumption. As discussed in Section \ref{sec:setup} the core idea behind our approach is to plug-in an estimate of $[\Phi(X)]_{m, k}$ into the oracle router \eqref{eq:oracle-router-2}
%  \[
%     \textstyle g_\mu^\star(X)  = \argmin_m \big\{ \sum_{k = 1}^K \mu_k [\Phi (X)]_{m, k} \big\} \,.
%     \]
% A similar idea can also be found  in the context of binary classification in non-parametric settings: for $(X, Y) \in \cX \times \{0, 1\}$ drawn from the distribution $P$, they plug-in an estimator of $\eta(X) = P(Y = 1\mid X )$ into the Bayes classifier $f^\star(X) = \bbI\{\eta(X) \ge \nicefrac{1}{2}\}$ to obtain a minimax rate optimal classifier, which they call ``plug-in classifier''. In their context, the smoothness in $\eta$ controls how well it can be estimated from a dataset, which later affects the misclassification error for this plug-in classifier. Drawing a parallel to our context,
% \begin{enumerate}
%     \item Within the regression function $\eta_{\lambda, m}^\star(X) = \lambda \Phi^\star _m(X) + (1 - \lambda) \kappa_m(X)$ the $\kappa_m$ are already known and need not be estimated. Thus, we do not require any smoothness assumption for $\kappa_m$ and only require a smoothness condition for the unknown $\Phi_m^\star$.  
%     \item To make the setting more general, we could assume different smoothness parameters for different $\Phi_m^\star$; \eg\ $\Phi_m^\star$ is $\beta_m$ H\"older smooth, in which case it can be estimated at a minimax optimal $\ell_1$-error rate $\cO_P(n^{-{\beta_m}/{(2\beta_m + d)}})$ \citep{fan1997local}. But then the differences \[
%     \textstyle \eta_{\lambda, m_1}^\star(X) - \eta_{\lambda, m_2}^\star(X) = \lambda \big\{ \Phi^\star _{m_1}(X) -\Phi^\star _{m_2}(X)\big\}  + (1 - \lambda) \big \{ \kappa_{m_1}(X) - \kappa_{m_2}(X)\big \}\,, 
%     \] which are crucial for the prediction of oracle routers, will be estimated at a rate 
%     \[
%     \textstyle \cO_P\big(n^{-\frac{\beta_{m_1}}{2\beta_{m_1} + d}} \vee n^{-\frac{\beta_{m_2}}{2\beta_{m_2} + d}}\big) = \cO_P\big(n^{-\frac{\beta_{m_1} \wedge \beta_{m_2}}{2(\beta_{m_1} \wedge \beta_{m_2}) + d}} \big)\,,
%     \]
%     and in the worst case, at a rate $\cO_P(n^{-{\beta_{\min} }/{(2\beta_{\min}  + d})} )$ with respect to the smallest smoothness parameter $\beta_{\min} = \min_m \beta_m$. Since accurately estimating all of these pairwise differences is important to obtain a prediction similar to that of the oracle routers, the final rate of convergence rate for excess risk will be determined by the smallest smoothness parameter, in which case, the other smoothness parameters become irrelevant. Therefore, for a simpler exposition of the problem setting, we assume that the smoothness parameters of $\Phi_m^\star$ are all identical. 
% \end{enumerate}




Next, we introduce \emph{margin condition}, which quantifies the difficulty in learning the oracle router.  For a given $\mu$ define the margin as the difference between the minimum and second minimum of the risk values: 
{ \begin{equation}\label{eq:margin}
    \begin{aligned}
        & \textstyle \Delta_\mu(x) =  \\
  &  \begin{cases}
       \min\limits_{m \notin g_\mu(x)} \eta_{\mu, m}(x) - \min\limits_m \eta_{\mu, m}(x) & \text{if} ~ g_\mu^\star(x) \neq [M]\\ 
       0 & \text{otherwise}.
       \end{cases} 
    \end{aligned}
\end{equation}}

% At an $x$, the margin is simply the gap between the second-lowest and lowest coordinate values of $\eta_{\lambda, m}$. If all the coordinates are the same, then we set the margin at zero. 
\noindent Our definition of a margin generalizes the usual definition of the margin considered for binary classification with $0/1$ loss in \citet{audibert2007Fast}. Recall the binary classification example in \ref{example:binary-classification}, in which case, 
$[\Phi(X)]_{m , 1} =  P(Z \neq m\mid X) $. Since $K = 1$ we have 
$\eta_{\mu, m}(X) = P(Z \neq m\mid X) $, which further implies $\eta_{\mu, 0}(X) + \eta_{\mu, 1}(X) = 1$.
Thus for binary classification with $0/1$ loss, our definition of margin simplifies to 
\begin{align*}
\textstyle \min\limits_{m \notin g_\mu^\star(x)} \eta_{\mu, m}(x) - \min\limits_m \eta_{\mu, m}(x)\\
=  |\eta_{\mu, 1}(X) - \eta_{\mu, 0}(X)| = 2 |\eta_{\mu, 0}(X) - \nicefrac{1}{2}| \,,
\end{align*}
which is a constant times the margin $  |P(Y = 1\mid X) - \nicefrac{1}{2}| = |\eta_{\mu, 0}(X) - \nicefrac{1}{2}| $ in \citet{audibert2007Fast}. 


% Relating their framework to ours, for them $M = 2$ with the class indices $\{0, 1\}$. Moreover, for $m \in \{0, 1\}$ the loss regression function for classifying a sample $X$ as class $m$ is  $\eta_{\lambda, m}^\star(X) = P(Y \neq m\mid X) $, which satisfies $\eta^\star_{\lambda, 0}(X) + \eta^\star_{\lambda, 1}(X) = 1$. In this case, our definition of margin simplifies to $|\eta_{\lambda, 1}(X) - \eta_{\lambda, 0}(X)| = 2 |\eta_{\lambda, 1}(X) - \nicefrac{1}{2}|$, which is a constant multiplication of their definition of margin $  |P(Y = 1\mid X) - \nicefrac{1}{2}| = |\eta_{\lambda, 1}(X) - \nicefrac{1}{2}| $. 



Clearly, the margin determines the difficulty in learning the oracle router. A query $X$ with a small margin gap is difficult to route, because to have the same prediction as the oracle, \ie\  $\argmin_{m} \hat \eta_{\mu, m}(X) = \argmin_{m} \eta_{\mu, m}^\star(X)$ we need to estimate $ \eta_{\mu, m}^\star(X)$ with high precision. In the following assumption, we control the probability of drawing these ``difficult to route'' queries.

\begin{assumption}[Margin condition]\label{assmp:margin}
    For $\alpha, K_\alpha >0$ and any $t > 0$ the margin $\Delta_{\mu}$ \eqref{eq:margin} satisfies: \begin{equation}
        P_X \big\{0 < \Delta _\mu(X) \le t\big \}  \le K_\alpha t^{\alpha}\,. 
    \end{equation}
\end{assumption}
%From Proposition 3.4 of \cite{audibert2007Fast}, if $\alpha  (1 \wedge \gamma_{k})  \ge d$ for some $k$ then if $\mu = e_k$ for which the $g_\mu^\star$ never changeswe argue that when $\alpha  (1 \wedge \gamma_{k})  \ge d$ for some $k$ then for $\mu = e_k$ for which the $g_\mu^\star$ never changes its decision within the interior of $\supp(P_X)$. 
Following \citet{audibert2007Fast}, we focus on the cases where $\alpha < d$ and for every $k$ the $\alpha \gamma_k < d$. This helps to avoid trivial cases where routing decisions are constant over $P_X$ for some $\mu$.  %These are trivial cases, which we ignore. Thus, throughout our paper, we assume that $\alpha   < d$ and for every $k$ the $\alpha \gamma_k < d$.  
Next, we assume that $P_X$ has a density $p_X$ that satisfies a strong density condition described below.
% We start by formalizing the problem setup. We assume that the covariate space is $\cX$ is a compact set in $\reals^d$. Next, we assume that the density exists for the marginal probability $P_X$ and satisfies a strong density condition, which is formalized below. 
\begin{assumption}[Strong density condition] \label{assmp:strong-density}
Fix constants $c_0, r_0> 0$ and $0 \le \mu_{\min}  \le \mu_{\max} < \infty$. We say $P_X$ satisfies the strong density condition if its support is a compact $(c_0, r_0)$-regular set and it has density $p_X$ which is bounded: $\mu_{\min} \le p_X (x) \le \mu_{\max} $ for all $x$ within $\supp(P_X)$. A set $A \subset \reals^d$ is Lebesgue measurable and %\ie\ for the Lebesgue measure $\Lambda_d$ on $\reals^d$, any Lebesgue measurable set $A \subset \reals^d$ and 
$\text{for any} ~ 0 < r \le r_0, ~  x \in A$ it satisfies
\begin{equation}
    \Lambda_d (A \cap \cB(x, r, \ell_2)) \ge c_0 \Lambda_d(\cB(x, r, \ell_2)). %~ \text{for any} ~ 0 < r \le r_0, ~  x \in A,
\end{equation} %and the density $p_X$ is bounded as: $\mu_{\min} \le p_X (x) \le \mu_{\max} $ for all $x$ within $\supp(P_X)$. 
\end{assumption}
This is another standard assumption required for minimax rate studies in nonparametric classification problems \citep{audibert2007Fast,cai2019Transfer}. All together, we define $\cP(c_0, r_0, \mu_{\min}, \mu_{\max}, \beta_{m ,k}, K_{\beta, m, k}, \alpha, K_\alpha)$, or simply $\cP$, as the class of probabilities $P$ defined on the space $\cX \times \cY$ for which $P_X$  is  compactly supported and satisfies the strong density assumption \ref{assmp:strong-density} with parameters $(c_0, r_0, \mu_{\min}, \mu_{\max})$, and the H\"older smoothness assumption \ref{assmp:smooth} and the $(\alpha, K_\alpha)$-margin condition in Assumption \ref{assmp:margin} hold. We shall establish our minimax rate of convergence within this probability class. 










% In this section we provide a ``mini-max'' investigation on learning of the oracle $g^\star$. For this purpose, assume that 
% \begin{itemize}
    
%     \item {\bf Strong density condition:} $X$ is distributed in the space $[0, 1]^d$ that satisfies the strong density condition \citep{audibert2007Fast}.
%     \item {\bf H\"older smoothness:} The functions $\kappa_\lambda(x, l) \triangleq\ell (f^\star(x), f_l(x)) + \lambda c_l (x)$ are $\alpha$-H\"older smooth. 
% \item {\bf Noise condition:} For $t > 0$ there exists a $\gamma > 0$ such that 
% \[
% \textstyle P_X \big ( 0 <\max_l \big | \kappa_\lambda(x, l) - \min_{l' \neq l} \kappa_\lambda (x, l') \big | \le t \big ) = \cO(t^\gamma)
% \]
% \end{itemize}
% Denote $\cP$ as the class of all probabilities that satisfies the above conditions. 

% \SM{revise the lower bound in light of $\lambda  \ge c n^{\frac{\beta - \nicefrac d\alpha }{2\beta +d }}$ requirement.}
\subsection{The lower bound} 
Rather than the actual risk $\cR_P(\mu, g)$, we establish a lower bound on the excess risk:
\begin{equation}\label{eq:excess-risk}
    \cE_P(\mu, g) = \cR_P(\mu, g) - \cR_P(\mu, g_\mu^\star)\,,
\end{equation} that compares the risk of a proposed router to the oracle one. We denote $\Gamma = \{g: \cX \to [M]\}$ as the class of all routers. For an $n \in \bN$ we refer to the map $A_n: \cZ^n \to \Gamma$, which takes the dataset $\cD_n $ as an input and produces a router $A_n(\cD_n): \cX \to [M]$, as an algorithm. Finally, call the class of all algorithms that operate on $\cD_n$ as $\cA_n$. The following Theorem describes a lower bound on the minimax risk for any such algorithm $A_n$. 
\begin{theorem}\label{thm:lower-bound}
    For an $n \ge 1$  and $A_n \in \cA_n$ define  $\cE_P(\mu, A_n) = \Ex_{\cD_n}\big[\cE_P\big(\mu, A_n(\cD_n)\big)\big]$ as the excess risk of an algorithm $A_n$. There exists a constant $c> 0$ that is independent of both $n$ and $\mu$ such that for any $n\ge 1$ and $\mu\in \Delta^{K-1}$ we have the lower bound
    \begin{equation}\label{eq:lower-bound}
      \textstyle  \min\limits_{A_n \in \cA_n} \max\limits_{P \in \cP} ~~ \cE_P(\mu, A_n) \ge c \big \{\sum_{k = 1}^{K_1} \mu_k n^{- \frac{\gamma_k}{2\gamma_k + d}}\big\}^{1+\alpha} \,.
    \end{equation}
\end{theorem} 
This result is a generalization of that in \citet{audibert2007Fast}, which considers binary classification. 
\begin{remark} \label{remark:minimax-lower-bound}
    Consider the binary classification in Example \ref{example:binary-classification}. Since $K = 1$, the lower bound simplifies to $\cO(n^{-\nicefrac{\gamma_1 (1+ \alpha)}{2\gamma_1 + d}})$,  which matches with the rate in \citet[Theorem 3.5]{audibert2007Fast}. 
    Beyond $0/1$ loss, our lower bound also establishes that the rate remains identical for other classification loss functions as well. 
    
    % The case of $\lambda = 1$ is closely related to the usual classification tasks with a single objective function. In fact, binary classification with $0/1$-loss is a special case. To make this connection clear, consider $M = 2$ and the index set for the classes as $\{0, 1\}$. Moreover, assume that the loss is $0/1$, \ie\ for $m\in \{0, 1\}$ the  $Z_m = \ell\{ Y, f_m(X)\} \in \{0, 1\}$ and $Z_0 + Z_1 = 1$, in which case the loss of a router $g:\cX \to \{0, 1\}$ is 
    % \[
    % \begin{aligned}
    %      \textstyle \ell\{g; X, Y\} & \textstyle= \bbI\{ g(X) = 0\} Z_0 +  \bbI\{ g(X) = 1\} Z_1 \\
    %      & \textstyle= \bbI\{ g(X) = 0\} Z_0 +  \bbI\{ g(X) = 1\} (1 - Z_0) = \bbI \{g(X) \neq Z_0\} \,.
    % \end{aligned}
    % \] Thus, it is not surprising that for $\lambda = 1$ our rate of convergence $\cO(n^{\frac{-\beta(1 + \alpha)}{2\beta +d}})$ for the lower bound is exactly the same as in \citet[Theorem 3.5]{audibert2007Fast}. As such, {we broaden the framework of the minimax lower bound study for non-parametric classification tasks to (1) more than two classes, and (2) general loss functions.} To understand this, consider a classification task with $M$ classes and the loss function of a classifier $g: \cX \to [M]$ is $\ell\{ g; X, Y\} = \sum_{m = 1}^M \bbI \{g(X) = m\} \ell_m(X, Y)$ where $\ell_m(X, Y)$ is the loss incurred when a sample $(X, Y)$ is predicted as the class $m$. In that case, simply letting $\lambda = 1$ and $Z_m = \ell_{m}(X, Y)$ within the lower bound analysis, we obtain a rate of convergence $\cO(n^{\nicefrac{-\beta(1 + \alpha)}{(2\beta +d)}})$. Moreover, the analysis of the upper bound in Section \ref{sec:upper-bound} reveals that this rate is minimax optimal. 
\end{remark}


% \SM{mention how the true difficulty of the problem lies when the $\lambda$ are bounded away from zero because in that case one needs to accurately estimate the $\Phi_m^\star$. At $\lambda \to 0$ the importance is not on the unknown function.}

% \begin{remark}\label{remark:diff-in-lambda-lb} \label{remark:lower-bound-lambda}
%     The lower bound also highlights that ``it is easier to route for a smaller value $\lambda $''. Within the oracle router, we know the $(1 - \lambda) \kappa_m(X)$ part within the function $\eta_{\lambda, m}^\star(X) = \lambda \Phi_m^\star(X) + (1 - \lambda) \kappa_m(X)$. Thus, at an intuitive level, for smaller values of $\lambda$ there is less importance on the unknown $\lambda \Phi_m^\star(X)$ part, and thus the plug-in router in eq. \eqref{eq:plugin-router} can tolerate a larger noise in their estimations. Our lower bound makes this intuition precise: for a smoothness parameter $\beta$ the $\Phi_m^\star$ are estimated at a $\cO_P(n^{-\nicefrac{\beta}{(2\beta+d)}})$-rate, and thus both $\lambda \Phi_m^\star(X)$ and the whole $\eta_{\lambda, m}^\star(X)$ are estimated at a $\cO_P(\lambda n^{-\nicefrac{\beta}{(2\beta+d)}})$-rate. This intuition is more formally exposed in the upper bound study of excess risk in Theorem \ref{thm:upper-bound}, where we precisely quantify the relationship between the error in the estimation of $\Phi_m^\star$ and the convergence rate for excess risk (\cf\ Remark \ref{remark:upper-bound-lambda}).
%     Following this intuition, we can understand that learning a router for a smaller $\lambda$ is easier and for $\lambda = 1$ it is the hardest.
% \end{remark}

% This is the exact same rate of convergence obtained in \citet[Theorem 3.5]{audibert2007Fast}. Intuitively, for a fixed $\lambda$ the task of routing is equivalent to multi-class classification, so, it is not surprising that they have the same rate. 


% \SM{remark about $\lambda$}. 

% \begin{remark}
%     For a fixed $n$ our lower bound analysis in Theorem \ref{thm:lower-bound} is only valid for $\lambda \ge c_1 n^{\frac{\beta - \nicefrac{d}{\alpha}}{2\beta + d}}$. To address this gap, we note: 
%     \begin{itemize}
%         \item Firstly, because we know the cost functions $\kappa_m$, we can precisely find the oracle router $g^\star_{0}(X) = \argmin_m \kappa_m(X)$ at $\lambda = 0$. Furthermore, since we consider $\alpha \beta < d$ the $c_1 n^{\frac{\beta - \nicefrac{d}{\alpha}}{2\beta + d}}$ decreases to zero as $n$ grows to infinity. Thus, the gap in $\lambda$, where this lower bound is invalid, vanishes as the sample size increases to infinity. 
%         \item Regardless of this gap, we argue in Remark \ref{} that we can estimate the Pareto frontier for the performance-cost trade-off efficiently. 
%     \end{itemize}
% \end{remark}


% \SM{compare it to usual rate of convergence for classification when $\lambda = 1$}. 


% \subsection{Efficient learning of oracle routers}
% \label{sec:efficient-learning}
% Let us quickly recall our core idea behind it. For a $\lambda \in [0, 1]$ the true loss regression function $\eta_{\lambda, m}^\star(X)$ for the oracle router $g_\lambda^\star (X) = \argmin_m \eta_{\lambda, m}^\star(X)$ is  decomposed as: 
% \begin{equation} \label{eq:oracle-router}
%     \eta_{\lambda, m}^\star(X) = \lambda \Phi^\star_m(X) + (1 - \lambda) \kappa_m(X), ~ \Phi^\star _m(X) = \Ex_P[\ell\{ Y, f_m(X)\} \mid X ]\,. 
% \end{equation} Since we already know $\kappa_m(X)$ at a new $X$ the only unknown is the $\Phi^\star_m(X)$. Thus, we can plug-in its estimate  $\hat \Phi_m(X)$ within eq. \eqref{eq:oracle-router} and estimate the oracle router as:
% \begin{equation}\label{eq:plugin-router}
%     \hat g_\lambda(X) = \argmin_m \hat \eta_{\lambda, m}(X), ~~ \hat \eta_{\lambda, m}(X) = \lambda \hat \Phi_m(X) + (1 - \lambda) \kappa_m(X)  
% \end{equation} 
% Moreover, we evaluate their prediction errors and costs on a test split of the dataset as: 
% \begin{equation}
%    \textstyle  \hat \cE_\lambda  =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \ell\{Y_i', f_{\hat g_\lambda(X_i')}(X_i')\}, ~~ \hat \cC _\lambda =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \kappa_{\hat g_\lambda(X_i')}(X_i')\,. 
% \end{equation} 
% This plug-in approach is computationally efficient, as we can estimate oracle routers for all $\lambda$ in one go, instead of minimizing \ref{eq:ERM} at different $\lambda$'s. In addition to being computationally efficient, through a study on the minimax upper bound on excess risk in the next section we establish that this plug-in approach is also statistically efficient. Furthermore, we extend this approach to a general multi-objective classification problem. For now, we end this section by summarizing our steps in Algorithm \ref{alg:pareto-routers}. 


% \begin{algorithm}
%     \begin{algorithmic}[1]
% \Require Dataset $\cD_n$
% \State Randomly split the dataset into training and test splits: $\cD_n = \cD_{\text{tr}} \cup \cD_{\text{test}}$. 
% \State  Learn an estimate $\hat \Phi_m (X)$ of $\Phi_m^\star(X)$ using the training split $\cD_{\text{tr}}$. 
% \For{$\lambda \in [0, 1]$}
% \State  Define $\hat \eta_{\lambda, m}(X) =  \lambda \hat \Phi_m(X) + (1 - \lambda) \kappa_m(X)  $ and 
%  $\hat g_\lambda(X) = \argmin_m \hat \eta_{\lambda, m}(X)$. If there is a tie within the $\argmin$, break the tie randomly.
%  \State Calculate $\hat \cE_\lambda  =  \frac1{|\cD_{\text{test}}|} \sum_{(X, Y) \in \cD_{\text{test}}}  \ell\{Y, f_{\hat g_\lambda(X)}(X)\}$
%  \State \quad\quad  and $\hat \cC_\lambda  =  \frac1{|\cD_{\text{test}}|} \sum_{(X, Y) \in \cD_{\text{test}}}  \kappa_{\hat g_\lambda(X)}(X)$
% \EndFor

% \Return $\{g_\lambda: \lambda \in [0, 1]\}$ and $\hat\cF = \{(\hat \cE_\lambda, \hat \cC_\lambda): \lambda \in [0, 1]\}$. 
% \end{algorithmic}
% \caption{Learning of oracle routers}
% \label{alg:pareto-routers}
% \end{algorithm}


% \SM{talk about the computational efficiency, that we can obtain all the routers in one go. Also, provide a teaser that in the next section we shall establish that its statistically efficient as well.}





% Given a router $\hat g:[0, 1]^d \to \Delta^ L$ we define the excess risk as:
% \begin{equation}
%    \textstyle \cE_P (\hat g) = \cR_P(\hat g) - \cR_P(g^\star) = \Ex_P\big[\sum_{l = 1}^L\{g_l(x_0)- g_l^\star(X_0)\}\kappa_\lambda(X_0 , l) \big]
% \end{equation} We shall show that 
% \begin{equation}
%    \inf_{\hat g} \sup_{P\in \cP} \textstyle \Ex_P \big[ \cE_\lambda (\hat g) \big ] \asymp n ^{- \frac{\alpha(1 + \gamma)}{2\alpha + d}}\,.
% \end{equation}



\subsection{The upper bound }\label{sec:upper-bound}
Next, we show that if algorithm the $A_n$ corresponds to CARROT, the performance of $\hat{g}_{\mu}$ matches the lower bound in Theorem \ref{thm:lower-bound} (\cf\ equation \ref{eq:lower-bound}). En-route to attaining $\hat{g}_{\mu}$, we need an estimate $\hat \Phi(X)$ of $\Phi(X) = \Ex_P[Y \mid X ]$. %In this section, we ask what is the needed performance of this estimate? More importantly, we also study if the plug-in approach leads to statistically efficient estimates of the oracle routers, or in other words does the performance of $\hat{g}_{\mu}$ match \ref{eq:lower-bound} 
Our strategy will consist of two steps: 
\begin{itemize}
    \item First,  we establish an upper bound on the rate of convergence for excess risk \eqref{eq:excess-risk} for the plug-in router in terms of the rate of convergence for $\hat \Phi(X)$. 
    \item Then we discuss the desired rate of convergence in $\hat \Phi(X)$ so that the upper bound has the identical rate of convergence to the lower bound \eqref{eq:lower-bound}. Later in Appendix \ref{sec:reg-fn-estimate} we provide an estimate $\hat \Phi(X)$ that has the required convergence rate. 
\end{itemize}
These two steps, together with the lower bound in \eqref{eq:lower-bound} establish that our plug-in router achieves the best possible rate of convergence in excess risk. 

We begin with an assumption that specifies a rate of convergence for $[\hat \Phi(X)]_{m, k}$. 
\begin{assumption} \label{assmp:convergence}
    For some constants $\rho_1, \rho_2 > 0$ and any $n \ge 1$ and $t > 0$ and almost all $X$ with respect to the distribution $P_X$ we have the following concentration bound:
    \begin{align}\label{eq:concentration-phi}
        \max_{P\in \cP} P \big \{ \max_{m, k} a_{k, n}^{-1}\big |[\hat \Phi (X)]_{m, k} - [\Phi  (X)]_{m, k}\big |
        \ge t\big \} \nonumber \\
        \le  \rho_1 \exp\big (- \rho_2  t^2 \big )\,,  
    \end{align}  where for each $k$ the  $\{a_{k,n}; n \ge 1\}\subset (0, \infty)$ is a sequence that decreases to zero. 
\end{assumption}
Using this high-level assumption, in the next theorem, we establish an upper bound on the minimax excess risk for CARROT that depends on both $a_{k, n}$ and $\mu$.  
\begin{theorem}[Upper bound]\label{thm:upper-bound}
  Assume \ref{assmp:convergence}.   If all the $P\in \cP$ satisfy the margin condition \ref{assmp:margin} with the parameters $(\alpha, K_\alpha)$ then there exists a $K> 0$ such that for any $n \ge 1$ and $\mu\in \Delta^{K-1} $ the excess risk for the router $\hat g_\mu$ in Algorithm \ref{alg:pareto-routers} is upper bounded as 
    \begin{equation}
        \max_{P\in \cP} \Ex_{\cD_n}\big [\cE_P(\hat g_\lambda,\lambda)\big ] \le\textstyle K \big \{\sum_{k = 1}^{K_1} \mu_k a_{k, n}\big\}^{1+\alpha} \,.
    \end{equation}
\end{theorem} 
% \begin{remark} \label{remark:upper-bound-lambda}
%     Recall the Remark \ref{remark:lower-bound-lambda}, where we discuss that it is easier to route for smaller $\lambda$. Indeed, under Assumption \ref{assmp:convergence} the same holds for $\hat \eta_{\lambda, m}(X) -  \eta_{\lambda, m}^\star(X) = \lambda \{ \hat \Phi_m(X) - \Phi^\star_m(X)\}$ at a rate $\lambda a_n^{-1}$, which, under the $\alpha$-margin condition (Assumption \ref{assmp:margin}), reveals such a dependence for the minimax upper bound on $\lambda$. 
% \end{remark}


\begin{remark}[Rate efficient routers] \label{cor:efficient-routers}
    When $a_{k, n} = n^{-\nicefrac{\gamma_k}{(2\gamma_k +d)}}$ the upper bound in Theorem \ref{thm:upper-bound} has the $\cO(\{\sum_{k = 1}^{K_1}\mu_k n^{-\nicefrac{\gamma_k}{(2\gamma_k+d)}}\}^{1+\alpha})$-rate, which is identical to the rate in the lower bound (\cf\ Theorem \ref{thm:lower-bound}), suggesting that the minimax optimal rate of convergence for the routing problem is 
\begin{equation}
    \label{eq:minimax-rate}
     \textstyle  \min\limits_{A_n \in \cA_n} \max\limits_{P \in \cP} ~~ \cE_P(A_n, \lambda) \asymp \textstyle  \cO\big ( \big \{\sum_{k = 1}^{K_1} \mu_k n^{- \frac{\gamma_k}{2\gamma_k + d}}\big\}^{1+\alpha}\big ) \,.
\end{equation}
   Following this, we conclude: When $a_{k, n} = n^{-\nicefrac{\gamma_k}{(2\gamma_k +d)}}$ the plug-in approach in Algorithm \ref{alg:pareto-routers}, in addition to being computationally efficient, is also minimax rate optimal. 
%\begin{enumerate}
   % \item When $a_{k, n} = n^{-\nicefrac{\gamma_k}{(2\gamma_k +d)}}$ the plug-in approach in Algorithm \ref{alg:pareto-routers}, in addition to being computationally efficient, is also minimax rate optimal in excess risk. 
   % \item  Following up on the Remark  \ref{remark:minimax-lower-bound}, this result generalizes the minimax study of non-parametric binary classification to (a) more than two classes, and (b) classification loss functions beyond $0/1$-loss. 
%\end{enumerate}
\end{remark} 
An example of an estimator $\hat{\Phi}$ that meets the needed conditions for $a_{k, n} = n^{-\nicefrac{\gamma_k}{(2\gamma_k +d)}}$ to hold is described in Appendix \ref{sec:reg-fn-estimate}. 
% \begin{remark} \label{remark:difficulty-routing}
% The optimal rate of convergence in \eqref{eq:minimax-rate} is particularly small for small values of $\sum_{k = 1}^{K_1} \mu_k$; in fact, it's identical to zero when $\sum_{k = 1}^{K_1} \mu_k = 0$. This is quite intuitive from the expression of $g_\mu^\star$ in Lemma \ref{lemma:oracle-router}.  For $\sum_{k = 1}^{K_1} \mu_k = 0$ the $g_\mu^\star(X) = \argmin_{m} \{\sum_{k\ge K_1+1} \mu_k [\Phi(X)]_{m, k}\}$ is precisely known to us, thus the excess risk for routing is identical to zero.
    
% \end{remark}

   
%     This leads to the two following conclusions: 
%     \begin{enumerate}
%         \item For any $\lambda$ the minimax optimal rate of convergence for the routing problem is 
%         \[
%         \textstyle \textstyle  \min_{A_n \in \cA_n} \max_{P \in \cP} ~~ \cE_P(A_n, \lambda) \asymp  \cO\big ( \big\{\lambda n^{-\nicefrac{\beta}{(2\beta+d)}}\big\}^{1+\alpha}\big ) \,.
%         \] 
%         This reveals 
        
        
%         Unsurprisingly, this is identical to the optimal rate of convergence in non-parametric classification problems \citep{audibert2007Fast}. Repeating the intuition again, for a fixed $\lambda$ the routing problem 
%         is essentially a multiclass identical minimax optimal rate of convergence for excess risk. 
%         \item  A more interesting observation is that if $\hat \Phi_m$ converges to $\Phi_m^\star$ at a rate $a_n^{-\frac{1}{2}} = n^{-\frac{\beta}{2\beta +d}}$ then our one-shot approach in Algorithm \ref{alg:pareto-routers} achieves this optimal minimax rate of convergence in excess risk and thus is a \emph{rate efficient} estimator for Pareto routers. We shall show later in Section \ref{sec:reg-fn-estimate} that a local polynomial regression estimator with a suitable bandwidth achieves this desired rate. 
%         \end{enumerate}



% \begin{remark}
%     Remark about the importance of $\lambda$. 
% \end{remark}

% \begin{remark}
%     Let us quickly recall the gap in the validity in our lower bound in Theorem \ref{thm:lower-bound}, that the rate in the lower bound is not true when $0 < \lambda < c_1 n ^{\frac{\beta - \nicefrac{d}{\alpha}}{2\beta +d}}$. However, the rate in the upper bound continues to hold for all $0 \le \lambda \le 1$. 
% \end{remark}


% Now, we make this statement precise and show that for such an $\hat \Phi $ the excess risk \eqref{eq:excess-risk} achieves the rate in the lower bound \eqref{eq:lower-bound}. 

% \begin{theorem}[Upper bound]\label{thm:upper-bound}
%     Suppose that for some $\rho_1, \rho_2 > 0$ and any $n \ge 1$ and $t > 0$ and almost all $x$ with respect to $P_X$ we have the following concentration bound for $\hat \Phi$:
%     \begin{equation}\label{eq:concentration-phi}
%         \max_{P\in \cP} P_{\cD_n} \big \{ \|\hat \Phi(x) - \Phi^\star (x)\|_1 \ge t\big \} \le  \rho_1 \exp\big (- \rho_2 a_n t^2 \big )\,, 
%     \end{equation}
%     where $\{a_n; n \ge 1\}\subset \reals$ is a sequence that increases to $\infty$.  
%     Fix a $\lambda \in [0, 1]$.  Then, if all the $P\in \cP$ satisfies the margin condition \ref{assmp:margin} with the parameters $(\alpha, K_\alpha)$ then there exists a $K> 0$ such that for any $n \ge 1$ the excess risk for the router $\hat g_\lambda$ in \eqref{eq:eff-estimate-router} is upper bounded as 
%     \begin{equation}
%         \max_{P\in \cP} \Ex_{\cD_n}\big [\cE_P(\hat g_\lambda,\lambda)\big ] \le K a_n^{-\frac{1+ \alpha}{2}}\,. 
%     \end{equation}
%     Thus, as long as $a_n = n^{{  2\beta/(2\beta + d)}}$  for any $\lambda \in [0, 1]$ the excess risk for the router $\hat g_\lambda$ in \eqref{eq:eff-estimate-router} has the rate of convergence $a_n^{- {(1 + \alpha)}/{2}} = n^{- {\beta(1 + \alpha)}/{(2\beta + d)}}$ that matches with the lower bound rate in \eqref{eq:lower-bound}. 
% \end{theorem}






% \subsection{Efficiency of the estimation Pareto frontier}

% As mentioned in Section \ref{sec:efficient-learning} and Algorithm \ref{alg:pareto-routers} we estimate the performance-cost trade-off for Pareto routers in a very simple manner: first estimate the Pareto routers $\hat g_\lambda$ in a training split of the dataset, then evaluate their average performances and costs in the remaining test split as
% \[
% \textstyle \hat \cE_\lambda  =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \ell\{Y_i', f_{\hat g_\lambda(X_i')}(X_i')\}, ~~ \hat \cC _\lambda =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \kappa_{\hat g_\lambda(X_i')}(X_i')\,. 
% \] In this section we evaluate the efficiency of estimating the Pareto front $\{ (\hat \cE_\lambda, \hat \cC_\lambda): 0 \le \lambda \le 1\}$ in this manner. Note that the true Pareto front is $\{ ( \cE_\lambda^\star,  \cC_\lambda^\star): 0 \le \lambda \le 1\}$ where 
% \[
% \textstyle \cE^\star_\lambda = \Ex_P [\ell\{ Y, f_{g_\lambda^\star(X)}(X)\}], ~~ \cC_\lambda^\star =  \Ex_P [\kappa _{g_\lambda^\star(X)}(X)]\,. 
% \] To evaluate their differences, focus only on $\hat \cE_\lambda - \cE_\lambda^\star$, as the analysis of $\hat \cC_\lambda - \cC_\lambda^\star$ is very similar. Defining $\widetilde \cE_\lambda = \Ex_P [\ell\{ Y, f_{\hat g_\lambda(X)}(X)\}]$, we can decompose the difference as 
% \begin{equation}
%     \textstyle \hat \cE_\lambda - \cE_\lambda^\star = \{\hat \cE_\lambda - \widetilde \cE_\lambda\}  + \{\widetilde \cE_\lambda-  \cE_\lambda^\star\} 
% \end{equation} The first term is $\cO (n^{-\nicefrac12})$. Now, to bound the second term, notice that 
% \[
% \textstyle \cE_P(\hat g_\lambda,\lambda) \le 
% \]


% that for $h = n ^{-1/(2\beta + d)}$ the concentration bound in \eqref{eq:concentration-phi} is satisfied with $a_n = n^{-2\beta/(2\beta + d)}$, therefore the router derived from such $\hat\Phi$ using \eqref{eq:eff-estimate-router} achieves the same rate of convergence as in the lower bound \eqref{eq:lower-bound}, \ie\ rate optimal. 

==> sections/mild_density.tex <==
\section{Minimax study under mild density condition}

==> sections/setup.tex <==
\section{Plug-in approach to routing}
\label{sec:setup}

%To describe the approach, let us introduce some notation. We have $M$ pre-trained LLMs indexed as $m \in [M] = \{1, \dots, M\}$ and $K$ metrics indexed as $k\in [K] = \{1, \dots, K\}$. %Throughout our paper, we index the models as $m \in [M]$ and the metrics as $k \in [K]$. 
%We denote a generic input or query as $X\in \cX$, where $\cX$ is the space of inputs.  Thus, for any input $X$, the metrics of interest are stored in a $M\times K$ matrix. We denote this matrix as $Y \in \reals^{M \times K}$, whose $(m, k)$-th entry $[Y]_{m, k}$ is the metric value for obtaining a prediction from the $m$-th model evaluated with respect to $k$-th metric.  For all metrics, we assume that a lower value is preferred. With this convention, we shall also refer to them as risks. For a probability distribution $P$ in the sample space $\cX \times \reals^{M\times K}$ we assume that the training dataset $\cD= \{(X_i, Y_i)\}_{i = 1}^n$ is an $\iid$ sample from $P$. 


We will consider a convex combination of our $K$ metrics with coefficients $\mu \in \Delta^{K-1} \triangleq \{(\mu_1, \dots, \mu_K): \mu_k \ge 0, \sum_k \mu_k = 1\}$ and a generic point $(X, Y)\sim P$. The $\mu$-th convex combination of the risks (or, $\mu$-th risk) can be written as $Y\mu\in \reals^{M}$, with the risk incurred for obtaining a prediction from the $m$-th model is 
\[
\textstyle [Y\mu]_m = \sum_{k = 1}^K [Y]_{m, k} \mu_k\,.
\] We want to learn a predictive router $g: \cX \to [M]$, that takes $X$ as an input and predicts the index of the LLM to be used for inference. The average $\mu$-th risk for using the router $g$ is 
\begin{equation}\label{eq:RM}
  \textstyle   \cR_P(g, \mu) = \Ex\big [\sum_{m = 1}^M[Y\mu]_m \bbI\{g(X) = m\} \big]\,. 
\end{equation} For a given $\mu$ let us refer to the minimizer $g_\mu^\star$ as an oracle router. Remember our objective: we would like to learn the oracle routers $g_\mu^\star$ at every value of $\mu$. While one may minimize an empirical risk corresponding to $\cR_P(g, \mu)$ to estimate the oracle router at a particular $\mu$, this approach is not scalable, any small change in $\mu$ would require refitting a new router. Given this, we develop a plug-in approach which lets us estimate the oracle routers at every value of $\mu$. The key intuition lies within an explicit form of the $g_\mu^\star$ that we provide in the next lemma. 
\begin{lemma} \label{lemma:oracle-router}
    Let us define $\Phi(x) = \Ex [Y\mid X = x]$ and $\eta_{\mu, m}(x) = \sum_{k = 1}^K \mu_k [\Phi (x)]_{m, k} $. Then for any $\mu\in \Delta^{K-1}$ the oracle router that minimizes $\cR_P(g, \mu)$ is 
    \begin{align} \label{eq:oracle-router-2}
        \textstyle g_\mu^\star(X) & \textstyle = \argmin_m ~ \eta_{\mu, m} (X)\\ 
       & \textstyle  = \argmin_m \big\{ \sum_{k = 1}^K \mu_k [\Phi (X)]_{m, k} \big\} \, \nonumber.
    \end{align}
\end{lemma}
The key conclusion of \ref{lemma:oracle-router} is the expression $ g_\mu^\star(X)= \argmin_m \{ \sum_{k = 1}^K \mu_k [\Phi (X)]_{m, k} \} $. %where we have isolated the effects of $\mu$. 
It suggests a straightforward approach to estimate $g_\mu^\star(X)$ at all values of $\mu$.  Namely, we only need to plug-in an estimate of $\Phi(X) = \Ex[Y \mid X]$ to the expression of $g_\mu^\star(X)$. Compared to minimizing empirical risk at different values of $\mu$, this plug-in approach is more scalable if the practitioner plans on tuning $\mu$. %In addition to estimating the routers, we also estimate the average risks 
%\[
%\textstyle \cR(\mu, k) = \Ex \big[\sum_{m = 1}^M[Y]_{m, k} \bbI\{g_\mu^\star(X) = m\}\big]
%\]
%on a test split of the dataset, which would be useful for understanding the trade-off across different risks.
We summarize our approach in algorithm \ref{alg:pareto-routers}. 
\begin{algorithm}
    \begin{algorithmic}[1]
\REQUIRE Dataset $\cD_n$
\STATE Randomly split the dataset into training and test splits: $\cD_n = \cD_{\text{tr}} \cup \cD_{\text{test}}$. 
\STATE  Learn an estimate $\hat \Phi (X)$ of $\Phi(X)$ using the $\cD_{\text{tr}}$. 
\FOR{$\mu \in \Delta^{K-1}$}
\STATE  Define $\widehat g_\mu(X) = \argmin_m \widehat \eta_{\mu, m}(X)$ where $\widehat \eta_{\mu, m}(X) =  \sum_{k = 1}^K \mu_k [\widehat \Phi (X)]_{m, k}   $. Break any tie within $\argmin$ randomly.
 \STATE Calculate 
 
 $\widehat \cR(\mu, k)  =  \frac1{|\cD_{\text{test}}|} \sum\limits_{(X, R) \in \cD_{\text{test}}}  [R]_{m, k} \bbI\{ \widehat g_\mu(X) = m\} $
\ENDFOR

\STATE {\bfseries Return:} $\{\widehat g_\mu: \mu \in \Delta^{K-1}\}$ and $ \{\widehat \cR(\mu, k): \mu \in \Delta^{K-1}, k\in [K]\}$. 
\end{algorithmic}
\caption{CARROT}
\label{alg:pareto-routers}
\end{algorithm}

%\begin{algorithm}[H]
  % \caption{ICL Refinement}\label{alg:label improvement}
%\begin{algorithmic}
  % \STATE {\bfseries Input:} Corrupted label pairs $\tilde{D}: \{(X_i, \tilde{Y}_i)\}_{i=1}^n$, source LLM $\cS$.
   %\REPEAT
   %\STATE Initialize $noChange = true$.
 %  \FOR{$i =1, 2, \dots, n$}
   %\IF{$x_i > x_{i+1}$}
  % \STATE Select in-context-learning examples  $\tilde{D}_{\text{ICL}}^i: \{(X_j, \tilde{Y}_j)\}_{j=1}^{n_{\text{ICL}}}$ from $\tilde{D}\backslash\{(X_i, \tilde{Y}_i)\}$
 %  \STATE Construct concatenated prompt $[\tilde{D}^i_{\text{ICL}} \circ X_i]$, and draw re-sampled label $\hat{Y}_i \sim \cS(\cdot|[\tilde{D}_{\text{ICL}} \circ X_i] )$.
   %\ENDIF
  % \ENDFOR
  % \STATE {\bfseries Return:} $\hat{\cD} \triangleq \{X_i, \hat{Y}_i\}_{i=1}^n$
   %\UNTIL{$noChange$ is $true$}
%\end{algorithmic}
%\end{algorithm}

%\SM{talk a bit about interpretibility and computational efficiency}

==> sections/upper-bound.tex <==
\section{Efficient learning of Pareto routers} 
\label{sec:efficient-learning-algorithm}


\subsection{The upper bound}\label{sec:upper-bound}

Recall in Algorithm \ref{alg:pareto-routers} we say that we require an ``efficient estimate'' $\widehat \Phi$ of the function $\Phi^\star$, whose $l$-th coordinate is $\Phi^\star_l(x) = \Ex_P[\ell\{Y, f_l(X)\mid X = x]$. Now, we make this statement precise and show that for such an $\widehat \Phi $ the excess risk \eqref{eq:excess-risk} achieves the rate in the lower bound \eqref{eq:lower-bound}. 

\begin{theorem}[Upper bound]\label{thm:upper-bound}
    Suppose that for some $\rho_1, \rho_2 > 0$ and any $n \ge 1$ and $t > 0$ and almost all $x$ with respect to $P_X$ we have the following concentration bound for $\widehat \Phi$:
    \begin{equation}\label{eq:concentration-phi}
        \max_{P\in \cP} P_{\cD_n} \big \{ \|\widehat \Phi(x) - \Phi^\star (x)\|_1 \ge t\big \} \le  \rho_1 \exp\big (- \rho_2 a_n t^2 \big )\,, 
    \end{equation}
    where $\{a_n; n \ge 1\}\subset \reals$ is a sequence that increases to $\infty$.  
    Fix a $\lambda \in [0, 1]$.  Then, if all the $P\in \cP$ satisfies the margin condition \ref{assmp:margin} with the parameters $(\alpha, K_\alpha)$ then there exists a $K> 0$ such that for any $n \ge 1$ the excess risk for the router $\widehat g_\lambda$ in \eqref{eq:eff-estimate-router} is upper bounded as 
    \begin{equation}
        \max_{P\in \cP} \Ex_{\cD_n}\big [\cE_P(\widehat g_\lambda,\lambda)\big ] \le K a_n^{-\frac{1+ \alpha}{2}}\,. 
    \end{equation}
    Thus, as long as $a_n = n^{{  2\beta/(2\beta + d)}}$  for any $\lambda \in [0, 1]$ the excess risk for the router $\widehat g_\lambda$ in \eqref{eq:eff-estimate-router} has the rate of convergence $a_n^{- {(1 + \alpha)}/{2}} = n^{- {\beta(1 + \alpha)}/{(2\beta + d)}}$ that matches with the lower bound rate in \eqref{eq:lower-bound}. 
\end{theorem}




% {\bf Question:} How can we find Pareto front solutions efficiently without using a back-tracking technique, \ie\ fit different $g$ for different $\lambda$? The hint is to learn $f^\star(x)$ as $\widehat f(x)$ and for a $\lambda > 0$ then define 
% \[
% \textstyle \widehat g _\lambda (x) = \delta _{\widehat l(x)}, ~~ \widehat l(x) =  \argmin_ l\big\{\ell (\widehat f(x_0), f_l(x_0)) + \lambda c_l (x_0)\big\}
% \] Show that $\widehat g_\lambda$ achieved the rate at lower bound. 


\subsection{Efficient learning of the loss regression function}
\label{sec:reg-fn-estimate}
We consider \emph{local polynomial regression} (LPR) to estimate the loss regression function. For a sample point $Z_i = (X_i, Y_i)$ we define the observed loss vector $\ell_i \in \reals^L$ where $[\ell_i]_l = \ell\{Y_i,f_l(X_i)\}$. Consider a symmetric kernel $\psi: \reals^d \to \reals_+$ and define $\Theta(\lfloor \beta \rfloor)$ as the class of all $\lfloor \beta \rfloor$-degree polynomials from $\reals^d$ to $\reals$. For a bandwidth $h > 0$ we define the LPR estimate as 
\begin{equation}
    \widehat \Phi_l(x) = \widehat\theta_x^{(l)}(0), ~~ \widehat \theta_x^{(l)} \in \argmin_{\theta \in \Theta(\lfloor \beta \rfloor)}  \textstyle \sum_{i = 1}^n \psi (\frac{X_i - x}{h}) \big [\ell \{Y_i, f_l(X_i)\} - \theta (X_i -x )\big]^2 \,. 
\end{equation}
In their Theorem 3.2 \citet{audibert2007Fast} establishes that for $h = n ^{-1/(2\beta + d)}$ the concentration bound in \eqref{eq:concentration-phi} is satisfied with $a_n = n^{-2\beta/(2\beta + d)}$, therefore the router derived from such $\widehat\Phi$ using \eqref{eq:eff-estimate-router} achieves the same rate of convergence as in the lower bound \eqref{eq:lower-bound}, \ie\ rate optimal. 

==> sections_arxiv/extensions.tex <==
\section{Routing in a general multi-objective framework}\label{sec:general-multi-obj}

In this section, we discuss a natural extension of the routing problem with general metrics. Since most of the constructions are very similar to the construction in the Introduction section \ref{sec:intro}, we keep our discussion short.  Say, we are provided $M$ pre-trained models, denoted as $f_1, \dots,f_M$. Given model $f_m$ and a sample point $(X, Y)$,  we are interested in $L$ different loss metrics, among which the first $L_1 $ many, denoted as $\ell_1\{f_m; X, Y\} , \dots, \ell_{L_1}\{f_m; X, Y\}$, depends on $f_m$, $X$ and $Y$, while the next $L_2 = L - L_1$ many, denoted as $\ell_{L_1+ 1}(f_m; X), \dots , \ell_{L}(f_m; X)$, depends only on $f_m$ and $X$.  In that case we consider a compromise between these $L$ losses: for an $\lambda = (\lambda_1 , \dots, \lambda_L) \in\Delta^{L-1} $ the linear loss trade-off in eq. \eqref{eq:linearized-loss} naturally extends to 
\begin{equation} \label{eq:linearized-loss-gen}
 \textstyle \eta_{\lambda, m}(X, Y) =  \sum_{l = 1}^{L_1}\lambda_l \ell_l\{f_m; X, Y\} + \sum_{l = L_1 + 1}^{L}\lambda_l \ell_l\{f_m; X\}   \,.
\end{equation} 
To make it even more general, assume that we have a classification task with $M$ classes, \ie \ the outcome $Y \in \{1, \dots, M\}$ is now categorical. Additionally, as a multi-objective problem we have $L$ different loss metrics, among which the first $L_1 $ many $\ell_1\{m; X, Y\} , \dots, \ell_{L_1}\{m; X, Y\}$ are losses  of predicting a sample $(X, Y)$ as the class $m$, while the next $L_2 = L - L_1$ many $\ell_{L_1+ 1}\{m; X\}, \dots , \ell_{L}\{m; X\}$ is the cost of predicting the sample $X$ as the class $m$. Then the aggregated loss is 
\begin{equation} \label{eq:linearized-loss-gen-2}
 \textstyle \eta_{\lambda, m}(X, Y) =  \sum_{l = 1}^{L_1}\lambda_l \ell_l\{m; X, Y\} + \sum_{l = L_1 + 1}^{L}\lambda_l \ell_l\{m; X\}   \,.
\end{equation} 

For a particular $\lambda \in \Delta^{L-1}$ we want to estimate the optimal/Bayes/admissible classifier $g_\lambda^\star$ that minimized the average of the aggregates loss trade-off:
\begin{equation}
    \textstyle g_\lambda^\star = \argmin_{g: \cX \to [M]}  \Ex_P\big[\sum_{m = 1}^M \bbI\{g(X) = m\} \eta_{\lambda, m} (X, Y) \big ]
\end{equation}
Similar to Lemma \ref{lemma:oracle-router}, defining $\Phi_{l, m}^\star(X) = \Ex[\ell_l\{f_m; X,Y\} \mid X]$ for $l \in [L_1]$ and $\Phi_{l, m}^\star(X) = \ell_l\{f_m; X\} $ for $l \in \{L_1 + 1, \dots, L\}$ the Bayes classifier $g_\lambda^\star$ has the explicit form  (\cf\ Lemma \ref{lemma:bayes-classifier-gen})
\begin{equation}\label{eq:oracle-router-gen}
  \textstyle  g_\lambda^\star (X) = \argmin_m  \eta_{\lambda, m}(X), ~~ \eta_{\lambda, m}(X) = \sum_{l = 1}^L \lambda_l \Phi_{l, m}^\star (X)\,.
\end{equation}
A natural extension of Algorithm \ref{alg:pareto-routers} requires us to estimate each of the functions $\Phi_{l, m}^\star$ as $\widehat \Phi_{l, m}$ then estimate all Bayes classifiers in a one-shot plug-in approach as:
\[
\textstyle \widehat g_\lambda(X) = \argmin_m  \{\sum_{l = 1}^L \lambda_l \widehat \Phi_{l, m} (X) \}\,.
\] 
Note that, for $l \ge L_1+ 1$ the functions $\Phi_{l, m}^\star$ are known, so they need not be estimated; in these cases, we simply let $\widehat \Phi_{l, m} = \Phi_{l ,m}^\star$. 
Having estimated $\widehat g_\lambda$, we can then evaluate them on a test data split with respect to each of the individual metrics to estimate the Pareto frontier and examine the optimal trade-off between the objectives.
We describe the procedure in Algorithm \ref{alg:pareto-routers-gen}.  

\begin{algorithm}
    \begin{algorithmic}[1]
\Require Dataset $\cD_n$
\State Randomly split the dataset into training and test splits: $\cD_n = \cD_{\text{tr}} \cup \cD_{\text{test}}$. 
\State  Learn estimates $\widehat \Phi_{l, m} (X)$ of the function $\Phi_{l, m}^\star(X)$ using the training split $\cD_{\text{tr}}$. 
\For{$\lambda \in \Delta^{L-1}$}
\State  Define $\widehat \eta_{\lambda, m}(X) =  \sum_{l = 1}^L \lambda_l \widehat \Phi_{l, m} (X)  $ and 
 $\widehat g_\lambda(X) = \argmin_m \widehat \eta_{\lambda, m}(X)$
 \For{$l \in \{1, \dots, L\}$}
 \State Calculate $\widehat \cE_{l, \lambda}  =  \frac1{|\cD_{\text{test}}|} \sum_{(X, Y) \in \cD_{\text{test}}}  \ell_l\{Y, f_{\widehat g_\lambda(X)}(X)\}$
 \EndFor
\EndFor

\Return $\{g_\lambda: \lambda \in \Delta^{L-1}\}$ and $\widehat\cF = \{(\widehat \cE_{1, \lambda}, \dots, \widehat \cE_{L, \lambda}): \lambda \in \Delta^{L-1}\}$. 
\end{algorithmic}
\caption{Learning of Bayes classifiers}
\label{alg:pareto-routers-gen}
\end{algorithm}


Except for some minor differences, the minimax rate analysis of the estimate of $g_\lambda^\star$ is identical to Section \ref{sec:lower-bound}. We assume that
\begin{enumerate}
    \item For $1 \le l \le L_1$ the $\Phi_{l, m}^\star$ functions are $(\beta_l, K_{\beta, l})$-smooth, which is similar to the Assumption \ref{assmp:smooth}. Recall the discussion following Assumption \ref{assmp:smooth}; (1) Since $\Phi_{l, m}$ are known for $l \ge L_1 + 1$ a smoothness assumption on them is not necessary, and (2) We could assume different smoothness for different $\Phi_{l, m}^\star$, \ie\ they are $\beta_{l, m}$ smooth, but the rate will only involve the smallest smoothness, \ie\ $\beta_{l, \min} = \min_m \beta_{l, m}$. Thus, for simplicity, we assume that for a given $l$ the $\beta_{l, m}$ are identical for different $m$. 
    \item The margin condition in Assumption \ref{assmp:margin} is satisfied with the new definition of $\eta_{\lambda, m}(X) = \Ex[\eta_{\lambda, m}(X, Y)\mid X]$ with parameters $(\alpha, K_\alpha)$.
    \item  The $P_X$ is compactly supported and satisfies the strong density condition, as in the assumption \ref{assmp:strong-density}.
\end{enumerate}

%  and that the margin condition is satisfied  Furthermore, we assume the 
% \SM{talk about how the worst smoothness parameter is the one that matters.}


Under these assumptions, we establish the upper and lower bound analysis for the minimax rate of convergence in excess risk
\[
\textstyle \cE_P(g, \lambda) = \cL_P(g, \lambda) - \cL_P(g_\lambda^\star, \lambda)\,.
\]
For this purpose, let us quickly recall the notation and definitions necessary to describe the lower and upper bounds. We denote the class of all probability distributions on $\cX \times \cY$ space by $\cP$.
We also denote $\Gamma = \{g: \cX \to [M]\}$ as the set of all classifiers and $\cA_n$ as the class of learning algorithms, such that an algorithm $\cA_n \ni A_n: \cZ^n \to \Gamma $ that takes the dataset $\cD_n $ as input and produces a classifier $A_n(\cD_n): \cX \to [M]$.

\begin{theorem}
\label{thm:bound-gen}
Suppose that $\max_{l \in  [L_1]}\beta_l <  \nicefrac{d}{\alpha}$. Then we have the following lower and upper bounds for the excess risk. 
\begin{itemize}
    \item {\bf Lower bound:} For $n \ge 1$  and $A_n \in \cA_n$ define $\cE_P(A_n, \lambda) = \Ex_{\cD_n}\big[\cE_P\big(A_n(\cD_n), \lambda\big)\big]$. There exist constants $c_1, c_2> 0$ that are independent of $n$ and $\lambda$ such that for any $n\ge 1$ and $ \lambda \in \Delta^{L-1}$ we have the lower bound
    \begin{equation} \label{eq:lower-bound-gen}
      \textstyle  \min\limits_{A_n \in \cA_n} \max\limits_{P \in \cP} ~~ \cE_P(A_n, \lambda) \ge c \big \{\sum_{l = 1}^{L_1}\lambda_l n^{- \frac{\beta_l}{2\beta_l + d}}\big\}^{1+\alpha} \,.
    \end{equation}  
    \item  {\bf Upper bound:} For $l \le L_1$ and $m\in [M]$ suppose that there are estimators $\widehat\Phi_{l, m}$ for $\Phi^\star_{l, m}$ that satisfies the following: for constants $\rho_{l, 1}, \rho_{l, 2} > 0$ and any $n \ge 1$ and $t > 0$ and almost all $X$ with respect to $P_X$ we have 
    \begin{equation} \label{eq:concentration-phi-gen}
        \max_{P\in \cP} P \big \{ \max_m \big |\widehat \Phi_{l, m} (X) - \Phi^\star_{l, m}  (X)\big |  \ge t\big \} \le  \rho_{l, 1} \exp\big (- \rho_{l,2} a_{l, n}^2 t^2 \big )\,,  
    \end{equation}  where the sequence $\{a_{l, n}; n \ge 1\}\subset (0, \infty)$  increases to $\infty$. Then there exists a $K> 0$ such that for any $n \ge 1$ and $\lambda \in \Delta^{L-1} $ the excess risk for the router $\widehat g_\lambda$ in Algorithm \ref{alg:pareto-routers-gen} is upper bounded as 
    \begin{equation} \label{eq:upper-bound-gen}
      \textstyle   \max\limits_{P\in \cP} \Ex_{\cD_n}\big [\cE_P(\widehat g_\lambda,\lambda)\big ] \le K \big\{ \sum_{l = 1}^{L_1}\lambda_l a_{l, n}^{-1}\big\} ^{1+ \alpha}\,. 
    \end{equation}
    \item  {\bf Local polynomial estimator:} Assume that $\ell_l \{Y_i, f_m(X_i)\}$ are sub-Gaussian, \ie\ there exists constants $c_{l, 1}$ and $c_{l, 2}$ such that  
    \[
    \textstyle P\big ( |\ell_l \{Y, f_m(X)\} | > t \mid X\big ) \le c_{l, 1} e^{-c_{l, 2}t^2}\,. 
    \] If $\psi$ satisfies the regularity conditions with parameter $\beta_l$ in (\cf\ Definition \ref{def:kernel-reg})  and $k = \lfloor \beta_l \rfloor$ then for $h = n^{-\frac{1}{2\beta_l + d}}$ the inequality in \eqref{eq:concentration-phi-gen} holds for 
    \begin{equation}\label{LPR-gen}
    \widehat \Phi_{l, m}(x_0) = \widehat\theta_{x_0}^{(m)}(0), ~~ \widehat \theta_x^{(m)} \in \argmin_{\theta \in \Theta(k)}  \textstyle \sum_{i = 1}^n \psi (\frac{X_i - x_0}{h}) \big [\ell \{Y_i, f_m(X_i)\} - \theta (X_i -x_0 )\big]^2 \,. 
\end{equation}
    with $a_{l, n} = n^{\nicefrac{2\beta_l}{(2\beta_l + d)}}$, where $\Theta(k)$ is the class of all $k$ degree polynomials. 
\end{itemize} 

  
\end{theorem}
% \SM{Discuss the optimality in remarks.} 
\SM{comment about $\max_{l \in  [L_1]}\beta_l <  \nicefrac{d}{\alpha}$.}
We end our section with a few remarks. 

\begin{remark}[Rate optimality for plug-in routers]

Firstly, given that the upper bound in eq.  \eqref{eq:upper-bound-gen} for plug-in router described in Algorithm \ref{alg:pareto-routers-gen} with local-polynomial estimator for $\widehat \Phi_{l, m}(X)$ achieves the same rate of convergence as the lower bound in \eqref{eq:lower-bound} we conclude that the minimax optimal rate of convergence in excess risk is 
\begin{equation} \label{eq:optimal-rate-gen}
    \textstyle \min\limits_{A_n \in \cA_n} \max\limits_{P \in \cP} ~~ \cE_P(A_n, \lambda) \asymp \cO \Big(\big \{\sum_{l = 1}^{L_1}\lambda_l n^{- \frac{\beta_l}{2\beta_l + d}}\big\}^{1+\alpha}\Big)\,. 
\end{equation} Moreover, this also implies that the plug-in router can achieve this optimal rate as long as the bounds in eq. \eqref{eq:concentration-phi-gen} are satisfied with $a_{l, n} = n^{\nicefrac{2\beta_l}{(2\beta_l + d)}}$. 
    
\end{remark}

\begin{remark}[Difficulty in routing with respect to $\lambda$]
Moreover, the rate in eq. \eqref{eq:optimal-rate-gen} implies that for a smaller $\lambda_l$ the errors in estimating $\Phi_{l, m}^\star$ have a lesser impact on the excess risk convergence. This conclusion is very much related to our Remark \ref{remark:diff-in-lambda-lb}, and thus we keep our discussion brief and ask readers to revisit the said remark. We end with a quick observation that the hardest instance to classify is when $\lambda_{l_{\min}} = 1$ for the lowest smoothness parameter, \ie\ $l_{\min} = \argmin_{l \le L_1} \beta_l$. 

    
\end{remark}


\begin{remark}

{\bf (Minimax rate study for non-parametric classification with multiple objectives)}
Compared to \citet{audibert2007Fast}, our study of the optimal minimax rate provided in this section generalizes the setting on three fronts: (1) the number of classes can be more than two, (2) general classification loss functions beyond $0/1$-loss and (3) multiple objectives. In this general setting, we show that the plug-in classifiers described in Algorithm \ref{alg:pareto-routers-gen} are both computationally and statistically (rate optimal) efficient for estimating the entire class of Bayes classifiers $\{g_\lambda^\star: \lambda\in \Delta^{L-1}\}$. 
    
\end{remark}

==> sections_arxiv/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Consider a prediction task: Let $(X, Y)$ be a random pair that takes a value in the space $\cZ \triangleq \cX \times \cY$ with a joint distribution $P$. We consider $X \in \cX \subset \reals^d $ as covariates and $Y \in \cY$ as the response, and given $X$ we want to predict $Y$ as a function of $X$.  Although the standard approach would be to learn a prediction model $f: \cX \to \cY$ from $\cD$ using statistical learning methods, learning such $f$ is often very challenging due to the requirement of a large sample size and computing resources. 


Consider a standard prediction task: for an $(X, Y) \in \cX \times \cY$ drawn from the distribution $P$ we want to predict $Y$ using $X$, where $\cX \subset \reals^d$ is the covariates space and $\cY$ is the response space. For the prediction task, we want to learn a predictor $f : \cX \to \cY$ such that, given a new $(X, Y) \sim P$, the error in predicting $Y$ as $f(X)$ is as small as possible. To learn such $f$, we have a dataset $\cD_n = \{(X_i, Y_i)\}_{i = 1}^n \subset \cX \times \cY$ of size $n$ drawn \emph{i.i.d.} from the distribution $P$, and a standard statistical technique is to estimate $f$ by minimizing an empirical risk calculated with $\cD_n$. 
In this paper, we are particularly interested in prediction tasks in which learning $f$ in such a manner is very challenging or even impossible due to the requirements of a large sample size and computing resources. Instead, we have access to a collection of pre-trained models $f_1, \dots, f_M: \cX \to \cY$ that may aid our prediction task, and for a new $X$ we want to pick the ``best capable'' model for prediction.  


As a motivating example, consider the task of building a question and answering (Q\&A) system, \ie\ we want to learn a large language model (LLM) for text generation, which, given a question, generates the correct answer. As is well known by now, training such models from scratch is notoriously difficult in terms of their required data and computation resources, and is certainly outside of the capacity of an everyday researcher. As a more feasible approach, we turn to the Internet, where a collections of pre-trained LLMs are readily available for our use. Rather than training an LLM from scratch, we pick the ``best capable'' model to answer a question.


% But LLMs come in a wide variety of LLMs exist; in terms of their \emph{sizes}, which can range in size from one billion to hundreds of billions of parameters; \emph{expertise}, based on the dataset on which it has been trained, \eg text, math or science Q\&A, as well as \emph{costs} to obtain a prediction.
% Broadly speaking, larger models tend to be more capable but
% come at a higher cost, while smaller models tend to be less capable but cheaper to serve.
% Thus, a learner is presented with the problem of choice: given a new question, which LLM is best suited? 


There is a wide variety of LLMs available in the Internet --- their \emph{sizes} range from less than a billion to hundreds of billion of parameters; they may have a diverse \emph{expertise} based on their training datasets, \eg\ reasoning, math or coding Q\&A's; as well as their \emph{costs} of prediction might also be different. Broadly speaking, larger models (\eg\ GPT4) tend to be more capable but
come at a higher cost, while smaller models tend to be less capable but are cheaper to serve. 
In terms of model capability, we focus on the two following metrics: 
\begin{itemize}
    \item {\bf Prediction error:} we have a prediction loss function $\ell$ such that the error in predicting a response $Y$  as $f_m(X)$ from the $m$-th model is $\ell\{Y, f_m(X)\} \in \reals$. We want to pick the model with the smallest prediction error. 
    \item {\bf Prediction cost:} together with a pre-trained model $f_m$, we also have a cost function $\kappa_m: \cX \to \reals$ that, given an input $X$, quantifies the cost of obtaining the prediction $f_m(X)$ as $\kappa_m(X)$. Usually, the prediction cost for an LLM is related to factors such as the sizes of models, input tokens, etc. 
\end{itemize}
Intuitively, we would like to use a more expensive model like GPT4 for a question that is difficult to answer. On the other hand, a smaller model with less prediction cost might be sufficient for a question that is easy to answer. Thus, we want to find the LLM that can correctly answer a question at the cheapest prediction cost. 

% Thus, we have a problem of choice: \emph{given a new question, which LLM is best suited to answer it?} 



The task of picking the best prediction model is called \emph{routing} and has attracted a growing interest in the LLM community \citep{lu2023routing,wang2023fusing}, due to it's capability of harnessing the complementary expertise of a heterogeneous class of LLMs to achieve better performance at a reduced prediction cost. 
% To formally introduce the problem, assume that we have access to $M$ pre-trained models $f_1, \dots, f_M: \cX \to \cY$ and given a new $X\in \cX$ we need to pick the ``best capable'' one to predict $Y$. 
In this paper, we consider routing with two metrics, namely prediction error and cost, but our framework can also be extended to more than two metrics (\cf\ Section \ref{sec:general-multi-obj}). As hinted before, the two metrics are often at odds with each other: a larger model will have a smaller prediction error, but at a higher cost, whereas a smaller model will have a lower prediction cost but a higher prediction error. This is a well-known issue in most multi-objective learning problems and in such scenarios it is often standard to consider a ``trade-off'' between the prediction error and the cost via a simple weighted linearization: for $\lambda \in [0,1 ]$ we define the trade-off loss as 
\begin{equation} \label{eq:linearized-loss}
  \eta_{\lambda, m}(X, Y) =  \lambda \ell\{Y, f_m(X)\} + (1 - \lambda) \kappa_m(X)  \,.
\end{equation}
For such a particular trade-off our routing problem is formalized as the following: learn a function $g: \cX\to \{1, \dots, M\}$ 
that predicts the index of the model to be used for predicting the final outcome, \ie\ given an $(X, Y)$ we predict $Y$ as $f_{g(X)}(X)$. We refer to such a $g$ as \emph{router}. We want to learn the best possible router, also referred to as oracle router and Pareto router, that  
minimized the average trade-off loss: 
\begin{equation} \label{eq:risk-trade-off}
  \textstyle g_\lambda^\star =   \argmin_g \big \{ \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y) \big]\big \} \,.
\end{equation} Here, the $\lambda$ in the subscript of  $g_\lambda^\star$ emphasises the dependence of oracle router on the trade-off parameter $\lambda$, as for different $\lambda$'s the  $g_\lambda^\star$'s might be different. 

By this point, the readers may have realized that this is inherently a classification problem; routers are essentially classifiers, whose outcomes are indices of LLMs. Often, this is more tractable than learning a predictor $f:\cX \to \cY$ from scratch or through fine-tuning, especially when $P$ includes a diverse set of prediction tasks. 
Both of our benchmark datasets contain the
MMLU \citep{hendrycks2020measuring},
which is a multiple choice question-answer benchmark with 57 different tasks organized by topics. The Open LLM Leaderboard \citep{open-llm-leaderboard-v2} combines MMLU with five other question-answer datasets. While one may find it challenging to train an LLM that is strictly the best on all of these benchmarks, a more feasible approach is to \emph{route through} pre-trained models that are expert in those particular tasks.


Since routing is essentially a classification problem, we can use standard statistical learning techniques to learn the oracle routers; given a $\lambda$ we estimate $g_\lambda^\star$ using an empirical risk minimization (ERM): 
\begin{equation} \label{eq:ERM}
  \textstyle  \widehat g_\lambda = \argmin_g \frac1n \sum_{i = 1}^n \sum_{m = 1}^M \ell_{\text{class}}(g(X_i), m) \eta_{\lambda, m}(X_i, Y_i)\,. 
\end{equation} where $\ell_{\text{class}}$ is a suitable loss for multiclass classification. Moreover, we can evaluate the predictive error and cost for  $\widehat g_\lambda$ on a different test data split $\cD_\text{test} = \{(X_i' ,Y_i')\}_{i = 1}^{n_{\text{test}}} \sim  \textrm{iid} ~  P $: 
\begin{equation} \label{eq:perf-cost}
   \textstyle  \widehat \cE_\lambda  =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \ell\{Y_i', f_{\widehat g_\lambda(X_i')}(X_i')\}, ~~ \widehat \cC _\lambda =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \kappa_{\widehat g_\lambda(X_i')}(X_i')\,. 
\end{equation}



% In our formulation of model routing, we only need to learn a classifier with outcome space $[M]$ that selects the best-suited model for prediction. In other words, we have reduced the outcome space from an arbitrary $\cY$ to a mere $[M]$. 


% such that given a new $(X, Y)$ the model model indexed by $g(X)$ is best suited to predict the outcome $Y$, \ie\ 




% Now, we want to learn a function $g: \cX \to \{1, \dots , M\}$ which, for a new $X$, predicts that the model indexed by $g(X)$ is best suited to predict the outcome. We refer to this $g$ as \emph{router}. For a pair $(X, Y)$ a router $g$  incurs a trade-off loss $\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y)$, and naturally, we want to the best router that minimizes the average of trade-off loss: 
% \begin{equation} \label{eq:risk-trade-off}
%   \textstyle  \min_g \big \{ \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y) \big]\big \} \,.
% \end{equation}
% At this point, the reader may have realized that this is a classification problem with $M$ classes. Often, this is more tractable than learning a predictor $f:\cX \to \cY$ from scratch, especially when $\cY$ is very complicated. For our LLM example, $\cY$ is the space of all possible answers, and training a $f:\cX \to \cY$ is very difficult. In our formulation of model routing, we only need to learn a classifier with outcome space $[M]$ that selects the best-suited model for prediction. In another word, we have reduced the outcome space from  an arbitrary $\cY$ to a mere $[M]$. 




% \begin{itemize}
%     \item {\bf Prediction error:} we have a prediction loss function $\ell$ such that the loss for predicting a response $Y$ using the $m$-th model is $\ell\{Y, f_m(X)\} \in \reals$. We want to pick the model with the smallest loss. 
%     \item {\bf Prediction cost:} together with a pre-trained model $f_m$, we also have a cost function $\kappa_m: \cX \to \reals$ that, given an input $X$, quantifies the cost of obtaining the prediction $f_m(X)$ as $\kappa_m(X)$. Usually, this prediction cost is related to factors such as the sizes of models, input tokens, etc. Although a large model (\eg\ GPT4) can accurately answer most questions, they are also more expensive to use. For a question that is easy to answer, we might turn to a smaller model, which can provide a good answer at a much lower cost. 
% \end{itemize}

% Now we are presented with a problem with multiple objectives: prediction error vs. cost. Moreover, they are often at odds with each other: a larger model will have a smaller prediction error, but at a higher cost, whereas a smaller model will have a lower prediction cost but a higher prediction error.  In such scenarios one often considers a ``trade-off'' loss between the prediction error and the cost via a simple weighted linearization: for $\lambda \in [0,1 ]$
% \begin{equation} \label{eq:linearized-loss}
%   \eta_{\lambda, m}(X, Y) =  \lambda \ell\{Y, f_m(X)\} + (1 - \lambda) \kappa_m(X)  \,.
% \end{equation}
% Now, we want to learn a function $g: \cX \to \{1, \dots , M\}$ which, for a new $X$, predicts that the model indexed by $g(X)$ is best suited to predict the outcome. We refer to this $g$ as \emph{router}. For a pair $(X, Y)$ a router $g$  incurs a trade-off loss $\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y)$, and naturally, we want to the best router that minimizes the average of trade-off loss: 
% \begin{equation} \label{eq:risk-trade-off}
%   \textstyle  \min_g \big \{ \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = m\} \eta_{\lambda, m}(X, Y) \big]\big \} \,.
% \end{equation}
% At this point, the reader may have realized that this is a classification problem with $M$ classes. Often, this is more tractable than learning a predictor $f:\cX \to \cY$ from scratch, especially when $\cY$ is very complicated. For our LLM example, $\cY$ is the space of all possible answers, and training a $f:\cX \to \cY$ is very difficult. In our formulation of model routing, we only need to learn a classifier with outcome space $[M]$ that selects the best-suited model for prediction. In another word, we have reduced the outcome space from  an arbitrary $\cY$ to a mere $[M]$. 
% In general, this routing approach is particularly suited for very complicated $\cY$, as in those cases learning a direct predictive model $f:\cX \to \cY$ usually requires a large dataset and computation resource.  



% Returning to our routing task,  we show in Lemma \ref{lemma:oracle-router}, for $\eta_{\lambda, m} ^\star(X) = \Ex_P [\eta_{\lambda, m}(X, Y) \mid X]$, the best router that minimizes the trade-off risk \eqref{eq:risk-trade-off} is $g_\lambda^\star(X) = \argmin_l ~ \eta_{\lambda, m} ^\star(X)$. We also refer to $g_\lambda^\star$ as a Pareto router. We can use standard statistical learning techniques to learn this Pareto routers; given a $\lambda$ we estimate $g_\lambda^\star$ using an empirical risk minimization (ERM): 
% \begin{equation}
%   \textstyle  \widehat g_\lambda = \argmin_g \frac1n \sum_{i = 1}^n \sum_{m = 1}^M \ell_{\text{class}}(g(X_i), m) \eta_{\lambda, m}(X_i, Y_i)\,. 
% \end{equation} where $\ell_{\text{class}}$ is a suitable loss for multiclass classification. Moreover, we can evaluate the predictive error and cost for  $\widehat g_\lambda$ on a different test data split $\cD_\text{test} = \{(X_i' ,Y_i')\}_{i = 1}^{n_{\text{test}}} \sim  \textrm{iid} ~  P $: 
% \begin{equation}
%    \textstyle  \widehat \cE_\lambda  =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \ell\{Y_i', f_{\widehat g_\lambda(X_i')}(X_i')\}, ~~ \widehat \cC _\lambda =  \frac1{n_\text{test}} \sum_{i = 1}^{n_\text{test}}  \kappa_{\widehat g_\lambda(X_i')}(X_i')\,. 
% \end{equation}



% \todo{revise from here.}
\noindent What is a suitable trade-off, \ie\ what is a good choice of $\lambda$? Instead of making this decision on our own, we want users to decide on this based on their preferred trade-off between performance and cost. To aid in this decision, we want to provide them with an estimate of the Pareto frontier curve to exhibit the trade-off in the prediction error and cost
\begin{equation}
    \textstyle \widehat \cF = \{(\widehat \cE _\lambda, \widehat \cC_\lambda ): \lambda \in [0, 1]\}\,, 
\end{equation} along with the class of all estimates of the oracle routers $\{\widehat g_\lambda: \lambda \in [0, 1]\}$. A naive approach could be to report both $\widehat g_\lambda$ and $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ on a sufficiently fine grid of $\lambda$, where for each $\lambda$ on the grid, they are estimated using eq. \eqref{eq:ERM} and \eqref{eq:perf-cost}. But this defeats one the main purpose of the routing problem, reducing the computational requirement, as we now need to learn $\widehat g_\lambda$ on this suitable grid of $\lambda$. 


% Suppose that we want users to pick this $\lambda$ according to their preferred trade-off between performance and cost. For this, we want to provide them with an estimate of the Pareto frontier curve for the error and cost trade-off $\widehat \cF = \{(\widehat \cE _\lambda, \widehat \cC_\lambda ): \lambda \in [0, 1]\}$ so that they can make informed decisions about $\lambda$. Notice that, to calculate $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ we require $\widehat g_\lambda$. So, a naive approach could be to learn $\widehat g_\lambda$ and $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ on a sufficiently fine grid of $\lambda$'s and then interpolate for $(\widehat \cE _\lambda, \widehat \cC_\lambda )$ on the remaining $\lambda$'s to estimate the full curve. But this defeats the main purpose of the routing problem, reducing the computational requirement, as we now need to learn $\widehat g_\lambda$ on this suitable grid of $\lambda$. 


\emph{\bf Is there a more efficient way?} In this paper, we devise a computationally efficient approach to learn $\widehat g_\lambda$ for all $\lambda \in [0, 1]$ and use them to calculate $\widehat \cF$. The key intuition of our approach lies in the mathematical form of the oracle routers:  we establish in Lemma \ref{lemma:oracle-router} that  $g_\lambda^\star(X) = \argmin_m \eta_{\lambda, m} ^\star(X)$  where the loss regression functions $\eta_{\lambda, m} ^\star(X) = \Ex _P[\eta_{\lambda, m}(X, Y)\mid X]$ can be decomposed as  
\begin{equation}\label{eq:reg-decomposition}
    \eta_{\lambda, m} ^\star(X) = \Ex _P[\eta_{\lambda, m}(X, Y)\mid X] = \lambda \Ex_P[\ell\{Y , f_m(X)\}\mid X] + (1 - \lambda) \kappa_m(X)\,. 
\end{equation} 
The decomposition follows directly from Eq. \eqref{eq:linearized-loss}. Within this decomposition, the $\kappa_m$ is known to us, and thus only the $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$ remains unknown. Note that, $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$ is a regression function to predict $\ell\{Y , f_m(X)\}$ using $X$, and therefore can be learned by training a regression model on the training samples, where $\ell\{Y_i, f_m(X_i)\}$'s are treated as responses instead of $Y_i$'s. Let us denote this estimator by $\widehat \Phi_m(X)$. Now, we can replace $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$ by $\widehat \Phi_m(X)$ within the decomposition in eq. \eqref{eq:reg-decomposition} to obtain a plug-in estimator for $\eta_{\lambda, m} ^\star(X)$, denoted as $\widehat \eta_{\lambda, m}(X)$. Then, our estimated router is simply $\widehat g_\lambda (X) = \argmin_{m} \widehat \eta_{\lambda, m}(X)$. In our whole procedure, we only need to estimate $M$ different regression functions $\Ex_P[\ell\{Y , f_m(X)\}\mid X]$, which is \emph{computationally more efficient} than to learn a router for each value of $\lambda$ on a suitable grid. 


While the procedure is computationally efficient, \emph{does it also lead to statistically efficient estimates of the oracle routers?} To answer this question, we perform a minimax investigation on the excess risk (defined in eq. \eqref{eq:excess-risk}), and show that for a suitable choice of $\widehat \Phi_m$ (\cf\ Remark \ref{cor:efficient-routers}) our plug-in routers achieve the minimax optimal rate of convergence. Broadly speaking, the steps in our minimax investigation are as follows: 
\begin{itemize}
    \item In Theorem \ref{thm:lower-bound} we consider a setting similar to non-parametric classification problems considered in \citet{audibert2007Fast} and establish a lower bound on the minimax rate of convergence for the excess risk.
    \item  In Theorem \ref{thm:upper-bound} we establish a matching upper-bound rate of convergence of excess risk when $\widehat \Phi_m(X)$ has a ``suitable'' rate of convergence (\cf\ Corollary \ref{cor:efficient-routers}). 
    \item In Section \ref{sec:reg-fn-estimate} we propose an estimate $\widehat \Phi_m(X)$ that achieves our desired rate of convergence. 
\end{itemize}
Finally, we utilize our approach on two benchmark datasets, namely \texttt{RouterBench}\footnote{https://huggingface.co/datasets/withmartian/routerbench}\citep{hu2024routerbench} and \openllm\
\footnote{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard} \citep{open-llm-leaderboard-v2}
to estimate the oracle routers and the Pareto frontier of error and cost trade-off. 
% Both of the benchmark datasets contain a diverse set of tasks, such as reasoning, math, coding, etc, which necessitates the routing rather than fine-tuning.  
As a sneak peek at our findings, in \routerbench\ through routing, we can achieve performance similar to GPT4 at half the cost, whereas $95\%$ of performance at less than $20\%$ of the cost. 


On a more technical side, our routing task, at its heart, is a multi-objective classification problem. Within this context, our contributions are the following: 
\begin{itemize}
    \item In the context of our routing application, we were required to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$. 
    \item  We establish minimax rates for multi-objective classification problems: in Section \ref{sec:lower-bound} we work with two objectives, namely performance and cost, which is relevant to our routing application, and in Section \ref{sec:general-multi-obj} we further extend the setting to a general instance of multiple objectives. In both cases, we establish that simple plug-in routers are minimax rate optimal for the entire collection of oracle routers. To the best of our knowledge, our paper is the first to analyze minimax optimality on the entire collection of oracle classifiers in classification problems with multiple objectives. 
    \item  For a multi-objective classification problem, we provide a computationally and statistically efficient approach to estimate all the oracle classifiers.  
\end{itemize}



% \SM{(1) talk about the extension to multi class classification, (2) introduction of a new notion of margin and explain how it relates to margin in binary case, (3) }

% We quantify the capability of a model in two front:


% % This problem is called the \emph{routing} problem. \SM{introduce some the routing and related linerature here.}
% % To formally introduce the routing problem, assume that we have access to $M$ pre-trained prediction models $f_1, \dots, f_M: \cX \to \cY$ and given a new $X\in \cX$ we need to pick the ``best capable'' one for our prediction task. We quantify the capability of a model in two front:




% \begin{itemize}
%     \item {\bf Accuracy:} for the response $Y$ and it's prediction $f_m(X)$ we consider a prediction loss function: $\ell\{Y, f_m(X)\} \in \reals$.        
%     \item {\bf Cost:} along with a pre-trained model $f_m$, we also receive a $\kappa_m: \cX \to \reals$ that, given an input $X$, quantifies the cost of obtaining the prediction $f_m(X)$ as $\kappa_m(X)$. \SM{say something a bit more about both loss and the cost.}
% \end{itemize} 



% Now, we're presented with a muli-objective problem, and for a given $\lambda > 0$ it is often standard to choose a combination  $\eta_{\lambda, m}(X, Y) \triangleq  \lambda \ell\{Y, f_m(X)\} + (1 - \lambda) \kappa_m(X)$. To this end, we want to learn a router $g: \cX \to \{1, \dots, L\}$ that minimizes our average cost-adjusted loss:
% \begin{equation}
%   \textstyle  \cL_P(g, \lambda) =  \Ex_P \big[\sum_{m = 1}^M \bbI \{ g(X) = l\} \eta_{\lambda, m}(X, Y) \big]\,.
% \end{equation}
% We provide the oracle router in the following  lemma: 







% \paragraph{The problem: learning the Pareto routers.} Of course, the oracle router depends on $\lambda > 0$, and given a $\lambda$ we can estimate the oracle router model as $\widehat g_\lambda$ using standard statistical learning techniques. But, say, we want to provide users with a class $\widehat \cG = \{\widehat g_\lambda: 0\le  \lambda \le 1\}$ that efficiently estimates the class $\cG^\star = \{g_\lambda^\star: 0\le \lambda\le 1 \}$ of oracle routers, which we call ``Pareto routers''. Together with them, we want to provide estimates of expected performance and cost in $P$, \ie\ an estimate of the Parato metric curve
% \begin{equation}
%     \cM^\star = \big\{ \big(\cL_P(g_\lambda^\star, 1), \cL_P(g_\lambda^\star, 0)\big): 0\le \lambda \le 1 \big\}
% \end{equation}
% so that the said users can make their own informed choice of $\lambda$ by looking at the performance vs. cost ``trade-off''. 

% \paragraph{Efficient learning of the Pareto routers.}
% How do we learn this $\widehat \cG$? Do we train separate routers for separate values of $\lambda$, which might be resource intensive? Through our minimax analysis, we show that $\cG^\star$ can be learned efficiently using a simple two-step procedure:


% \begin{algorithm}
%     \begin{algorithmic}[1]
% \Require data $\cD$
% \State Learn an ``efficient'' predictor $\widehat \Phi: \cX \to \reals^L$ for $\Phi^\star: \cX \to \reals^L$ where the $l$-th co-ordinate of $\Phi^\star(X)$ is $\Phi^\star_l(X) = \Ex_P[\ell\{Y, f_m(X)\}\mid X ]$. The term ``efficient'' is made more precise later in Section \ref{sec:upper-bound}. 
% \State For $0 \le \lambda \le 1$ estimate $\widehat g_\lambda$ as \begin{equation}\label{eq:eff-estimate-router}
%         \widehat g_\lambda(X) = \argmin_l \{\lambda \widehat \Phi(X) + (1 - \lambda) \kappa_m(X)\}\,. 
%     \end{equation}
% \end{algorithmic}
% \caption{Learning of Pareto routers}
% \label{alg:pareto-routers}
% \end{algorithm}


% This two-step procedure greatly reduces our computation burden for the learning of $\cG^\star$ since we no longer need to train $\widehat g_\lambda$ for individual $\lambda$'s, which can be computationally intensive. Instead, we only need to learn $\Phi^\star$ once and easily obtain the class $\widehat\cG$ from \eqref{eq:eff-estimate-router}. 

% \paragraph{Minimax investigation of Pareto routers.} To argue that our two-step procedure in Algorithm \ref{alg:pareto-routers} is minimax rate optimal,  we establish the following: For any $0\le \lambda\le 1$
% \begin{itemize}
%     \item Within a standard setting that is often considered in investigating minimax rates for non-parametric classification problems \citep{audibert2007Fast}, we establish a lower bound for the minimax rate of convergence for the excess risk of a router (\cf\ Theorem \ref{th:lower-bound} ). 
%     \item In Section \ref{sec:upper-bound} we show that as long as $\widehat \Phi$ satisfies the concentration bound in \eqref{} the excess risk of the $\widehat g_\lambda$ defined in \eqref{eq:eff-estimate-router} achieves the same minimax rate of convergence, which establishes that $\widehat g_\lambda$ is minimax rate-optimal.  
% \end{itemize}



% \paragraph{Application to the \texttt{RouterBench} dataset.} \texttt{RouterBench}\footnote{https://huggingface.co/datasets/withmartian/routerbench}\citep{hu2024routerbench} is a Q\&A dataset comprising of over $\sim 30000$ prompts and the responses from 11 different LLMs, along their associated costs and a performance scores. We use our proposed algorithm \ref{alg:pareto-routers} to learn the Pareto routers, where the performance score predictor $\widehat \Phi$ is trained on a training split of the dataset  and estimate the Parato metric curve on the remaining test split. \SM{Say somethings about the findings in a couple of lines. Keep it short.}


% \SM{Possible generalization to multiple metrics. This can go into conclusion section.}



\paragraph{Organization of the paper.} We end our introductory section with a short description of the organization of our paper. In Section \ref{sec:lower-bound} we establish information-theoretic lower bounds on the excess risk in estimating oracle routers and develop a computationally efficient algorithm to estimate them that achieves the same rates in their upper bound. In Section \ref{sec:routing-application} we use this algorithm for routing in two benchmark datasets. In Section \ref{sec:general-multi-obj} we extend the routing problem to general metrics and discuss an efficient estimation algorithm and establish minimax optimal rate of convergence for the oracle routers, which is in the similar vain in Section \ref{sec:lower-bound}. We end our paper with a discussion in Section \ref{sec:discussion}. 


\subsection{Related literature}


\paragraph{Performance vs cost trade-off in LLM predcitions.} Several recent studies have explored optimizing the cost and performance trade-offs in the implementation of
large-language models (LLMs). LLM-BLENDER \citep{jiang2023llm} ensembles outcomes from
multiple LLMs to select the best response. Frugal-ML, Frugal-GPT \citep{chen2020frugalml,chen2023frugalgpt} and FrugalFoE \cite{wang2023fusing} employ an LLM cascade to sequentially query LLMs until a reliable response is found. AutoMix \citep{madaan2023automix} relies on a smaller model to self-verify its response before potentially considering a larger model. While these approaches rely
on multiple LLM queries, our approach routes each query to a single LLM, an approach also considered in \citet{hu2024routerbench}. We complement these works by providing a statistically principled approach to learning this performance vs. cost trade-off. 

\paragraph{Ensemble learning.} The routing problem is closely related to ensemble learning that combines multiple models to obtain better performance. Classical ensemble methods include bagging (bootstrap aggregating), boosting, and
stacking (model blending) \citep{breiman1996bagging,breiman1996stacked,freund1996experiments,friedman2001greedy,wolpert1992stacked}. Most of these works implicitly assume that the models in the ensemble have \emph{similar expertise}, and
thus it is beneficial to aggregate their predictions, whereas in our case, models may have \emph{complementary expertise}, and averaging their outputs might be detrimental because most of them may not be suitable for an input. Therefore, we choose to predict using the model with the best outcome, rather than aggregating them. 

\paragraph{Minimax study in non-parametric classification.} One of the earliest work on the minimax rate of convergence in non-parametric classification settings is by \citet{audibert2007Fast}. These techniques were later adopted for investigating the ability of transfer learning under a distribution shift; some prominent examples being \citep{kpotufe2018Marginal,cai2019Transfer,maity2020Minimax}. All of these works consider binary classification with $0/1$ loss. In comparison, our minimax investigation differs in two fronts: we extend the settings to classification with more than two classes and general cost functions. 
% To quantify the difficulty of classification in our extended framework through a margin condition, as done in \citet{audibert2007Fast} for binary classification with $0/1$ loss, we needed to extend the notion of margin appropriately (\cf\ eq. 
 \eqref{eq:margin}). 

\paragraph{Multiobjective learning}

==> sections_arxiv/mild_density.tex <==
\section{Minimax study under mild density condition}

==> sections_arxiv/upper-bound.tex <==
\section{Efficient learning of Pareto routers} 
\label{sec:efficient-learning-algorithm}


\subsection{The upper bound}\label{sec:upper-bound}

Recall in Algorithm \ref{box:CARROT} we say that we require an ``efficient estimate'' $\widehat \Phi$ of the function $\Phi^\star$, whose $l$-th coordinate is $\Phi^\star_l(x) = \Ex_P[\ell\{Y, f_l(X)\mid X = x]$. Now, we make this statement precise and show that for such an $\widehat \Phi $ the excess risk \eqref{eq:excess-risk} achieves the rate in the lower bound \eqref{eq:lower-bound}. 

\begin{theorem}[Upper bound]\label{thm:upper-bound}
    Suppose that for some $\rho_1, \rho_2 > 0$ and any $n \ge 1$ and $t > 0$ and almost all $x$ with respect to $P_X$ we have the following concentration bound for $\widehat \Phi$:
    \begin{equation}\label{eq:concentration-phi}
        \max_{P\in \cP} P_{\cD_n} \big \{ \|\widehat \Phi(x) - \Phi^\star (x)\|_1 \ge t\big \} \le  \rho_1 \exp\big (- \rho_2 a_n t^2 \big )\,, 
    \end{equation}
    where $\{a_n; n \ge 1\}\subset \reals$ is a sequence that increases to $\infty$.  
    Fix a $\lambda \in [0, 1]$.  Then, if all the $P\in \cP$ satisfies the margin condition \ref{assmp:margin} with the parameters $(\alpha, K_\alpha)$ then there exists a $K> 0$ such that for any $n \ge 1$ the excess risk for the router $\widehat g_\lambda$ in \eqref{eq:eff-estimate-router} is upper bounded as 
    \begin{equation}
        \max_{P\in \cP} \Ex_{\cD_n}\big [\cE_P(\widehat g_\lambda,\lambda)\big ] \le K a_n^{-\frac{1+ \alpha}{2}}\,. 
    \end{equation}
    Thus, as long as $a_n = n^{{  2\beta/(2\beta + d)}}$  for any $\lambda \in [0, 1]$ the excess risk for the router $\widehat g_\lambda$ in \eqref{eq:eff-estimate-router} has the rate of convergence $a_n^{- {(1 + \alpha)}/{2}} = n^{- {\beta(1 + \alpha)}/{(2\beta + d)}}$ that matches with the lower bound rate in \eqref{eq:lower-bound}. 
\end{theorem}




% {\bf Question:} How can we find Pareto front solutions efficiently without using a back-tracking technique, \ie\ fit different $g$ for different $\lambda$? The hint is to learn $f^\star(x)$ as $\widehat f(x)$ and for a $\lambda > 0$ then define 
% \[
% \textstyle \widehat g _\lambda (x) = \delta _{\widehat l(x)}, ~~ \widehat l(x) =  \argmin_ l\big\{\ell (\widehat f(x_0), f_l(x_0)) + \lambda c_l (x_0)\big\}
% \] Show that $\widehat g_\lambda$ achieved the rate at lower bound. 


\subsection{Efficient learning of the loss regression function}
\label{sec:reg-fn-estimate}
We consider \emph{local polynomial regression} (LPR) to estimate the loss regression function. For a sample point $Z_i = (X_i, Y_i)$ we define the observed loss vector $\ell_i \in \reals^L$ where $[\ell_i]_l = \ell\{Y_i,f_l(X_i)\}$. Consider a symmetric kernel $\psi: \reals^d \to \reals_+$ and define $\Theta(\lfloor \beta \rfloor)$ as the class of all $\lfloor \beta \rfloor$-degree polynomials from $\reals^d$ to $\reals$. For a bandwidth $h > 0$ we define the LPR estimate as 
\begin{equation}
    \widehat \Phi_l(x) = \widehat\theta_x^{(l)}(0), ~~ \widehat \theta_x^{(l)} \in \argmin_{\theta \in \Theta(\lfloor \beta \rfloor)}  \textstyle \sum_{i = 1}^n \psi (\frac{X_i - x}{h}) \big [\ell \{Y_i, f_l(X_i)\} - \theta (X_i -x )\big]^2 \,. 
\end{equation}
In their Theorem 3.2 \citet{audibert2007Fast} establishes that for $h = n ^{-1/(2\beta + d)}$ the concentration bound in \eqref{eq:concentration-phi} is satisfied with $a_n = n^{-2\beta/(2\beta + d)}$, therefore the router derived from such $\widehat\Phi$ using \eqref{eq:eff-estimate-router} achieves the same rate of convergence as in the lower bound \eqref{eq:lower-bound}, \ie\ rate optimal. 

==> sections_iclr/experiments.tex <==
\section{Routing in benchmark case-studies}
\label{sec:routing-application}
We use CARROT (Algorithm \ref{alg:pareto-routers}) to perform routing on several benchmark datasets. %task on two benchmarks: {RouterBench} \citep{hu2024routerbench} and {Open LLM leaderboard v2} \cite{open-llm-leaderboard-v2}. The broad question that we address here is to understand the performance vs. cost trade-off in LLM predictions. 
% \SM{revisit this once we have all the expt. details.}


\subsection{Datasets} \label{sec:datasets}

%\begin{wrapfigure}[17]{r}{0.5\textwidth} % 'r' for right, '0.4\textwidth' for width

%\vspace{-0.3cm}
    %\centering
    %\includegraphics[width=\linewidth]{plots/open-llm.pdf} % Replace with your image file
    %\caption{This is a wrapped figure.}
    %\label{fig:wrapped}
    %\label{fig:open-llm-leaderboard}
%\end{wrapfigure}


\paragraph{RouterBench:} RouterBench \citep{hu2024routerbench} is a benchmark dataset for routing tasks consisting of approximately 30k prompts and responses from eleven ($M = 11$) different LLMs.  The data includes prompts from 8 benchmarks covering commonsense reasoning, knowledge-based understanding, conversation, math, and coding. %Paired with each question are model responses, estimated costs associated with the responses (which need to be predicted at test time), and finally a performance score on whether a model got the answer correct. All prompts have a single correct answer, and LLM predictions are compared with that correct answer to obtain a performance score as $0/1$, where $1$ corresponds to a correct answer.  
\paragraph{Open LLM leaderboard:} The {Open LLM leaderboard v2}\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard}} \citep{open-llm-leaderboard-v2} is an open-source benchmarking platform that comprises responses and evaluations of a collection of LLMs on six benchmarks comprising a diverse collection of tasks. %As before, the dataset includes the questions, responses from LLMs, and their evaluation scores as $0/1$ based on whether the answer was correct. 
%For this dataset, we focus on the scenario where cost can be deterministically computed for each LLM once we know the input prompt; this scenario is a good approximation to situations in which LLMs are required to sample just a few tokens to accomplish the target task. To compute the cost of an LLM query, we tokenize the input prompt and compute the cost according to the guideline of TogetherAI \footnote{\url{https://www.together.ai/pricing}}. We use $M=18$ different open language models both available in the Open LLM leaderboard v2 and on TogetherAI, including model families such as LLaMa-3.1, Qwen2.5, and Gemma 2. More related details are provided in the Appendix \ref{append:llms_open}. 
%We focus on the following five benchmarks (around 21k examples) from the Open LLM leaderboard v2, which comprise multiple-choice questions: MATH Lvl 5 \citep{hendrycks2021measuringmathematicalproblemsolving}, MMLU-PRO \citep{wang2024mmluprorobustchallengingmultitask}, BBH \citep{suzgun2022challengingbigbenchtaskschainofthought}, GPQA \citep{rein2023gpqagraduatelevelgoogleproofqa}, MUSR \citep{sprague2023musr}. These five benchmarks are varied and designed to simulate real-world scenarios where LLMs encounter a wide range of prompts. MATH Lvl 5 focuses solely on mathematical word problems, whereas MMLU-PRO and GPQA include both mathematical and advanced science questions. In contrast, BBH emphasizes logical deduction and linguistic reasoning challenges. Lastly, MuSR serves as a benchmark for assessing multistep soft reasoning tasks framed within natural language narratives. In situations in which queries are diverse, the router can explore the strengths and weaknesses of each language model.
\paragraph{\newdata:} We introduce (and evaluate CARROT on) \newdata, a large and diverse dataset designed for training and evaluating routers. \newdata\ integrates 13 state-of-the-art language models and prompts from 6 benchmarks, including GPQA \citep{rein2023gpqagraduatelevelgoogleproofqa}, MuSR \citep{sprague2024musrtestinglimitschainofthought}, MMLU-Pro \citep{wang2024mmluprorobustchallengingmultitask}, MATH \citep{hendrycks2021measuringmathematicalproblemsolving}, OpenHermes \citep{teknium_openhermes_2.5}, and RAGBench \citep{friel2025ragbenchexplainablebenchmarkretrievalaugmented}. Compared to existing routing benchmarks such as RouterBench, \newdata\ offers several key advantages: 
\begin{enumerate}
    \item \newdata\ encompasses a highly diverse set of questions, including instruction queries.
    % , which is feasible due to the evaluation based on LLaMa-3.1-70b-Instruct. 
    \item Unlike previous benchmarks, it does not rely on few-shot prompting and utilizes chat templates appropriate for each model, making it more representative of real-world use cases.
    \item It leverages LLaMa-3.1-70b-Instruct \citep{grattafiori2024llama3herdmodels} to evaluate LLM responses against the ground truth, similarly to \citet{ni2024mixeval}. This is crucial for evaluating on open-ended instruction queries as well as mitigating errors associated with traditional automatic evaluation methods like exact match.
    % \footnote{Without in-context examples and when using chat templates LLMs tend to perform better, but exact match evaluation is no longer reliable due to varying answer styles of LLMs.}
    \item We provide input and output token counts for each LLM-prompt pair, enabling flexibility when conducting cost-aware analysis.
\end{enumerate}
We will open-source \newdata\ and a platform that allows practitioners to extend \newdata\ by adding new queries and seamlessly evaluating state-of-the-art models on them. For further details, please refer to Appendix \ref{sec:append:sprout}.
% First,  Second,  Finally, 



%\SM{comment about the diversity in task in these two benchmarks? and how router can help? Connect this to intro.}

\subsection{Estimating the oracle router}
CARROT requires an estimate for the function $\Phi^\star_m(X) = \Ex_P[ Y_m\mid X]$. In our benchmark tasks, $Y_m$ is 2-dimensional, consisting of model performance measured as accuracy and model cost measured in dollars. In the RouterBench and \newdata\ datasets the cost is treated as unknown, while in the Open LLM leaderboard v2, most evaluations are likelihood-based, thus cost is essentially the length of the input, i.e., a known function. In all cases, the accuracy $Y_{\text{acc}, m}$ is binary, and thus %thus $\Phi^\star_m(X) = P(Z_m = 1\mid X)$.  
we can view its estimation as a binary classification problem, where our objective is to predict the probability that $m$-th model will answer the question $X$ correctly, \ie\ $P_m(X) = P(Y_{\text{acc}, m} = 1\mid X)$) $Y_{\text{acc}, m}$. Using this intuition, we train several multi-label classification models $\widehat P: \cX \to [0, 1]^M$ on a training data split consisting of $80\%$ of the full dataset, where the $m$-th coordinate of $\widehat{P}(X)$ is the predicted probability that $m$-th model accurately answers the question $X$. %, \ie\ $\widehat \Phi_m(X) = \widehat P(Z_m = 1\mid X)$. 
To train $\widehat P$ we consider two procedures: 
\begin{enumerate}
    \item  {\bf CARROT (KNN):} We embed the model inputs using the {text-embedding-3-small} model from OpenAI \citep{openai2023textembedding3small}. On these text embeddings, we train a multi-label K-nearest-neighbors (KNN) classifier.

    \item {\bf CARROT (Roberta):} We fine-tune the pre-trained weights of the {{roberta-base}}\footnote{\url{https://huggingface.co/FacebookAI/roberta-base}} architecture. In order to enhance efficiency, across $m$ we allow $\hat{P}$ to share the same network parameters, except for the final classification layer.
    
\end{enumerate}
%(i) We fine-tune the pre-trained weights of the {\texttt{roberta-base}}\footnote{https://huggingface.co/FacebookAI/\texttt{roberta-base}} architecture; to enhance efficiency across $m$ we allow $\hat{P}$ to share the same network parameters, except for the final classification layer. (ii) %{\texttt{roberta-base}}\footnote{https://huggingface.co/FacebookAI/\texttt{roberta-base}} and %\texttt{bert-base-case}\footnote{https://huggingface.co/google-bert/bert-base-uncased}. 
%o further enhance our predictive ability for model correctness, we take a simple multi-task learning approach \citep{caruana1993multitask} to train the $\widehat \Phi_m$'s; they share the same network parameters, except for the final classification layer, which is based on the assumption is that the representation at the penultimate layers for $\widehat \Phi_m$'s are identical. We utilize a \texttt{HuggingFace} API framework \footnote{https://huggingface.co/docs/transformers/en/tasks/sequence\_classification} for training the $\widehat\Phi$, whose exact choices of hyperparameters are provided in Appendix \ref{}. 

As mentioned above, in the RouterBench and \newdata\ task the cost remains to be estimated. We train multi-label regression models $\widehat C: \cX \to \reals^M$, where $\hat{C}_m(X) =\mathbb{E}[Y_{\text{cost}, m}|X]$ is the estimated cost of calling model $m$ for query $X$. In the case of \newdata\ we actually estimate the input and output token count, and convert this to a cost using collected pricing numbers (see Table \ref{tab:price_by_token_newdata}). Depending on the technique used for performance estimation, we use either the {roberta-base} or text-embedder plus KNN strategy outlined above for fitting $\hat{C}$ (note that the models may be altered for a multi-output regression task, but otherwise remain identical).  In the case of Open LLM leaderboard v2, we compute the cost of input $X$ by calculating its length measured as the number of input tokens and retrieving the price per token from TogetherAI (see Table  \ref{tab:llms_open} for prices per 1M of input tokens).

Having estimated the $\widehat \Phi_m$'s, we use them in Algorithm \ref{alg:pareto-routers} to estimate the oracle routers and predict their performances vs costs on the remaining $20\%$ test split of the dataset. These cost-accuracy tradeoff curves are provided in Figure \ref{fig:mainfig} (left for RouterBench), Figure  \ref{fig:mainfig} (right Open LLM leaderboard v2), and Figure \ref{fig:fmselect} (left for \newdata) along with the accuracies and costs of the individual LLMs within the dataset. 

%\SM{also plot how many $\%$ of times GPT4 was called by the router?}

% Our Algorithm \ref{alg:pareto-routers} requires an estimate for the loss regression function $\Phi^\star_m(X) = \Ex_P[\ell\{ Y, f_m (X)\}\mid X]$. Furthermore, a key takeaway from our rate upper bound analysis in Section \ref{sec:upper-bound} is that the performance of our estimated routers depends on the rate of convergence for estimating $\Phi^\star_m(X) = \Ex_P[\ell\{ Y, f_m (X)\}\mid X]$. Alternatively speaking, we need to estimate $\Phi^\star_m(X)$ accurately. 

% Returning to our benchmark case-studies, the $Z_m = \ell\{ Y, f_m (X)\}$'s are binary, and thus $\Phi^\star_m(X) = P(Z_m = 1\mid X)$.  Therefore, we can view the estimation of $\Phi^\star_m(X)$ as a binary classification problem, where our objective is to predict whether the model $m$ will answer the question $X$ correctly. Using this idea, we train a multi-label classification model $\widehat \Phi: \cX \to [0, 1]^M$ on a training datasplit consisting of $80\%$ of the full dataset, where the $m$-th coordinate of $\widehat \Phi(X)$ is the predicted probability that $m$-th model accurately answers the question $X$, \ie\ $\widehat \Phi_m(X) = \widehat P(Z_m = 1\mid X)$. We train $\widehat\Phi$ with \texttt{\texttt{roberta-base}}, \texttt{bert-base-case} architectures. To further enhance our predictive ability for model correctness, we take a simple multi-task learning approach \citep{caruana1993multitask} to train the $\widehat \Phi_m$'s; they share the same network parameters, except for the final classification layer. 

% Having estimated the $\widehat \Phi_m$'s we use them in our Algorithm \ref{alg:pareto-routers} to estimate the Pareto routers and predict their performances vs costs on the remaining $20\%$ test split of the dataset. These accuracy-cost trade-off curves are provided in Figure \ref{}, along with the accuracies and costs of the individual LLMs within the dataset. 

\subsection{Baseline methods}
%We consider two families of benchmarks. The first is a collection of methods that learn a binary router from preference data, while the second baseline is an inefficient version of our estimates for the routing Pareto frontier.
\citet{ong2024routellmlearningroutellms} (RouteLLM) proposes a collection of methods for learning binary routers from preference data (data consisting of queries $q$ and labels $l_{i,j}$ indicating a winner between model $i$ and $j$). While the usage of preference data is slightly different from ours, we implement their methods on our data by creating pseudo-preference data between two models. In particular, we select a costly and high-performing model and a cheaper model and say the costly model wins if and only if it is correct while the cheaper model is incorrect. On this pseudo preference data, we fit two methods from \citet{ong2024routellmlearningroutellms} for learning win probabilities between expensive and cheap models: the first is a matrix factorization method, called {\bf RouteLLM (MF)}, while the second uses fine-tuned {roberta-base}, called {\bf RouteLLM (Roberta)}. A follow-up method to these is Routing on Random Forests (RoRF) from Not-Diamond \citep{notdiamond2023rorf}, referred to as {\bf Not-Diamond RoRF}. This method uses a text-embedder and random forest model to predict the win probability; we provide a comparison to this method with the {text-embedding-3-small} embedder from OpenAI. As in \citet{notdiamond2023rorf}, we use a slightly different procedure to construct the preference data; a label can take one of four possible values (one for each combination of correct/incorrect from each model), and the costly model is favored if either both models are wrong or the cheaper model is incorrect while the expensive model is correct. For RouterBench, we consider GPT-4 and mixtral 8x7b to be the costly and cheaper models while for the Open LLM Leaderboard, we use Qwen2.5 72b and Qwen2.5 7b.

%\textbf{ERM Router:} In the original RouterBench paper, the authors propose using empirical risk minimization (ERM) and linear interpolation to traverse the routing Pareto frontier \citep{hu2024routerbench}. We implement the ERM router and demonstrate that our method allows the practitioner to traverse the Pareto frontier smoothly. This essentially acts as an empirical verification of Lemma \ref{lemma:oracle-router}
\subsection{Results} %In both {RouterBench} and {Open LLM leaderboard v2} benchmarks we train the loss regressor $\widehat \Phi$ over ten different training and test splits of the datasets that are determined by some prespecified seed values. In both Figures \ref{fig:open-llm-leaderboard} and \ref{fig:RouterBench} we provide error-bars for both average accuracy and cost metrics calculated for the individual LLMs and estimated routers for \openllm\ and \RouterBench\ benchmarks. In both cases, the effect of the baseline architecture (\texttt{\texttt{roberta-base}} vs \texttt{bert-base-case}) were negligible, as we did not see significant differences in the estimated Pareto curves. 

% \begin{figure}
%     \centering
%         \includegraphics[width=0.38\textwidth]{plots/RouterBench (2).pdf} 
%         %\caption{Test 1}
%         %\label{fig:RouterBench}
%     %\hfill
%     %\begin{minipage}{0.49\textwidth}
%       % \includegraphics[width=\textwidth]{plots/router-vs-gpt4.pdf}
%       %  \caption{Test 2}
%      %   \label{fig:router-vs-gpt4}
%     %\end{minipage}
%     \vspace{-0.3cm}
% \caption{RouterBench: performance of several routers and individual LLMs on test data-split.}
% \label{fig:RouterBench-main}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{plots/hf-leaderboard1.pdf}
%     \vspace{-0.3cm}
%     \caption{Open LLM leaderboard v2: performance of several routers and individual LLMs on test data-split.}
%     \label{fig:rexp_open_llm}
% \end{figure}


\begin{figure}
       \centering
       \begin{subfigure}
           \centering
           \includegraphics[width=0.4\linewidth]{plots/RouterBench2.pdf} 
           %\caption{RouterBench}
           %\label{fig:RouterBench-main}
       \end{subfigure}
       \begin{subfigure}
           \centering
           \includegraphics[width=0.4\linewidth]{plots/hf-leaderboard1.pdf}
           %\caption{Open LLM leaderboard v2}
           %\label{fig:rexp_open_llm}
       \end{subfigure}
       \caption{Left: Routerbench Right: Open LLM leaderboard v2}
       \label{fig:mainfig}
   \end{figure}

\paragraph{Performance against baselines:} In {RouterBench} we were unable to achieve significantly better accuracy than GPT-4; however, we were able to greatly reduce the prediction cost. A direct comparison between routers and GPT-4 with respect to average accuracy versus cost is provided in Figure \ref{fig:mainfig} (left), where we see that routers can achieve an accuracy similar to GPT-4 at half the cost, while achieving $95\%$ of the accuracy at only $20\%$ of the cost. On the other hand, we showed that CARROT can outperform the best model (Qwen2-72B) by a large margin in {Open LLM leaderboard v2} (see the right side of Figure \ref{fig:mainfig}). In both datasets, we see that our routers significantly outperform the binary routers of \citet{ong2024routellmlearningroutellms} and \citet{notdiamond2023rorf}. This is due to the fact that we route to \emph{all possible models}, which increases the accuracy coverage and decreases the cost of the cheapest accurate model for a given query.

%In {Open LLM leaderboard v2}, the model {Qwen2-72B} has the best accuracy ($0.563$) %\pm 0.008)
%but has the highest cost (\$$10^{-9}  %\pm 5.5 \times 10^{-6}
%$ per query) while in RouterBench GPT-4 has the best accuracy %($0.833 %\pm %0.008
%$) but has the highest cost (\$$3.3\times 10^{-4} %\pm 5.5 \times 10^{-6}
%$ per query).% Through routing, on Open LLM leaderboard v2 we were able to improve the accuracy almost by $5\%$ and reduce the prediction cost to one-fourth of the previous cost (see Figure \ref{fig:rexp_open_llm}). %(for $\lambda = 0.995$  and  {\texttt{roberta-base}} architecture the accuracy is... %$0.592 \pm 0.007$ and the cost is $5.08\times 10^{-5} \pm 8.8\times 10^{-7}$). 

To verify our theory, we also compare to the ERM router, which directly minimizes ERM risk of \eqref{eq:RM} for a particular combination of accuracy and cost metrics. CARROT matches the ERM router performance, as demonstrated in Appendix Figures \ref{fig:rbenchsupp} and \ref{fig:rexp_open_llm2}, verifying Lemma \ref{lemma:oracle-router}.%the theoretical findings.

% For simplicity, we reserve comparisons of our CARROT to the ERM router, that directly minimizes ERM risk of \eqref{eq:RM} for a particular combination of accuracy and cost metrics, to the supplementary material (\cf\ Figures \ref{fig:rbenchsupp} and \ref{fig:rexp_open_llm2}).

\paragraph{Performance on \newdata:} The performance of CARROT on \newdata\ is illustrated in Figure \ref{fig:fmselect} (left); a trend similar to our findings for RouterBench and the Open-LLM Leaderboard-v2 emerges. Moreover, Figure \ref{fig:IBMMix-spider} shows that CARROT can achieve similar or better performance of {GPT-4o} with a fraction of the cost. 
% \begin{figure}
%     \centering
% \includegraphics[width=.8\linewidth]{plots/fmselect_perf_cost.pdf}

% \vspace{-0.3cm}
%     \caption{Test performance on \newdata.}
%     \label{fig:ROOT In Distribution}
% \end{figure}


\begin{figure}[ht]
       \centering
       \begin{subfigure}
           \centering
           \includegraphics[width=0.38\linewidth]{plots/fmselect_perf_cost.pdf}
           %\caption{Accuracy versus cost performance on \newdata.}
           %\label{fig:ROOT In Distribution}
       \end{subfigure}
       \hspace{0.05\textwidth} % Space between subfigures
       \begin{subfigure}
           \centering
           \includegraphics[width=0.28\linewidth]{plots/fmselect_model_selection.pdf}
    %\caption{Left: Test Performance on \newdata\ Right: Model selection proportions on \newdata\ }
           %\label{fig:model selection}
       \end{subfigure}
       \caption{Left: Test Performance on \newdata\ Right: Model selection proportions on \newdata\ }
       %\caption{CARROT in \newdata.}
       \label{fig:fmselect}
   \end{figure}

%In \texttt{RouterBench}  the \texttt{gpt-4-1106-preview} model, which is often considered as the state of the art, had the highest accuracy ($0.788 \pm 0.004$) but at the highest cost ($0.003 \pm 4.02 \times 10^{-5}$). Although we were unable to achieve significantly better accuracy than GPT-4, we were able to greatly reduce the prediction cost. A direct comparison between routers and GPT-4 with respect to average accuracy versus cost is provided in Figure \ref{fig:router-vs-gpt4}, where we see that routers can achieve an accuracy similar to GPT-4 at half the cost, while achieving $95\%$ of the accuracy at only $20\%$ of the cost. 

%\paragraph{Ablation studies:}



% \begin{figure}[h]
%   \centering
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth]{plots/RouterBench.pdf}
%     \caption{First subfigure}
%     \label{fig:RouterBench}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.48\textwidth}
%     \includegraphics[width=\textwidth]{plots/router-vs-gpt4.pdf}
%     \caption{Second subfigure}
%     \label{fig:router-vs-gpt4}
%   \end{subfigure}
%   \caption{A figure with two subfigures}
%   \label{fig:main}
% \end{figure}


\paragraph{How CARROT chooses models:} %We take this opportunity to provide interpretable insights into our model selection process in this application. 
Figure \ref{fig:fmselect} (right) presents the distribution of selected models in \newdata\ across some (average cost, average accuracy) pairs in the test split. As we move from left to right in Figure \ref{fig:fmselect} (right), the selection strategy gradually shifts from prioritizing cost efficiency with smaller models such as {llama-3-2-1b-instruct} and {llama-3-2-3b-instruct} to favoring more capable and expensive models like {llama-3-3-70b-instruct}, {gpt-4o}, and {gpt-4o-mini}.

% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{plots/fmselect_model_selection.pdf}
%     \vspace{-0.3cm}
%     \caption{Model selection proportions on \newdata\ across several accuracies on the test split.}
%     \label{fig:model selection}
% \end{figure}




==> sections_iclr/intro.tex <==
\section{Introduction}
\label{sec:intro}


%The rapid advancement of large-language models (LLMs) is remarkable, as they 

% Large language models (LLMs) can now routinely tackle a variety of tasks in academic, industrial, and everyday contexts \citep{minaee2024large}. This continued success has inspired the rapid introduction of new LLMs for both general and specialized purposes. Although this abundance has the potential to provide practitioners with flexibility, the sheer number of options often makes it challenging to select a suitable model given budget and performance needs. In particular, given a question of interest, how should one know which LLM to send it to? In a perfect world, one might simply opt to use the most powerful model, but for many, this will quickly lead to prohibitive financial and computational costs. 



Large language models (LLMs) have demonstrated the capability to effectively address a diverse array of tasks across academic, industrial, and everyday settings \citep{minaee2024large}. This continued success has catalyzed the rapid development of new LLMs tailored for both general and specialized applications \citep{myrzakhan2024open}. While %the proliferation of these models
this offers practitioners increased flexibility, the vast number of available options may pose a daunting challenge in their real-world deployment. Particularly, determining the optimal LLM for a given query remains a significant challenge. In a perfect world, all queries can be routed to the most powerful model, but for many, this may quickly become prohibitively expensive.



% \begin{figure}[h]
%     \centering
%         \includegraphics[width=0.4\textwidth]{plots/fmselect_gpt4o_comparison.pdf} 
%         %\caption{Test 1}
%         %\label{fig:RouterBench}
%     %\hfill
%     %\begin{minipage}{0.49\textwidth}
%       % \includegraphics[width=\textwidth]{plots/router-vs-gpt4.pdf}
%       %  \caption{Test 2}
%      %   \label{fig:router-vs-gpt4}
%     %\end{minipage}
% \caption{Percent of GPT-4o performance achieved by CARROT across dataset at various discounted costs, where the blue dotted line indicates similar ($100\%$) performance to GPT-4o.}
% \label{fig:IBMMix-spider}
% \end{figure}

%Although some proprietary models, like GPT-4, offer outstanding performance, they often come with significant costs due to high API prices.

%A common approach to address this issue is to optimize LLMs to maintain a desirable performance at a uniformly cheaper cost. To do so, researchers have tried chain-of-thought reasoning \citep{wei2022chain,wu2023chain} to improve performance (at a relatively fixed cost), and weight quantization \citep{lin2024awq,zhao2024atom} or model distillation \citep{hsieh2023distilling}  to reduce model size. These techniques can be effective in reducing the serving cost of a single model but have not uniformly addressed the cost of deployment that LLMs often incur. %given the rapid rise in the number of available LLMs, these techniques are certainly not scalable in the long run. 


A common approach to address this issue %Another popular approach 
is \emph{routing} \citep{shnitzer2023large, hu2024routerbench, ong2024routellmlearningroutellms, notdiamond2023rorf,akota2024}. There are two paradigms of routing; \emph{non-predictive} routers repeatedly call LLMs and evaluate the responses to select the best one for a given query. Examples include Fusion of Experts (FoE) \citep{wang2023fusing}, FrugalGPT \citep{chen2024frugalgptTMLR}, and techniques that cascade answers from weak to strong LLMs \citep{yue2024largelanguagemodelcascades}. The obvious disadvantage non-predictive routing is the required inference of many LLMS for all queries, even those that are not suitable for the task at hand. As a workaround, researchers have also considered \emph{predictive routers}, which take LLM queries as inputs and output guesses at the most appropriate LLM.  %Routing has several advantages over optimizing a single LLM. First, as we shall see later, it treats each LLM as an input-output black-box, avoiding the need to delve into intricate infrastructure details, thus making it both flexible and scalable. Secondly, routing can allow practitioners to ``customize" the criteria by which LLM's are selected. 
A key limitation of the prior literature on predictive routing is \emph{the avoidance of the cost prediction problem}. In \citet{shnitzer2023large} only performance is considered. The methods RouteLLM %their router cannot handle the inclusion of cost into the model selection desiderata. 
\citep{ong2024routellmlearningroutellms} RoRF \citep{notdiamond2023rorf} incorporates model cost by creating binary routers that select between a large costly model and a cheap small model. While this does incorporate cost, we shall see that the reduced flexibility of binary routing leads to performance degradation in practice. Finally, in \citet{akota2024} cost prediction is considered, but the authors assume that cost may be inferred from available API pricing; this does not hold if model responses are open-ended, and thus may vary in length. 


%\my{discuss limitations of key methods: they don't explicitly consider cost. My paper just tries to choose best model; RouteLLM implicitly considers cost by routing between small and big models, but this limits its ability to benefit from diverse strengths of many available closed- and open-source models.}
%while a single LLM, especially the small ones, may struggle to perform well on an expanding landscape of LLM tasks, by escaping the reliance on a single LLM, routing allows us to benefit from the diversity of LLMs. 
% \SM{mention somewhere that the collection of LLMs can be easily extended on the fly.}

% Let us understand the task of routing from a statistician's point of view. Given spaces of inputs $\cX$ and outputs $\cY$ we have a collection of input-output black-box models, denoted as $f_1, \dots, f_M: \cX \to \cY$.


To address these shortcomings, we develop CARROT: a Cost AwaRe Rate Optimal rouTer and collect the Smart Price-aware ROUTing (\newdata) dataset. \newdata\ is representative of both performance and cost of state-of-the-art LLMs across varying practical use-cases. Additionally, we use it to train the final version of CARROT. CARROT is designed to function as an estimate of \emph{the oracle router}. As a concrete example of the oracle router, consider model performance and inference cost as the metrics of interest. First, based on their needs, a practitioner selects a convex combination of performance and cost as the model metric. Next, the oracle router takes in a query and produces the LLM that minimizes this specific model metric. To do this selection, the oracle router needs to perfectly predict the metrics of interest (cost, performance) for each model given any query. Inspired by this, CARROT %\my{before talking about plug-in, should we explain what an "oracle" router would look like. Then its limitations motivating the plug-in approach} This leads us to 
utilizes a simple two-stage approach. We first attain an estimator for each of the metrics (\eg\ cost and performance) for each model given a query, then we plug in these estimators to the formed risk function and select a model that minimizes the appropriate convex combination of the estimated metrics. Although CARROT utilizes a simple approach, it has three distinct advantages.
\begin{wrapfigure}[23]{r}{0.45\textwidth}
\vspace{-0.4cm}
  \begin{center}
     \includegraphics[width=\linewidth]{plots/fmselect_gpt4o_comparison.pdf} 
  \end{center}
  \caption{Percent of GPT-4o performance achieved by CARROT across datasets at various discounted costs, where the blue dotted line indicates similar ($100\%$) performance to GPT-4o.
  }
\label{fig:IBMMix-spider}
\end{wrapfigure}

 % \colorbox{red!5!white}
% {\parbox{\dimexpr\linewidth-2\fboxsep}{%
 % \begin{itemize}
  % \item {\bf Computational efficiency.} For any collection of models and any collection of metrics CARROT can estimate the oracle router for any convex combination of the metrics with only one stage of model training.
   %\item {\bf High-quality data} To obtain a router that can be subsequently used in practice, we collect a new routing dataset representative of both performance and cost of state-of-the-art LLMs and varying practical use-cases. 
   % verify the efficacy of CARROT on a new routing dataset  The final version of CARROT is trained on \newdata\, a new, high-quality, routing dataset we develop.
  % \item {\bf Statistical efficiency.} An information-theoretic minimax investigation reveals that CARROT is a statistically efficient estimator for the oracle router in terms of sample complexity.
 % \end{itemize}
 % }}

\paragraph{Computational efficiency:} A practitioner may be interested in several possible convex combinations to understand the trade-offs across various metrics. In that case, learning a router per combination may not be practical. Our approach allows re-use of a plug-in estimate of the metrics for each combination, easing computational concerns. Furthermore, the metrics of interest may vary from practitioner to practitioner. CARROT allows the flexible addition of any metrics; one only needs to acquire estimators for them. As a demonstration of CARROT's efficiency, we utilize it to estimate the Pareto frontier of performance and cost trade-off on 
% two classic benchmark datasets, 
{RouterBench}\footnote{\url{https://huggingface.co/datasets/withmartian/routerbench}}\citep{hu2024routerbench}, open-LLM-leaderboard-v2\
\footnote{\url{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard}} \citep{open-llm-leaderboard-v2}, and our new SPROUT dataset. %\newdata\footnote{\href{https://huggingface.co/datasets/CARROT-LLM-Routing/SPROUT}{\texttt{https://huggingface.co/datasets/CARROT-LLM-Routing/SPROUT}}} dataset.

\paragraph{New dataset for routing:} \newdata\ covers 13 state-of-the-art language models (e.g. Llama-3-herd \citep{grattafiori2024llama3herdmodels}, GPT-4o \citep{openai2024gpt4}, \etc ) and approximately $45$k prompts from 6 benchmarks covering RAG, science, reasoning, and GPT-4 generated user queries. For all models, we use zero-shot prompting and corresponding chat templates to represent practical use cases and collect input and output token counts to allow flexibility when studying cost-performance trade-offs. We defer further details about \newdata\ and its advantages over other routing datasets to Section \ref{sec:datasets} and Appendix \ref{sec:append:sprout}.

% Furthermore, to ensure that all \newdata\ queries represent real-world use cases, zero-shot prompting is used along with an evaluation system based on MixEval \citep{ni2024mixeval}. We defer further details about \newdata\ and its advantages over other routing datasets to Section \ref{sec:datasets} and Appendix \ref{sec:append:sprout}.

As a sneak peek, in Figure \ref{fig:IBMMix-spider}, we present the ratio of CARROT's performance to GPT-4o's \citep{openai2024gpt4} on several key benchmarks across diverse use cases represented in \newdata. At $30 \%$ of the cost, CARROT matches or exceeds the performance of GPT-4o on each benchmark. Both \newdata\ and the corresponding CARROT router will be publicly released.

% Of course, any router is only as good as the data that it is trained on. To ensure that CARROT is ready to accurately route a diverse set of queries to a state-of-the-art set of LLMs, we also develop (and train on) the Scalable Price-aware Routing (\newdata) dataset. \newdata\
 % covers 13 state-of-the-art language models (e.g. Llama-3-herd \citep{grattafiori2024llama3herdmodels}, GPT-4o \citep{openai2024gpt4}, \etc ) and approximately $45$k prompts from 6 benchmarks covering RAG, science, reasoning, and GPT-4 generated user queries. Furthermore, to ensure that all \newdata\ queries represent real-world use cases, zero-shot prompting is used along with an evaluation system based on MixEval \citep{ni2024mixeval}. We defer further details about \newdata\ and its advantages over other routing datasets to Section \ref{sec:datasets} and Appendix \ref{sec:append:sprout}.
 
%\my{discuss our new dataset - I'll write it}

% Collecting adequate data for training a router has its own challenges; one needs to collect answers along with their evaluations on performance and costs for each combination of LLMs and queries, which could make the whole data generating process expensive. Thus, statistical efficiency is also an important consideration for any routing procedure.

% Collecting adequate data for training router has its own challenge; inference for each query needs to be answers along with their evaluations on performances and costs need to be collected for each combination of LLMs and queries, which could make the data generating process expensive. Thus, statistical efficiency is also an important consideration for any routing procedure.

%Given that training data is not limitless \my{can mention that specifically for routing it is expensive to collect - gotta run all LLMs and evaluate everything - it could be made clear from previous paragraph too}, statistical efficiency is also an important consideration for any routing procedure. 

% \vspace{-0.2cm}

\paragraph{Statistical efficiency} Collecting adequate data to train a router is quite expensive as we need to generate and evaluate with every LLM for every query.
% challenging; for each LLM and every query one must collect a response \emph{and} an evaluation from a judge of that response. By necessity, this collection process must include inference from closed source models such as Claude 3.5 \citep{TheC3} and GPT-4o.  This makes the routing data gathering process expensive; for example, gathering \newdata\ for one model can cost hundreds of dollars.  %answers along with their evaluations on performance and costs for each combination of LLMs and queries, which makes whole data generating process expensive. 
% Clearly, routing data is not limitless, so
Thus, statistical efficiency is an important consideration for any routing procedure. To investigate statistical efficiency, we connect the routing problem to multi-objective classification with a wide class of possible loss functions (this depends on the convex combination of model metrics on hand). Here, identities of the possible models act as the label space of the multi-class classification problem. Given this, one contribution of our work is to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us to introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$.  Additionally, our work analyzes minimax optimality on the entire collection of oracle classifiers in classification problems with all possible trade-offs between multiple objectives, which, to the best of our knowledge, is a novel contribution.

For space purposes, we discuss how these contributions fit into the related literature in Appendix \ref{sec:related-work}.

%Our theoretical contributions allow us to establish that simple plug-in routers are minimax rate optimal. This, along with our empirical demonstrations, shows that CARROT is both computationally and statistically efficient. %approach to estimate the entire collection of oracle classifiers.
 
%a model like GPT-4 \citep{openai2024gpt4} may offer outstanding performance, but model calls often come with significant costs due to high API prices. On the other hand, a practitioner could opt to query an open-source LLM (e.g. a model in the Llama family \citep{grattafiori2024llama3herdmodels}) which comes with reduced pricing but at a possibly reduced performance.
%if for any query and any LLM (e.g GPT-4 \citep{openai2024gpt4} or Llama3 \citep{grattafiori2024llama3herdmodels}) the practitioner knew the associated cost and performance, they could always select the cheapest model that provides a satisfactory response.

%At this point, let us take a step back and provide more context to the ``best-suited'' models. A practitioner may be interested in various (conflicting) metrics such as various notions of accuracy, cost, and run time. As a concrete example, consider model performance and inference cost; a model like GPT-4 \citep{openai2024gpt4} may offer outstanding performance, but model calls often come with significant costs due to high API prices. On the other hand, a practitioner could opt to query an open-source LLM (e.g. a model in the Llama family \citep{grattafiori2024llama3herdmodels}) which comes with reduced pricing but at a possibly reduced performance. 
%This hints at a possible trade-off between various metrics of interest. To make it general and satisfy a broad spectrum of users' needs, this paper will develop routers for arbitrary trade-offs.
%\my{small models still cost money or have to self-serve; also cite papers for models} 
%Next, having decided on such a trade-off, the goal of the router is to predict the identity of the LLM that is expected to have the best possible trade-off value.

%This is a standard multi-class classification problem: one can form a trade-off risk function by combining the desired metrics with a suitable convex combination; then the goal is to take a query and pick the model that minimizes the risk. Here, identities of the possible models act as the label space of the multi-class classification problem. In an ideal world, we could produce an oracle router that always picks the model with minimum. To do so, one would need to perfectly predict the metrics of interest (cost, performance) for each model for any query. Inspired by this, we %\my{before talking about plug-in, should we explain what an "oracle" router would look like. Then its limitations motivating the plug-in approach} This leads us to 
%propose a simple two stage router in Section \ref{sec:setup}. We first attain an estimator for each of the metrics (e.g cost or accuracy) for each model given query $X$, then we plug in these estimators to the formed risk function and select a model that minimizes the appropriate convex combination of the estimated metrics.

%Given this, a predictive router is essentially a classifier that predicts the index of the best model, and thus can be efficiently learned by minimizing a standard classification loss using the pairs of query and convex combination of metrics. 

%Although this is a simple approach, it has a couple of distinct advantages. First, a practitioner may be interested in several possible convex combinations to understand the trade-offs across various metrics. In that case, learning a router per combination through direct optimization may not be practical. Our approach allows re-use of a plug-in estimate of the metrics for each model, easing computational concerns. Furthermore, the metrics of interest may vary from practitioner to practitioner. Our approach allows the flexible addition of any metrics; one only needs to acquire estimators for them.



%In short, our plug-in approach  has three advantages: 
%\begin{activitybox}

 %\paragraph{Simplicity.} It is simple, easily interpretable, and adapts to a broad spectrum of users' preferred trade-off, even when a new model or metric is introduced to the problem.

 %\paragraph{Computational efficiency.} It provides a computationally scalable approach to estimate routers for an arbitrary combination of metrics.


 %\paragraph{Statistical efficiency.} An information-theoretic minimax investigation reveals that the plug-in approach is statistically efficient in terms of sample complexity.

%\end{activitybox}



% \colorbox{red!5!white}{\parbox{\dimexpr\linewidth-2\fboxsep}{%
% \begin{itemize}
%  \item {\bf Computational efficiency.} It provides a computationally scalable approach to estimate routers for all combinations of metrics.
%  \item {\bf Statistical efficiency.} An information-theoretic minimax investigation reveals that the plug-in approach is statistically efficient in terms of sample complexity.
% \end{itemize}
% }}
   
%Empirically, our approach has been compared against several state-of-the-art routers on two benchmark datasets, namely {RouterBench}\footnote{https://huggingface.co/datasets/withmartian/routerbench}\citep{hu2024routerbench} and open-LLM-leaderboard-v2\
%\footnote{https://huggingface.co/spaces/open-llm-leaderboard/open\_llm\_leaderboard} \citep{open-llm-leaderboard-v2}
%to estimate the oracle routers and the Pareto frontier of performance and cost trade-off. 
% Both of the benchmark datasets contain a diverse set of tasks, such as reasoning, math, coding, etc, which necessitates the routing rather than fine-tuning.  
%As a sneak peek, in routerbench through our routing approach, we can achieve performance similar to GPT4 at half the cost, and $95\%$ of performance at less than $20\%$ of the cost. 

%On the theoretical side, the routing problem, at its heart, is a multi-objective classification problem with a wide class of possible loss functions (this depends on the convex combination of model metrics on hand). Given this, one contribution of our work is to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$.  Additionally, our work analyzes minimax optimality on the entire collection of oracle classifiers in classification problems with all possible trade-offs between multiple objectives, which, to the best of our knowledge, is a novel contribution.
%\my{we haven't established the connection between routing and classification yet - maybe do it earlier when explaining oracle router and plug-in router}

% Our theoretical contributions allow us to establish that simple plug-in routers are minimax rate optimal. This, along with our empirical demonstrations, shows that CARROTS is both computationally and statistically efficient. %approach to estimate the entire collection of oracle classifiers.

%\begin{itemize}
    %\item In the context of our routing application, we were required to extend previous minimax studies in nonparametric classification \citep{audibert2007Fast} on two fronts: (1) with more than two classes, and (2)  with general losses beyond $0/1$-loss. Both of these extensions require us introduce a generalized definition of margin (\cf\ eq. \eqref{eq:margin}), which reduces to the usual margin definition as in \citet{audibert2007Fast} when the classification task is binary and the loss is $0/1$. 
    %\item  We establish minimax optimal rates for multi-objective classification problems, which, to the best of our knowledge, is the first to analyze minimax optimality on the entire collection of oracle classifiers in classification problems with multiple objectives. 
    %\item  For a multi-objective classification problem, we establish that simple plug-in routers are minimax rate optimal, which provides a computationally and statistically efficient approach to estimate the entire collection of oracle classifiers.  
%\end{itemize}


\subsection{Notation and preliminaries}

To begin, let us introduce our notation. We have $M$ pre-trained LLMs indexed as $m \in [M] = \{1, \dots, M\}$ and $K$ metrics indexed as $k\in [K] = \{1, \dots, K\}$. %Throughout our paper, we index the models as $m \in [M]$ and the metrics as $k \in [K]$. 
We denote a generic input or query as $X\in \cX$, where $\cX$ is the space of inputs.  Thus, for any input $X$, the metrics of interest are stored in a $M\times K$ matrix. We denote this matrix as $Y \in \reals^{M \times K}$, whose $(m, k)$-th entry $[Y]_{m, k}$ is the metric value for obtaining a prediction from the $m$-th model evaluated with respect to $k$-th metric.  For all metrics, we assume that a lower value is preferred. With this convention, we shall also refer to them as risks. For a probability distribution $P$ in the sample space $\cX \times \reals^{M\times K}$ we assume that the training dataset $\cD= \{(X_i, Y_i)\}_{i = 1}^n$ is an $\iid$ sample from $P$. 

 For the probability distribution $P $ defined on the space $\cX \times \reals^{M \times K}$, we denote the marginal distribution of $X$ by $P_X$. Let us denote $\supp(\cdot)$ as the support of a probability distribution. Within the space $\reals^d$, we denote $\Lambda_d$ as the Lebesgue measure, $\|\cdot\|_2$ and $\|\cdot\|_\infty$ as the $\ell_2$ and $\ell_\infty$-norms, and $\cB(x, r, \ell_2)$ and $\cB(x, r, \ell_\infty)$ as closed balls of radius $r$ and centered at $x$ with respect to the $\ell_2$ and $\ell_\infty$-norms. 

==> sections_iclr/setup.tex <==
\section{Plug-in approach to routing}
\label{sec:setup}

%To describe the approach, let us introduce some notation. We have $M$ pre-trained LLMs indexed as $m \in [M] = \{1, \dots, M\}$ and $K$ metrics indexed as $k\in [K] = \{1, \dots, K\}$. %Throughout our paper, we index the models as $m \in [M]$ and the metrics as $k \in [K]$. 
%We denote a generic input or query as $X\in \cX$, where $\cX$ is the space of inputs.  Thus, for any input $X$, the metrics of interest are stored in a $M\times K$ matrix. We denote this matrix as $Y \in \reals^{M \times K}$, whose $(m, k)$-th entry $[Y]_{m, k}$ is the metric value for obtaining a prediction from the $m$-th model evaluated with respect to $k$-th metric.  For all metrics, we assume that a lower value is preferred. With this convention, we shall also refer to them as risks. For a probability distribution $P$ in the sample space $\cX \times \reals^{M\times K}$ we assume that the training dataset $\cD= \{(X_i, Y_i)\}_{i = 1}^n$ is an $\iid$ sample from $P$. 


We will consider a convex combination of our $K$ metrics with coefficients $\mu \in \Delta^{K-1} \triangleq \{(\mu_1, \dots, \mu_K): \mu_k \ge 0, \sum_k \mu_k = 1\}$ and a generic point $(X, Y)\sim P$. The $\mu$-th convex combination of the risks (or, $\mu$-th risk) can be written as $Y\mu\in \reals^{M}$, with the risk incurred for obtaining a prediction from the $m$-th model is 
\[
\textstyle [Y\mu]_m = \sum_{k = 1}^K [Y]_{m, k} \mu_k\,.
\] We want to learn a predictive router $g: \cX \to [M]$, that takes $X$ as an input and predicts the index of the LLM to be used for inference. The average $\mu$-th risk for using the router $g$ is 
\begin{equation}\label{eq:RM}
  \textstyle   \cR_P(g, \mu) = \Ex\big [\sum_{m = 1}^M[Y\mu]_m \bbI\{g(X) = m\} \big]\,. 
\end{equation} For a given $\mu$ let us refer to the minimizer $g_\mu^\star$ as an oracle router. Remember our objective: we would like to learn the oracle routers $g_\mu^\star$ at every value of $\mu$. While one may minimize an empirical risk corresponding to $\cR_P(g, \mu)$ to estimate the oracle router at a particular $\mu$, this approach is not scalable, any small change in $\mu$ would require refitting a new router. Given this, we develop a plug-in approach which lets us estimate the oracle routers at every value of $\mu$. The key intuition lies within an explicit form of the $g_\mu^\star$ that we provide in the next lemma. 
\begin{lemma} \label{lemma:oracle-router}
    Let us define $\Phi(x) = \Ex [Y\mid X = x]$ and $\eta_{\mu, m}(x) = \sum_{k = 1}^K \mu_k [\Phi (x)]_{m, k} $. Then for any $\mu\in \Delta^{K-1}$ the oracle router that minimizes $\cR_P(g, \mu)$ is 
    \begin{align} \label{eq:oracle-router-2}
        \textstyle g_\mu^\star(X) & \textstyle = \argmin_m ~ \eta_{\mu, m} (X)\\ 
       & \textstyle  = \argmin_m \big\{ \sum_{k = 1}^K \mu_k [\Phi (X)]_{m, k} \big\} \, \nonumber.
    \end{align}
\end{lemma}
The key conclusion of \ref{lemma:oracle-router} is the expression $ g_\mu^\star(X)= \argmin_m \{ \sum_{k = 1}^K \mu_k [\Phi (X)]_{m, k} \} $. %where we have isolated the effects of $\mu$. 
It suggests a straightforward approach to estimate $g_\mu^\star(X)$ at all values of $\mu$.  Namely, we only need to plug-in an estimate of $\Phi(X) = \Ex[Y \mid X]$ to the expression of $g_\mu^\star(X)$. Compared to minimizing empirical risk at different values of $\mu$, this plug-in approach is more scalable if the practitioner plans on tuning $\mu$. %In addition to estimating the routers, we also estimate the average risks 
%\[
%\textstyle \cR(\mu, k) = \Ex \big[\sum_{m = 1}^M[Y]_{m, k} \bbI\{g_\mu^\star(X) = m\}\big]
%\]
%on a test split of the dataset, which would be useful for understanding the trade-off across different risks.
We summarize our approach in algorithm \ref{alg:pareto-routers}. 
\begin{algorithm}
    \begin{algorithmic}[1]
\REQUIRE Dataset $\cD_n$
\STATE Randomly split the dataset into training and test splits: $\cD_n = \cD_{\text{tr}} \cup \cD_{\text{test}}$. 
\STATE  Learn an estimate $\hat \Phi (X)$ of $\Phi(X)$ using the $\cD_{\text{tr}}$. 
\FOR{$\mu \in \Delta^{K-1}$}
\STATE  Define $\widehat g_\mu(X) = \argmin_m \widehat \eta_{\mu, m}(X)$ where $\widehat \eta_{\mu, m}(X) =  \sum_{k = 1}^K \mu_k [\widehat \Phi (X)]_{m, k}   $. Break any tie within $\argmin$ randomly.
 \STATE Calculate 
 
 $\widehat \cR(\mu, k)  =  \frac1{|\cD_{\text{test}}|} \sum\limits_{(X, R) \in \cD_{\text{test}}}  [R]_{m, k} \bbI\{ \widehat g_\mu(X) = m\} $
\ENDFOR

\STATE {\bfseries Return:} $\{\widehat g_\mu: \mu \in \Delta^{K-1}\}$ and $ \{\widehat \cR(\mu, k): \mu \in \Delta^{K-1}, k\in [K]\}$. 
\end{algorithmic}
\caption{CARROT}
\label{alg:pareto-routers}
\end{algorithm}

%\begin{algorithm}[H]
  % \caption{ICL Refinement}\label{alg:label improvement}
%\begin{algorithmic}
  % \STATE {\bfseries Input:} Corrupted label pairs $\tilde{D}: \{(X_i, \tilde{Y}_i)\}_{i=1}^n$, source LLM $\cS$.
   %\REPEAT
   %\STATE Initialize $noChange = true$.
 %  \FOR{$i =1, 2, \dots, n$}
   %\IF{$x_i > x_{i+1}$}
  % \STATE Select in-context-learning examples  $\tilde{D}_{\text{ICL}}^i: \{(X_j, \tilde{Y}_j)\}_{j=1}^{n_{\text{ICL}}}$ from $\tilde{D}\backslash\{(X_i, \tilde{Y}_i)\}$
 %  \STATE Construct concatenated prompt $[\tilde{D}^i_{\text{ICL}} \circ X_i]$, and draw re-sampled label $\hat{Y}_i \sim \cS(\cdot|[\tilde{D}_{\text{ICL}} \circ X_i] )$.
   %\ENDIF
  % \ENDFOR
  % \STATE {\bfseries Return:} $\hat{\cD} \triangleq \{X_i, \hat{Y}_i\}_{i=1}^n$
   %\UNTIL{$noChange$ is $true$}
%\end{algorithmic}
%\end{algorithm}

%\SM{talk a bit about interpretibility and computational efficiency}
